No-Regret Caching via Online Mirror Descent

We study an online caching problem in which requests can be served by a local cache to avoid retrieval costs from a remote server. The cache can update its state after a batch of requests and store an arbitrarily small fraction of each file. We study no-regret algorithms based on Online Mirror Descent (OMD) strategies. We show that bounds for the regret crucially depend on the diversity of the request process, provided by the diversity ratio R/h, where R is the size of the batch, and h is the maximum multiplicity of a request in a given batch. We characterize the optimality of OMD caching policies w.r.t. regret under different diversity regimes. We also prove that, when the cache must store the entire file, rather than a fraction, OMD strategies can be coupled with a randomized rounding scheme that preserves regret guarantees, even when update costs cannot be neglected. We provide a formal characterization of the rounding problem through optimal transport theory, and moreover we propose a computationally efficient randomized rounding scheme.

==> 7.1._Experiments1.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate the performance of the different caching policies under synthetic traces and a real trace.  

\subsection{Experimental setup}


\subsubsection{Datasets.}
Throughout all experiments, we assume equal costs per file, i.e., $w_i = w'_i = 1, \forall i \in \mathcal{N}$. We generate the following synthetic datasets, summarized in Table~\ref{tab:notations_definitions}:


\noindent\textbf{Fixed Popularity.}
In this setting, we sample independently at any time individual requests from \emph{Zipf} distribution with exponent $\alpha = 0.8$. This distribution represents the popularity of the files.
We set the catalog size to $N =200$ and time horizon $T = 10^5$.  The cache capacity is $k = 10$, and the learning rate $\eta^*$ is the optimal learning rates corresponding to each algorithm.

\noindent\textbf{Batched Fixed Popularity}.
Similar to the above setting, we sample independently at any time individual requests from a \emph{Zipf} distribution. Except that the generated requests are grouped into batches of size $R = 5\times 10^3$. We take different exponents $\alpha$, this parameter controls the diversity of the files in the request batches. If $\alpha = 0$, then each file is requested with equal probability, %of each file to be requested,
corresponding to $\frac{R}{h} \to N$ (high diversity). As we increase $\alpha$, the requests become more concentrated; this corresponds to $\frac{R}{h} \to 1$ (low diversity). We consider exponents $\alpha \in \{0.1, 0.2, 0.7\}$, which  give  traces \emph{Batched Fixed Popularity} (1), (2), and (3), respectively, in Table \ref{tab:notations_definitions}. In all cases, we select catalog size $N = 200$, cache size $k \in \{2,5,10\}$, batch size $R = 5 \times 10^3$ and time horizon $T = 10^4$. 

\noindent\textbf{Transient Popularity}. We also generate two non-stationary request traces. In these traces, we reset the popularity distribution periodically.


In the first scenario, 
we consider a partial popularity change. Intuitively, we aim to model a situation where the supplier of the files periodically refreshes its library, and both catalog changes and the periods of stationarity are known (even though the popularity values are not).
  In every period of $10^3$ timeslots, the  we change the popularity of 10\% of the catalog  as follows: the popularities of most 5\% popular files are randomly assigned to the 
 least 5\% popular files, and vice versa.
 From the algorithmic perspective,
we set the targeted time horizon to be equal to the (known) period of stationarity; i.e., $T=10^3$. 
That is, when implementing OGD and OMD, we set the time horizon $T$ (used to determine $\eta$) to be equal to this period; at the end of each period $T$, we reset the caching decision of each algorithm, by spreading the mass uniformly among the files affected by this popularity change. %We set the period of stationarity to $T=10^3$. 
 This happens 5 times, resulting in a total of 5T batches in the entire trace. We  again generate different diversity regimes, with exponents $\alpha \in \{0.1, 0.4,0.7\}$, batch size $R=5 \times 10^3$, cache size $k =5$, catalog size $N = 500$. This gives  traces \emph{Partial Popularity Change} (1), (2) and (3), corresponding to the different exponents, respectively.
 

In the second scenario, we sample individual requests independently from a \emph{Zipf} distribution with exponent $\alpha=0.8$. Then, these individual requests are grouped into request batches. After every $5\times 10^4$ time slots we perform a circular shift by a step $50$ to the components of the popularity distribution vector. Hence,  the popularity profile of the requests changes significantly from one timeslot to the next. This gives the trace \emph{Changing Popularity}, with a total duration (total number of batches) of $15 \times 10^4$.


\noindent\textbf{Akamai CDN.}
We consider also a real file request collected from Akamai Content Delivery Network (CDN)~\cite{akamaiGiovanni}. We only consider 1 week of the Akamai CDN, and the catalog is truncated to  the $10^3$ most popular files. The requests arrive in batches of size $R = 5 \times 10^3$, and we target the time horizon to be the average number of batch requests collected in as single hour $ T = 100 $ ($5 \times 10^5$ individual file requests). The policies LRU, LFU and 2-LFU are allowed to process individual requests. We take the refresh periodicity of 2-LFU to be $T \times R$ requests. 



\begin{table}[!t]
%\centering
  \caption{Trace Summary}
  \label{tab:notations_definitions}
  \begin{tabular}{llllll}
    \hline
    Trace  & \# Batches &$T$ &$N$& $R$ & $h$ \\
    \hline
    Fixed Popularity & $10^5$ & $10^5$& 200&1 & 1\\
    Changing Popularity  & $15 \times 10^4$ & $15 \times 10^4$& 200&1 & 1\\
    Batched Fixed Popularity  (1) & $10^4$ & $10^4$&200& $5\times10^3$  & 40\\
    Batched Fixed Popularity  (2) & $10^4$ & $10^4$&200& $5\times10^3$  & 53\\
    Batched Fixed Popularity (3) & $10^4$ & $10^4$&200& $5\times10^3$  & 346\\
    Partial Popularity Change  (1)  & $5 \times 10^3$ & $10^3$&500& $5\times10^3$ & 40\\
    Partial Popularity Change  (2)  &  $5 \times 10^3$ & $10^3$&500& $5\times10^3$ & 169\\
    Partial Popularity Change  (3) &  $5 \times 10^3$  & $10^3$&500& $5\times10^3$ & 473\\
    Akamai CDN & $1.7\times 10^4$ & $10^2$ & $10^3$ & $5 \times 10^3$ & $380$ \\
    \hline
\end{tabular}
\end{table}

\subsubsection{Online Algorithms.} Starting with the gradient based algorithms, we implement $\OMD_\negent$ with the projection defined in Algorithm \ref{alg:bregman_divergence_projection}. We implement $\OGD$  using two implementations of the projection algorithm, one by Paschos et al. \cite{PaschosLearningToCache} for the setting $\frac{R}{h} = 1$, and one by Wang and Lu  \cite{wang2015projection} for the general setting $\frac{R}{h} \neq 1$. 

In addition, we implement the classical caching policies LRU, LFU and 2-LFU. LRU (least recently used) and LFU (least frequently used) are the classic caching policies. The 2-LFU is a Window-LFU \cite{karakostas2002exploitation}, where the time window is selected to be $W = T \times R$.  
Finally, we define \emph{Best Static} to be $\vec{x}^*
$, i.e. the state  storing the most $k$ popular files that is optimal when $w_i = 1, \forall i \in \mathcal{N}$. We also define \emph{Best Dynamic} to be the cache that stores the most $k$ popular files at any time for the synthetic traces. 

\noindent\textbf{Randomized Rounding.}
We also implement two rounding policies. To do so, we  generate fractional caching decisions by running $\OGD$ with learning rate $\eta = 0.01$. We round these both via (a) the independent sampling algorithm, and (b) the online coupled rounding 
in Algorithm \ref{algo:online_coupled_rounding}.


\subsubsection{Performance Metrics.} We measure performance  w.r.t.~four metrics  defined in Table~\ref{tab:performance_metrics}. The Normalized Average Cost $\mathrm{NAC}(\mathcal{A}) \in [0,1]$ corresponds the time-average fraction of cache misses up to time slot $t$, normalized by the batch size $R$.  The Normalized Moving Average Cost  $\mathrm{NMAC}(\mathcal{A}) \in [0,1]$ is computed similarly, using a moving average instead over a time window $\tau > 0$; we use $\tau = 500$ in this case.  We also consider the Time Average Regret $\mathrm{TAR} (\mathcal{A}) \in [0, R]$, which is precisely regret upto time slot $t$, scaled by $t$. Finally, when studying rounding algorithms, we also measure and report the Cumulative Update Cost $\mathrm{CUC}(\mathcal{A}) \in [0, \infty)$.

% \begin{table}[!t]
% %\centering
%   \caption{Performance Metrics}
%   \label{tab:performance_metrics}
%   \begin{tabular}{llll}
%     \hline
%     Performance metric & Definition & Range & Objective\\
%     \hline
%     Normalized Average Cost (NAC) & $ \displaystyle\mathrm{NAC} (\mathcal{A}) =  \frac{1}{R t} \sum^t_{s = 0 }f_{\vec{r}_s}(\vec{x}_s)$ & $[0,1]$ & $\downarrow$\\
%     Normalized Moving Average Cost (NMAC) &  $\displaystyle\mathrm{NMAC} (\mathcal{A}) =  \frac{1}{R \min(\tau,t)} \sum^t_{s = t-\min(\tau,t) }f_{\vec{r}_s}(\vec{x}_s)$& $[0,1]$ & $\downarrow$\\
%     Time Average Regret (TAR)& $\displaystyle\mathrm{TAR} (\mathcal{A}) = \frac{1}{t}\left(\sum^t_{s=1} f_{\vec{r}_s}(\vec{x}_s)- \sum^t_{s=1} f_{\vec{r}_s}(\vec{x_*}) \right)  $ & $[0,R]$ & $\downarrow$\\
%     Cumulative Update Cost (CUC) & $\displaystyle\mathrm{CUC} (\mathcal{A}) = \sum^t_{s=1} \updatecost_{\vec{r}_s} (\vec{x}_{s}, \vec{x}_{s+1} )$ & $ [0, \infty]$ & $\downarrow$\\
%     \hline
% \end{tabular}
% \end{table}

\begin{table}[!t]
%\centering
  \caption{Performance Metrics. All are better if lower.}
  \label{tab:performance_metrics}
  %\begin{small}
  \begin{tabular}{lll}
    \hline
    Performance metric & Definition & Range \\
    \hline
    Normalized Average Cost  & $ \displaystyle\mathrm{NAC} (\mathcal{A}) =  \frac{1}{R t} \sum^t_{s = 0 }f_{\vec{r}_s}(\vec{x}_s)$ & $[0,1]$\\
    Normalized Moving Average Cost  &  $\displaystyle\mathrm{NMAC} (\mathcal{A}) =  \frac{1}{R \min(\tau,t)} \sum^t_{s = t-\min(\tau,t) }f_{\vec{r}_s}(\vec{x}_s)$& $[0,1]$ \\
    Time Average Regret& $\displaystyle\mathrm{TAR} (\mathcal{A}) = \frac{1}{t}\left(\sum^t_{s=1} f_{\vec{r}_s}(\vec{x}_s)- \sum^t_{s=1} f_{\vec{r}_s}(\vec{x_*}) \right)  $ & $[0,R]$ \\
    Cumulative Update Cost & $\displaystyle\mathrm{CUC} (\mathcal{A}) = \sum^t_{s=1} \updatecost_{\vec{r}_s} (\vec{x}_{s}, \vec{x}_{s+1} )$ & $ [0, \infty]$ \\
    \hline
\end{tabular}
%\end{small}
\end{table}

%When comparing different policies, the static optimum incurs the same cost for all policies. Therefore it is enough to compare using the NAC metric instead of the regret. While in the real trace we use NMAC metric, to better capture the variability in real traces by averaging over the time window $\tau$, and we take $\tau = 500$.



%\subsubsection{Stationary requests under different diversity regimes}

%\subsubsection{Robustness to changing popularity requests}
% We first consider the scenario, where we have a partial popularity change. The supplier of the files is aware of the catalog change. Therefore, the targeted time horizon is the period of stationarity, this is take to be $T = 10^3 $. We reset the caching decision of each algorithm, by spreading the mass uniformly among the files affected by this popularity change. We generate different diversity regimes, with exponents $\alpha \in \{0.1, 0.4,0.7\}$, batch size $R=5 \times 10^3$, cache size $k =5$, catalog size $N = 500$. The popularity changes every $10^3$ requests, and we change 10\% of the catalog 5 times. Hence, $T= 5 \times 10^3$ is the total number of request batches. The change is a random shuffling of the popularity of the most 5\% popular files with least 5\% popular files. This gives the trace \emph{Partial popularity change trace} (1), (2) and (3) corresponding to the different exponents respectively.

  




==> acm-original-files/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> backup/S11-Related_work1.tex <==
Classical analysis techniques are based on the Time-to-Live (TTL) Caches. These cache models are used to encapsulate several caching policies such as LRU, FIFO and RND policies, this is analysed exactly by Berger et al. \cite{berger2014exact}, and approximately in the work of Gast and Houdt \cite{gast2017ttl}. The utility, or hit ratio are used as metrics to evaluate the performance of the different policies. 

Networks of caches found many applications in practice. This motivated several works to study the performance of cache networks. This is studied by Alouf et al. \cite{alouf2016performance} and Borst et al. \cite{borst2010distributed} for hierarchical network structures, e.g., the Domain Name Server (DNS) network architecture. More generally the work of Fong et al. \cite{fong1997}, Dehghan et al. \cite{dehghan2016complexity}, Ioannidis et al. \cite{ioannidis2010distributed} and Poularakis et al. \cite{poularakis2016exploiting} study distributed caching in networks.



%%%%%%%%%%% Adversarial, compare to dynamic optimum 
Caching under adversarial requests is a setting, in which the requests could potentially be generated by an adversary. A classical performance metric is to compare the performance of the cache relative to a dynamic optimum that is aware of the adversary's plan. This is classically studied under the name \emph{k-server} problem, this problem was introduced by Fiat et al. \cite{fiat1994competitive}. The performance metric is the bounded ratio between the cost experienced by a policy relative to a dynamic optimum. This ratio is called the \emph{competitive ratio}. More recently, Bubeck et al. \cite{bubeck_kserver_2018}, uses the framework of continuous online mirror descent to provide $o(k)$-competitive algorithm, that is independent of the underlying hierarchical separated tree (HST) metric.

%%%%%%%%%%% Adversarial, compare to fixed optimum
Recently, Paschos et al. \cite{PaschosLearningToCache} frame the caching problem as an online convex optimization problem. This setting also considers adversarial requests, with the distinction, that the performance metric is the difference between the cost experienced by a policy and the static optimum, this is called $regret$. They also give an online gradient descent policy that attains sub-linear regret. Bhattacharjee et al. \cite{FundamentalLimits} study the fundamental limits of this formulation.

% Regret vs Competitive ratio
Andrew et al.~\cite{taleoftwometrics} show that there is an intrinsic incompatibility between Regret and the competitive ratio, so that it is not possible for an algorithm to have both sub-linear regret and a constant competitive ratio. 

==> backup/S2-System_description1.tex <==
\section{System description}
\label{s:system}
\noindent\textbf{Remote Service and Local Cache.} We consider a system in which requests for files are served either remotely or by an intermediate cache of finite capacity. A cache miss incurs a file-dependent remote retrieval cost. Our goal is to study online algorithms for determining cache contents that attain sublinear regret. Formally, we consider stream of requests for  files of equal size from a catalog $\mathcal{N}=\{1,2,\dots, N\}$ .  These requests can be served by a remote server at cost $w_i \in \mathbb{R}_+$  per request for file $i\in\mathcal{N}$. This cost could be, e.g., an actual monetary cost for using the network infrastructure, or a quality of service cost incurred  due to fetching latency. Costs may  vary, as each file may be stored at a different remote location. We denote by %The cost of serving these files is summarized by a cost weight 
$\vec{w}=[w_i]_{i \in \mathcal{N}}\in \mathbb{R}_+^N$ the vector of costs %where $w_i \in \mathbb{R}_+$ is the cost of serving  file $i \in \mathcal{N}$. We assume that weights 
and assume that $\vec{w}$ is known.

 A local cache of finite capacity is placed in between the source of requests and the remote service. The local cache's role is to reduce the cost paid by the remote server, by satisfying requests locally. We denote by $k \in \{1,\dots,N\}$ the capacity of the cache. The cache is allowed to store fractions of files.  We assume that time is slotted, and  denote by $x_{t,i}\in[0,1]$  the fraction of file $i \in \mathcal{N}$ stored in the cache at  time slot $t \in \{1,2,\dots,T\}$.  The cache state is then given by vector $\vec{x}_t=[x_{t,i}]_{i\in \mathcal{I}}\in \mathcal{X}$, where $\mathcal{X}$ is the capped simplex  determined by the capacity constraint, i.e.: \begin{align}\mathcal{X} = \left\{ \vec{x} \in [0,1]^N : \sum^N_{i=1} x_i = k \right\}.\end{align}

\noindent\textbf{Requests.} We assume that a batch of multiple requests may arrive within a single time slot. Moreover, a file may be requested multiple times (e.g., by different users, whose aggregated requests form the stream reaching the cache) within a single time slot. We denote by $r_{t,i} \in \mathbb{N}$  the number of requests for file $i \in \mathcal{N}$ at time $t$, and by $\vec{r}_t=[r_{t,i}]_{i\in\mathcal{N}} \in \mathbb{N}^N$ the vector of such requests, representing the entire batch. We assume that the number of requests (i.e., the batch size) at each timeslot is given by $R \in \mathbb{N}$. We also assume that  the maximum multiplicity of a file in a batch is bounded by $h \in \mathbb{R}$. As a result, $\vec{r}_t$ belongs to set: 
\begin{align}\mathcal{R}_{R,h} = \left\{\vec{r} \in \{0,\dots, h\}^N : \sum^N_{i=1} r_i = R \right\}.\end{align}

Intuitively, the ratio $\frac{R}{h}$ defines the diversity of request batches in a timeslot. For example, as $\frac{R}{h} \to 1$, requests are concentrated on a single content. As $\frac{R}{h} \to N$, requests are spread evenly across the catalog $\mathcal{N}$. We note that this
generalizes Paschos et al.~\cite{PaschosLearningToCache}; their setting can be seen as the case $R = h = 1$ under our request model. 
We note that we make no prior assumptions on the stochasticity of request arrivals; put differently, we operate in the adversarial online setting, where a potential adversary may select an arbitrary request sequence in $\mathcal{R}_{R,h}$ to increase system costs.

\noindent\textbf{Service Cost Objective.} When a request batch  $\vec{r}_t$ arrives, the cache incurs the following cost:
\begin{align}
\label{e:cost}
f_{\vec{r}_t}(\vec{x}_t) = \sum^N_{i=1} w_i r_{t,i}(1 - x_{t,i}).\end{align}
In other words, for each file $i\in\mathcal{N}$, the remote server pays a cost proportional to the file fraction $(1-x_{t,i})$ missing from the local cache, weighted by the file cost $w_i$ and by the number of times $r_{t,i}$ that $i$ is requested in the current batch $\vec{r}_t$.


The cost objective \eqref{e:cost} captures several possible real-life settings. For example, assuming that each of the $R$ requests in the batch arrive and are served individually (e.g., either because they are spread-out within a timeslot, or because the fetching/QoS cost is paid separately for each user), leads to precisely the formulation in Eq.~\eqref{e:cost}. If, on the other hand, all requests are aggregated and served simultaneously, so that multiple requests for the same file are served by a single fetch operation, this can be captured by Eq.~\eqref{e:cost} with $h=1$ (so that the multiplicity of each file is at most 1, irrespective of how many users request it).

\noindent\textbf{Online Caching Algorithms and Regret.} Cache contents are determined online: that is, the cache has selected a state $\vec{x}_t \in \mathcal{X}$ at the beginning of a time slot.  The request batch $\vec{r}_t$ arrives, and the linear cost $f_{\vec{r}_t}(\vec{x}_t) : \mathcal{X} \to \mathbb{R}_+$ is incurred; the state is subsequently updated to $\vec{x}_{t+1}$. Formally, the  cache state is determined by an online policy $\mathcal{A}$, i.e.,  a sequence of mappings  $\{\mathcal{A}_t\}^{T-1}_{t=1}$, where for every $t \geq 1$, $\mathcal{A}_t : (\mathcal{R}_{R,h} \times \mathcal{X})^{t} \to \mathcal{X}$ maps the sequence of the request batches and previous decisions $\{(\vec{r}_s, \vec{x}_s)\}^{t}_{s=1}$ to the next state $\vec{x}_{t+1}\in \mathcal{X}$. We assume that the policy is initialised with a feasible state $\vec{x}_1\in \mathcal{X}$. 

 We measure the performance of an online algorithm $\mathcal{A}$ in terms of regret, i.e., the difference between the total cost experienced by a policy $\mathcal{A}$ over a time horizon $T$ and that of the best static state $\vec{x}_*$ in hindsight. Formally,
\begin{align}\text{Regret}_T(\mathcal{A}) = \underset{\{\vec{r}_1, \dots, \vec{r}_t\} \in \mathcal{R}^T_{R,h}}{\sup} \left\{ \sum^T_{t=1} f_{\vec{r}_t}(\vec{x}_t)- \sum^T_{t=1} f_{\vec{r}_t}(\vec{x_*}) \right\}. \label{eq:regret}\end{align}
where
$\vec{x_*}=\argmin_{\vec{x} \in \mathcal{X}}\sum^T_{t=1} f_{\vec{r}_t}(\vec{x})$ 
 is the optimal cache state (in hindsight). 
Note that, by taking the supremum in Eq.~\eqref{eq:regret}, we indeed measure regret in the adversarial setting, i.e., against an adversary that potentially picks requests in $\mathcal{R}_{R,h}$ trying to jeopardize  cache performance.
 
 %We are interested in the worst possible regret that can be incurred by $\mathcal{A}$:
%\begin{align}\text{Regret}_T(\mathcal{A}) = \underset{\{\vec{r}_1, \dots, \vec{r}_t\} \in \mathcal{R}^T_{R,h}}{\sup} \left\{ \sum^T_{t=1} f_{\vec{r}_t}(\vec{x}_t)-\underset{x_* \in \mathcal{X}}{\min} \sum^T_{t=1} f_{\vec{r}_t}(\vec{x_*}) \right\}. \end{align}

\noindent\textbf{Update Costs.} An online algorithm $\mathcal{A}$ updating the cache state at timeslot $t$ may require moving a portion of a file from a remote server to the cache. This is  not modeled in the cost (Eq.~\eqref{e:cost}) and, consequently, the regret (Eq.~\eqref{eq:regret}). This is indeed reasonable. First, the gradient-based algorithms we consider (see Sect.~\ref{sec:grad}) adapt the state by fetching fractions of files scaled by a gain $\eta\ll 1$; hence, by decreasing $\eta$, these update can be made arbitrarily small and, in particular, negligible compared to  file retrievals  satisfying requests, which are  accounted for in Eq.~\eqref{e:cost}. Second, even these negligible updates come for free for files requested in the previous timeslot. For example, increasing the $x_{i}$ for such a file $i$  can be performed by storing the small ($O(\eta)$) fraction of the ($1-x_i$) missing part of the file at the time of its retrieval. For these two reasons, we ignore this update cost in our analysis in  Sec.~\ref{sec:OMDanalysis}. In Sec.~\ref{xxx}, we revisit this issue, accounting also for update costs.   

==> backup/S4-Online_rounding.tex <==

\section{Online Rounding}
\label{sec:rounding}
In the previous sections, we assumed that the cache can store arbitrarily small chunks of a file. In practice the cache needs to store some metadata for each chunk and this overhead prevents the cache from splitting small files. These observations motivate us to study the case when the cache can only store the entire file, and the cache state consequently needs to be integral.

\subsection{Integral Caches} We denote the \emph{integral} cache configuration at time $t$ as $\boldsymbol{\zeta}_t$. It belongs to the set
%clearly a file can only have a finite number of chunks, and this can introduce application specific errors, e.g., rounding heuristics or the overhead cost caused by the chunks metadata, and these errors can be made more significant when the contents are small. To overcome these practical challenges, we are motivated to work with integral caching decisions. Let 
\begin{align}\mathcal{Z} = {\left\{ \boldsymbol{\zeta} \in \{0,1\}^N: \sum^N_{i=1} \zeta_i = k\right\}}.\end{align}
%be the set of possible integral cache configurations.

We are going to show that, by coupling OMD methods with opportune rounding techniques, the service-cost regret guarantees derived for the fractional setting transfer (in expectation) to the integral one. %
A straightforward approach is to use OMD to update a fractional state $\vec{x}_t\in \mathcal{X}$ and then randomly sample an integral state $\boldsymbol{Z}_t \in \mathcal{Z} $ after each round of requests so that $\mathbb{E}[\boldsymbol{Z}_t] = \vec{x}_t$, for all $t\geq 1$. 
%\begin{align}\mathbb{E}[\boldsymbol{Z}_t] = \vec{x}_t,\quad \text{for all}~t\geq 1.\end{align}
A random variable $\boldsymbol Z_t$ with the above marginals indeed exists, and can be sampled in polynomial time (see, e.g., \cite{geocaching2015, ioannidis2016adaptive}). In particular, 
Caratheodory's theorem \cite{rockafellar1970convex} guarantees that, for any~$\boldsymbol x_t$, the support of $\boldsymbol Z_t$ can be limited to at most $N$ cache configurations.  Warmuth and Kuzmin provided a practical algorithm~\cite[Algorithm 2]{WarmuthRandomizedPCA}.

When sampling occurs independently from the past, we refer to this rounding scheme as \emph{independent sampling}.
The expected service cost incurred through independent sampling is, by the linearity of $f_{\vec{r}_t}$: 
\begin{align}
  \mathbb{E} \left[\sum^T_{t=1} f_{\vec{r}_t} (\boldsymbol Z_t)\right] &=\sum^T_{t=1} \mathbb{E} \left[f_{\vec{r}_t} (\boldsymbol Z_t)\right] =\sum^T_{t=1} f_{\vec{r}_t} \left(\mathbb{E} \left[\boldsymbol Z_t\right]\right) = \sum_{t=1}^T f_{\vec{r}_t} (\vec{x}_t).
\end{align}
The best static configuration $\vec{x}_*$ in the fractional setting can always be selected to be integral; this is because the objective and constraints are linear, so integrality follows from the fundamental theorem of linear programming. Hence, the expected regret for the service cost coincides with the regret of the fractional caching policy.


\subsection{Update Cost} Similarly to  Sec.~\ref{sec:movement}, we can introduce the update cost as
\begin{align}
\label{eq:movement_integer}
\updatecost_{\vec{r}_t} (\boldsymbol\zeta_{t}, \boldsymbol\zeta_{t+1} ) = \sum_{i \notin \supp(\vec{r}_t)} w_i' \max(0, \boldsymbol\zeta_{t+1,i} - \boldsymbol\zeta_{t,i}),
\end{align}
and extend similarly the regret notion as in Eq.~\eqref{eq:regret_extended}. Unfortunately, the update cost \emph{cannot} be neglected in this integral setting: 
\begin{theorem}
\label{theorem:rounding_independent}
Online independent sampling can incur an extra update cost that is $\Omega(T)$ in expectation.
\end{theorem}
The proof can be found in Appendix \ref{proof:rounding_independent}. This result implies that, when considering the more general definition of regret including the update cost, OMD coupled with independent sampling loses its $\BigO{\sqrt{T}}$ regret guarantee. 
%
Independent sampling causes more frequent cache updates, as it samples $\boldsymbol\zeta_{t+1}$ ignoring the current state $\boldsymbol\zeta_t$. Intuitively, coupling the two consecutive states may significantly reduce the expected update cost. Moreover,  if we manage to achieve $\BigO{\sqrt{T}}$ update cost in expectation, by the upper bound in Eq.~\eqref{eq:rounding_regret_upper_bound}  the generalized  regret will also be $\BigO{\sqrt{T}}$. The following theorem provides a sufficient condition relating the expected update cost to the weighted $l_1$ norm of the fractional change $\vec x_{t+1} - \vec x_t$. The weighted $l_1$ norm is defined as
\begin{align}\norm{\vec{z}}_{1, \boldsymbol w'} :=  \sum^N_{i=1} w_i' |z_i|.\end{align}
%We observe that $\text{MC}_{\vec{r}_t} (\zeta_{t}, \zeta_{t+1} ) \le \norm{\zeta_{t+1} - \zeta_t}_{1, \boldsymbol w'}$.
We observe that $\updatecost_{\vec{r}_t} (\boldsymbol\zeta_{t}, \boldsymbol\zeta_{t+1} ) \le \norm{\boldsymbol\zeta_{t+1} - \boldsymbol\zeta_{t}}_{1,\boldsymbol w'}$.
\begin{theorem}
\label{theorem:rounding_coupled}
Consider an OMD Algorithm and a joint distribution of $(\boldsymbol Z_t,\boldsymbol Z_{t+1})$ %of the random variables $\boldsymbol\zeta_t$ and $\boldsymbolrho_{t+1}$,
that satisfies:
\begin{enumerate}
    \item $\mathbb{E}[\boldsymbol{Z}_t] = \vec{x}_t$ and $\mathbb{E}[\boldsymbol{Z}_{t+1}] = \vec{x}_{t+1}$.
    \item $\mathbb{E} \left[ \norm{\boldsymbol Z_{t+1} -\boldsymbol Z_{t}}_{1, \boldsymbol w'}\right] = \BigO{\norm{\vec{x}_{t+1} - \vec{x}_{t}}_{1, \boldsymbol w'}}$.
\end{enumerate}
This algorithm incurs an expected service cost equal to the service cost of the fractional sequence. Selecting $\eta = \Theta\left(\frac{1}{\sqrt{T}}\right)$, gives a \BigO{\sqrt{T}} expected update cost. The regret is therefore \BigO{\sqrt{T}}.
\end{theorem}
The proof can be found in Appendix \ref{proof:rounding_coupled}. In the following section we show that there exists a coupling satisfying the assumptions of Theorem~\ref{theorem:rounding_coupled}.

\begin{algorithm}[!t]
	\begin{algorithmic}[1]
		\Procedure {Online Coupled rounding}{$\vec{x}_t, \vec{x}_{t+1}, \vec{\zeta}_t, p_t$}
	    \State Compute $I = \left\{ i \in \mathcal{N}: x_{t+1,i} - x_{t,i} > 0 \right\}$.
	    \State $m_i \gets |x_{t,i+1} - x_{t,i}|$
	    \State Obtain a flow $[\delta_{i,j}]$ that transports $\sum_{i \in \mathcal{N} \setminus I} m_i$ mass from the nodes $i \in \mathcal{N} \setminus I$ to the nodes $j \in I$.
	    \State $\zeta, p \gets (\zeta_t, p_t)$
	    \For {$ i \in \mathcal{N} \setminus I$}
	        \For {$ j \in I $}
	        \State $\zeta, p \gets$ \textsc{Elementary $\delta$-movement}($\delta_{i,j}, i, j, \vec{x}, \vec{\zeta}, p, $)
	        \EndFor
	    \EndFor
	    \State $\zeta_{t+1}, p_{t+1} \gets \zeta, p$
	    \State \Return $\zeta_{t+1}, p_{t+1}$
		\EndProcedure
	\end{algorithmic}
	\caption{Online coupled rounding}
	\label{algo:online_coupled_rounding}
\end{algorithm}


\subsection{Online Coupled Rounding}
\label{sec:online_coupled_rounding}
Assume at time $t$ the random variable $\boldsymbol Z_t$ with $\mathbb{E}[{\boldsymbol Z_t}] = \vec{x}_t $ has been used to sample the integral state $\boldsymbol \zeta_t$ and that the a-priori probability to sample $\boldsymbol \zeta_t$ was $\mathbb P(\boldsymbol Z_t = \boldsymbol  \zeta_t) = p_t$. 

Algorithm~\ref{algo:online_coupled_rounding} takes as input the fractional states $\vec{x}_{t}$ and $\vec{x}_{t+1}$, the integral state $\boldsymbol\zeta_t$ and its corresponding probability $p_t$. It implicitly constructs a new random variable $\boldsymbol Z_{t+1}$ with $\mathbb{E}[\boldsymbol Z_{t+1}] = \boldsymbol x_{t+1}$ and samples the new integral state $\boldsymbol \zeta_{t+1}$ from it. In more detail, the algorithm generates a sequence of random variables whose marginal distribution is progressively closer to $\vec{x}_{t+1}$. The marginal distributions of two consecutive random variables differ only for a $\delta_{i,j}$ mass moved from file $i$ to file $j$, i.e., the marginal distribution changes from $\vec x$ to $\vec x - \delta_{i,j} \vec e_i + \delta_{i,j} \vec e_j$. 
Each intermediate random variable is sampled through the procedure \textsc{Elementary $\delta$-movement} that is detailed in Algorithm~\ref{algo:elementary_movement} in Appendix~ \ref{app:online_rounding}.
Algorithm~\ref{algo:online_coupled_rounding} returns the new state $\boldsymbol \zeta_{t+1}$ and its corresponding probability $p_{t+1}$.  
% G: REMOVED TO GAIN SPACE
%Note that the algorithm does not keep track of the probability distribution of each random variable $\boldsymbol Z_t$, but only of the probability such distribution assigns to the sampled state $\boldsymbol \zeta_t$.

Starting then from an arbitrary random variable $\boldsymbol Z_1$ with $\mathbb{E}[\boldsymbol Z_{1}] = \vec{x}_{1}$, we can at each time slot use a policy $\mathcal A$ to generate the new fractional state $\vec{x}_{t+1}$ and then Algorithm~\ref{algo:online_coupled_rounding} to sample the integral state. 

The following theorem shows that Algorithm~\ref{algo:online_coupled_rounding} used with an OMD algorithm satisfies the hypothesis of Theorem~\ref{theorem:rounding_coupled} and, hence, provides sublinear regret when the learning rate is opportunely selected.
\begin{theorem}
\label{theorem:algorithm_rounding_coupled}
Algorithm~\ref{algo:online_coupled_rounding} outputs a random integral cache configuration $\boldsymbol Z_{t+1}$ with $\mathbb E[\boldsymbol Z_{t+1}] = \boldsymbol x_{t+1}$.
If the input to Algorithm~\ref{algo:online_coupled_rounding} is sampled from a random variable $\boldsymbol Z_t$ with $\mathbb E[\boldsymbol Z_t] =\vec{x}_t$, then $\mathbb E_{\boldsymbol Z_t}\left[\mathbb E_{\boldsymbol Z_{t+1}| \boldsymbol Z_t} \left[\norm{\boldsymbol Z_{t+1} -\boldsymbol Z_{t}}_{1, \boldsymbol w'}\right]\right] =  \BigO{\norm{\vec{x}_{t+1} - \vec{x}_{t}}_{1, \boldsymbol w'}}$.
\end{theorem}
The proof can be found in Appendix \ref{proof:algorithm_rounding_coupled}. We show that the change from $\vec{x}_t$ to $\vec{x}_{t+1}$ can be decomposed in at most $N-1$ elementary operations (corresponding to calls to the procedure $\textsc{Elementary $\delta$-movement}$), and that for each of them 
the expected  $\vec{w}'$-weighted $l_1$-distance between the sampled integral configuration is bounded by 
$\delta_{i,j} (w'_i + w'_j + 2 \norm{\vec w'}_\infty)$.

Finally, we note that one can find the  joint probability distribution of  $\boldsymbol Z_t$ and $\boldsymbol Z_{t+1}$ by formulating an optimal transport problem \cite{peyre2019computational} to minimize $\mathbb E\left[\norm{\boldsymbol Z_{t+1} - \boldsymbol Z_t}_{1,\boldsymbol w'}\right]$. This approach may lead a smaller expected update cost, but it requires to explicitly consider all possible values of $\vec Z_t$ and $\vec Z_{t+1}$, that may be as many as $|\mathcal Z| = {N \choose k}$. Our algorithm instead efficiently builds the support of these random variables at each step to have size at most linear in $N$.



==> backup/Z-CacheNetworks.tex <==

\clearpage
\begin{center}
{\Large  Caching Networks}
\end{center}

\begin{table}[t!]
  \caption{Caching networks notation summary.}
  \label{tab:cn_notations_definitions}
  \begin{tabular}{c p{0.8\linewidth}}
    % \hline
    % Notation&Definition\\
    \hline
&\textbf{Caching Network} \\
\hline
    $G(\vertices, \edges)$ & weighted undirected graph with vertices $\vertices$ and edges $\edges$ \\
    $w_{(p_{u}, p_{v})}$ & weight of edge $(p_{u}, p_{v}) \in \edges$ \\
   $k^v$ & caching capacity of node $v \in \vertices$\\
   $\catalog$ & catalog of files \\ 
    $(i, \vec\path)$ & request for item $i \in \catalog$ along the routing path $\vec\path$\\
    $k_{\vec\path}(v)$ & the position of node $v \in \vec\path$\\
    $\requestSet $ / $ \requestSet_i$ & set of all possible requests / set of all possible requests for file $i$ \\
    $R$ & maximum number of requests in a request batch \\  
    $\pathSet$ & set of all possible routing paths \\
    $\vec r$ & request batch vector, where $r_{(i,\vec\path)}$ is the number of request for file $i$ along $\vec \path$\\
    $\setRequestBatch$ & set of all possible request batches \\ 
    $\vec\repo^v$ & vector of permanent allocations at node $v$, where $\repo^v_i$ indicates whether file $i$ is permanently stored at $v$ \\ $\vec\repo$ & vector of permanent allocations of the caching network\\
    $t$ & timeslot \\
    $T$ & time horizon\\
\hline
&\textbf{Fractional Caching Networks} \\
\hline
 $\x^v$ & fractional cache state of node $v$, where $x^v_i$ gives stored fraction of file $i$ at node $v$ \\
 $\statesSetFrac^v$ & set of all possible fractional caching configurations at node $v$ \\
 $\x$ & fractional cache state of the caching network\\
  $\statesSetFrac$ & set of all possible fractional caching configurations for the caching network\\
    $C_{\vec r}(\x)$ / $G_{\vec r}(\x)$ & caching network gain / caching network cost for the fractional state $\x$ when request batch $\vec r$ is received \\
    $\text{Regret}_{T, \statesSetFrac}(\mathcal{A})$ & regret of policy $\mathcal{A}$ over the fractional domain $\statesSetFrac$ and time horizon $T$\\
    $\updatecost^v (\x^v, \x'^v)$ & update cost at cache node $v$ when the cache state is changed from $\x^v$ to $\x'^v$\\
    $\widehat{\text{Regret}}_{T, \statesSetFrac}(\mathcal{A})$ & extended regret that includes the update cost\\
\hline
&\textbf{Integral Caching Networks} \\
\hline
 $\z^v$ & integral cache state of node $v$, where $x^v_i$ indicates whether file $i$ at node $v$ \\
 $\statesSetInt^v$ & set of all possible integral caching configurations at node $v$ \\
 $\z$ & fractional cache state of the caching network\\
  $\statesSetInt$ & set of all possible fractional caching configurations for the caching network\\
    $\psi\text{-Regret}_{T, \statesSetInt}(\mathcal{A})$ & discounted regret of policy $\mathcal{A}$ over the fractional domain $\statesSetInt$ and time horizon $T$\\
    $\psi\text{-}\widehat{\text{Regret}}_{T, \statesSetInt}(\mathcal{A})$ & discounted extended regret that includes the update cost \\
    $\psi$ & discounting factor equal to $1-\frac{1}{e}$ \\
   \hline
&\textbf{Distributed Online Mirror Ascent} \\
\hline 
$\Phi^v(\x^v)$ & local mirror map at node $v$ \\
$\Phi(\x)$ & global mirror map ($\Phi(\x) = \sum_{v \in \vertices }\Phi^v(\x^v) $) \\
$\eta^v$ & local learning rate at node $v$ \\
$\vec g$ & subgradient of the gain function\\
$\vec g^v$ & local subgradient at node $v$ \\
$\y$ &  intermediate cache state of node $v$ \\
$\Pi_{\statesSetFrac^v \cap \mathcal{D}^v}^{\Phi^v}(\y)$ & local projection of the intermediate cache state of node $v$\\
\hline
\end{tabular}

\end{table}



\section{Fractional Caching Networks}
\subsection{System Model}

Our system model is detailed below, and the notation used across the paper is summarized in Table~\ref{tab:cn_notations_definitions}.

\noindent\textbf{Cache Nodes.}  The caching network is modeled as an undirected weighted graph $G(\vertices, \edges)$, where $\weight_{(u,v)}$ is the weight of the edge $(u,v) \in \edges$. A vertex $v \in \vertices$ represents a cache node in the network, and the weight $w_{(u,v)}$  represents the routing cost along the communication link between cache nodes $u$ and $v$. 

We consider a stream of requests for files of equal size from a catalog $\catalog \triangleq \{1,2,\dots, N\}$. The catalog of files is guaranteed to be served within the network through designated repository cache nodes, and we denote by $\repoNodeSet_i$ the set of cache nodes that permanently store file $i \in \mathcal{N}$.
We define the permanent allocations $\repo^v_i$ at node $v \in \vertices$ determined by the sets of repository cache nodes, where $\repo^v_i = 1$ when $v$ permanently stores $i$ ($v \in \repoNodeSet_i$) , and  $\repo^v_i = 0$ otherwise; therefore, the vector of permanent allocations at node $v$ is given as $\vec \repo^v = [\mathds{1}_{\{ v \in \repoNodeSet_i\}}]_{i \in \catalog}$, and for all nodes $\vec \repo = [\mathds{1}_{\{ v \in \repoNodeSet_i\}}]_{(v,i) \in \vertices\times\catalog}$.


As in Sec.~\ref{s:system}, we assume that time is slotted, and we denote by $x^v_{t,i}\in [0,1]$  the fraction of file $i$ stored at node $v \in \vertices$  at timeslot $t \in \{1,2,\dots,T\}$.  The cache state is then given by vector $\vec{x}^v_t=[x^v_{t,i}]_{i\in \mathcal{N}}\in \statesSetFrac^v$, where $\statesSetFrac^v$ is the capped simplex  determined by the capacity constraint $\capacity^k$, i.e.: \begin{align}\statesSetFrac^v = \left\{ \vec{x} \in [\repo^v_i,1]^N : \sum^N_{i=1} x_i = k^v\right\}.\end{align}
Naturally, we can also define the fractional caching network state of the caching network at time slot $t$ as $\vec x = [x^v_i]_{(i,v) \in \catalog \times \vertices}$ in the set $\statesSetFrac \triangleq \bigtimes_{v \in \vertices} \statesSetFrac^v$. 

\noindent\textbf{Requests.}
We assume that every node has a predefined routing path towards a suitable repository node for each file $i \in \catalog$. The routing is therefore predetermined, and our decisions only concern placement of files (i.e., variables $x^v_m$).

A routing path $\vec \path$ of length $|\vec \path| = K$ is a sequence $\{\path_1, \path_2, \dots, \path_K\}$ of nodes $\path_k \in \vertices$ such that edge $(\path_k, \path_{k+1}) \in \edges$ for every $k \in \{1, 2, \dots, K{-}1\}$. We define $k_{\vec \path} (v)$ to be the position of node along a path $\vec \path$, where for every $\path_k \in \vec\path$ we have $k_{\vec \path} (p_k) = k $, otherwise $k_{\vec \path} (v) = +\infty$ for $v \not \in \vec \path$. We assume that paths are simple, i.e., they do not contain repeated nodes. Let $\pathSet$ be the set of all possible routing paths. A request is therefore characterized by the pair $(i, \vec \path)$, where $i$ is the file requested and $\vec \path$ is the routing path to be traversed. This mechanism is illustrated in Fig.~\ref{fig:system_model}.

We denote by $\requestSet$ the set of all possible requests, and by $\requestSet_i$ the set of all possible requests for file $i$. When a request for file $i$ is propagated from node $\path_1$ toward the associated repository node $\path_K \in \repoNodeSet_i$, any intermediate node along the path that stores $i$ can serve it. 

We consider a batch of requests can arrive within a timeslot. We denote by $r_{t,(i,\vec\path)} \in \mathbb{N} \cup \{0\}$  the number of requests for file $i \in \catalog$ along path $\vec \path$ at time $t$, and by $\vec{r}_t=[r_{t,(i,\vec\path)}]_{(i , \vec\path) \in \catalog \times \pathSet}$ the vector of such requests, representing the entire batch. We denote by $R$ the maximum number of requests that can be received at timeslot $t$ and by $\mathcal{B}$ the set of all possible request batches defined as 
\begin{align}
    \mathcal{B} \triangleq \left\{ \vec r \in \left(\naturals\cup \{0\}\right)^{\catalog \times \pathSet} : \sum_{(i,\vec \path) \in \catalog \times \pathSet } r_{(i, \vec \path)}\leq R\right\}.
\end{align}
When a request batch  $\vec{r}_t$ arrives, the system incurs the following cost:
\begin{align}
\label{e:cost}
C_{\vec r_t}( \vec x_t) = \sum_{(i,\vec\path) \in \requestSet} r_{t, (i, \vec \path)} \sum^{|\vec\path|-1}_{k=1} \weight_{\left(\path_k,\path_{k+1}\right)}\left(1- \min\left\{1, \sum^k_{k'=1} x^{\path_{k'}}_{i}\right\}\right),
\end{align}
 In other words, for request $(i, \vec \path)\in\requestSet$, the system pays a cost proportional to: (i) the number of times $r_{t,(i,\vec \path)}$ request~$(i,\vec\path)$ is received in the current batch $\vec{r}_t$, and (ii) the sum of routing costs $\weight_{\left(\path_k,\path_{k+1}\right)}$ scaled by the  file fraction $\left(1- \min\left\{1, \sum^k_{k'=1} x^{\path_{k'}}_{i}\right\}\right)$ remaining to be fetched  at node $\path_{k}$, until the first node $k_*$ is found such that $\sum^{k_*}_{k'=1} x^{\path_{k'}}_{i} \geq 1$.\footnote{When the files are  encoded by
rateless MDS coding (e.g., fountain codes~\cite{raptor2006}), a file can be decoded given that $M$ parity codes are received. As in~\cite{shanmugam2013femtocaching}, the fractional state $x^v_i$ represents the fraction of parity bit of file $i\in \catalog$ are stored at node $v \in \vertices$.} 
 
 Instead of working with the cost $C_{\vec r_t}( \vec x_t) $, we can equivalently consider the \emph{caching gain} defined as the cost reduction due to the presence of the caches (as in \cite{shanmugam2013femtocaching,ioannidis2016adaptive,neglia2019swiss}):
\begin{align}
G_{\vec r_t}( \vec x_t) &= C_{\vec r_t}( \vec\repo) -  C_{\vec r_t}(  \vec x_t) \\ &=  \sum_{(i,\vec\path) \in \requestSet} r_{t, (i, \vec \path)} \sum^{|\vec\path|-1}_{k=1} \weight_{\left(\path_k,\path_{k+1}\right)} \min\left\{1, \sum^k_{k'=1} x^{\path_{k'}}_{i}\right\}.
\label{e:gain_cache_network}
\end{align}
The first term $C_{\vec r_t}( \vec\repo)$ on the right hand side is the service cost when only the repository allocations are present in the network.  A summary of the 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{graphical_res/Aug/SystemCDN.pdf}
    \caption{Caching networks: a network of cache nodes can reply to  requests for files along predefined routing paths. A repository node at the end of each path ensures that requests are satisfied even when there are no allocations on intermediate cache nodes. }
    \label{fig:system_model}
\end{figure}

% \noindent\textbf{Offline Problem.} The static caching network allocation problem can be formulated as finding the caching network allocation $\vec x^*$ that maximizes the aggregate allocation gain  over the time horizon $T$, i.e., 
% \begin{align}
%   \vec x_*  \in \underset{\vec z \in \statesSetInt}{\arg\max}\left( \sum^T_{t=1} G_{\vec r_t}( \vec x)\right).
%   \label{eq:static_gain}
% \end{align}
% The gain function $G_{\vec r_t}$ is concave for any $\x \in \statesSetFrac$ and $\vec r_t \in \setRequestBatch$ and $\statesSetFrac$ is a convex set; thus, the offline problem is a convex optimization problem  that can be solved efficiently.
\noindent\textbf{Online Fractional Caching Networks Algorithms and Regret.} As in Sec~\ref{s:system}, the cache contents are determined online by an online policy $\mathcal{A}$.  We measure the performance of an online algorithm $\mathcal{A}$ in terms of regret. The regret is defined as the gain loss in comparison to the best static allocation in hindsight. Formally,

\begin{align}
\text{Regret}_{T, \statesSetFrac}(\mathcal{A}) = \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{B}^T}{\sup} \left\{ \sum^T_{t=1} G_{\vec r_t}(\vec{x}_*)-\sum^T_{t=1} G_{\vec{r}_t}(\vec{x}_t) \right\},
\label{eq:cn_fractional_regret}
\end{align}
where
$\vec{x_*}=\arg\max_{\vec{x} \in \mathcal{X}}\sum^T_{t=1} G_{\vec{r}_t}(\vec{x})$ 
 is the optimal static cache state (in hindsight). 
 
\noindent\textbf{Update Cost and Extended Regret}
We can extend the caching network model to include the update cost of the cache states  at the end of every time slot $t$. The update cost at node $v \in \vertices$ is defined as
\begin{align}
\updatecost^v (\x^v_{t}, \x^v_{t+1} ) = \sum_{i \in \catalog } w'^v_{i} \max(0, x^v_{t+1,i} - x^v_{t,i}),
\label{eq:cn_update_cost}
\end{align}
where $w'^v_i$ is the cost of retrieving file $i$ at node $v \in \vertices$. We can then define the extended regret as 
\begin{align}
\widehat{\text{Regret}}_{T, \statesSetFrac}(\mathcal{A}) = \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{B}^T}{\sup} \left\{ \sum^T_{t=1} G_{\vec r_t}(\x_*)- \sum^T_{t=1} G_{\vec{r}_t}(\x_t)  + \sum^T_{t=1} \sum_{v \in \vertices} \updatecost^v(\x^v_t, \x^v_{t+1})\right\}.
\label{eq:cn_fractional_extended_regret}
\end{align}

 
 
\begin{algorithm}[!t]
	\begin{algorithmic}[1]
	    \State Sample $\xi^v$ u.a.r in the interval $[0,1]$.
		\Procedure {OnlineMirrorAscent}{$\vec{x}_1 \gets\underset{\vec{x}^v \in \statesSetFrac^v \cap \mathcal{D}^v}{\arg\min} \,\Phi^v(\vec{x}^v),  \eta^v$}
		\State $\vec z_1 \gets \CoupledRounding(\vec x_t, \xi^v)$ \Comment{Sample the initial physical cache state}
		\For{$t \gets1,2,\dots,T$}\tabto {5cm}

		\State Compute $\vec g^v_t$ as in Sec.~\ref{s:distributed_gradient_computation} \Comment{Request batch $\vec r_t$}
		\State
		$\hat{\vec{x}}^v_t\gets\nabla {\Phi^v} (\vec{x}^v_t)$\tabto {5cm}\Comment{{ Map primal point to dual point}}
		\State
		$\hat{\vec{y}}^v_{t+1}   \gets\hat{\vec{x}}^v_t + \eta^v \vec g^v_t$\tabto {5cm}\Comment{{ Take gradient step in the dual}}
		\State
		$\vec{y}^v_{t+1}   \gets\left(\nabla {\Phi^v}\right)^{-1}(\hat{\vec{y}}^v_{t+1})$\tabto {5cm}\Comment{{ Map dual point to a primal point}}
		\State
		$\vec{x}^v_{t+1}\gets\Pi_{\statesSetFrac^v \cap \mathcal{D}^v}^{\Phi^v}(\vec{y}^v_{t+1})$\tabto {5cm}\Comment{{ Project new point onto feasible region}}
		\State $\vec z^v_t \gets \CoupledRounding(\vec x_t, \xi^v) $ \Comment{Sample a physical cache state.}
		\EndFor
		\EndProcedure
	\end{algorithmic}
	\caption{Online Mirror Ascent ($\text{OMA}_{\Phi^v}$).}
	\label{algo:cn_online_mirror_ascent}
\end{algorithm}

\subsection{Distributed Online Mirror Ascent over Caching Networks}
In this section, we propose a family of caching policies based on Online Mirror Ascent (OMA) denoted by \AlgoName{} that operate in a distributed fashion without requiring global knowledge of the allocation state and requests arrival. 

For every timeslot $t$ the policy \LocalAlgoName{} in Algorithm~\ref{algo:cn_online_mirror_ascent} configured with mirror map $\Phi^v: \mathcal{D}^v\to \mathbb{R}$ and learning rate $\eta^v \in \reals_+$ updates the fractional caching states $\x^v_t\in\statesSetFrac^v{\subset} [0,1]^\catalog$ at every node $v \in \vertices$.  \LocalAlgoName{} uses a local mirror map $\Phi^v: \mathcal{D}^v \to \mathbb{R}_+$  to map $\x_t^v$ to a dual space before applying the gradient ascent method using a local subgradient $\vec g^v$; 
then the obtained state is mapped back to the primal space (lines 6--8 of Algorithm~\ref{algo:cn_online_mirror_ascent}). To compute a feasible fractional state $\x_{t+1}^v$, we perform a projection to the set $\statesSetFrac^v$  on node $v$ (line 6 of Algorithm~\ref{algo:cn_online_mirror_ascent}). \AlgoName{} is the collection of \LocalAlgoName{} policies running at each node $v \in \vertices$.
% We configure at each node the neg-entropy mirror map $\Phi^v(\x^v) = \sum_{i\in\catalog}\x^v_{i} \log(\x^v_{i})$.

% \noindent\textbf{Integral State Update.}
% Once the fractional state $\x^v$ has been updated, the final step of \LocalAlgoName{} is to determine a new random discrete allocation $\z^v$ and update the physical cache state accordingly. 

% The sampled allocation $\z^v$ should \textit{(i)}~comply with the capacity constraint on node $v$ (i.e., $\z_v \in \statesSetInt^v$) and \textit{(ii)} be consistent with the fractional state, i.e., $\mathds{E}[\z^v_{i}] = \x^v_{i} \; \forall  i \in \catalog$. This is achieved by calling \CoupledRounding{} in Algorithm~\ref{algo:online_coupled_rounding}.


In the next subsection we detail how each node computes its contribution to the global subgradient.


\subsection{Distributed Subgradient Computation}
\label{s:distributed_gradient_computation}
At the end of every time slot $t$, a subgradient $\vec{g}_t$ of the gain function in Eq.~\eqref{e:gain_cache_network} at point $\x_t \in \statesSetFrac$  is computed in a distributed fashion: each node $v$ evaluates the $(v,i)$-th component of the subgradient for any $i \in \catalog$ as follows (see Appendix~\ref{appendix:subgradient_expression}):
\begin{align}
   g^v_{t,i} = \sum_{(i,\vec\path) \in \requestSet_i}  r_{t, (i, \vec \path)} \sum^{|\vec\path|-1}_{k=k_{\vec \path} (v)}  \weight_{\left(\path_k,\path_{k+1}\right)} \mathds{1}_{\left\{\sum^k_{k'=1}x^{\path_{k'}}_{i} <  1 \right\}}.
   \label{eq:subgradient_expression}
\end{align}
The denote by $\vec g_t^v = [g^v_{t,i}]_{i \in \catalog}$ the vector of subgradient components local to node $v \in \vertices$ at timeslot $t$.

The subgradient can be computed at each node using only information from the control messages collected at the end of the time slot $t$ that piggy-pack the requests traffic. The steps needed to compute the subgradient are as follows.
\begin{enumerate}
    \item  At the end of the time slot,  each node generates a control message for every received request type $(i, \vec \path) \in \requestSet$ that is propagated along $\vec \path$. The control message contains the quantity $r_{i, (i, \vec\path)} \geq 1$ (the multiplicity of the request), and a cumulative counter $Z$ initialized to zero.
    \item 
    As the control message travels upstream, intermediate nodes add to $Z$ the local values $x^{\path_{k'}}_i$. This message is propagated until $Z \geq 1$, and let $k_*$ be the rank of such cache node.
    \item Once the $k_*$-th node is reached, a control message is sent down in the opposite direction, accumulating the routing costs $\weight_{\left(\path_k,\path_{k+1}\right)}$ scaled by the request multiplicity $r_{i, (i, \vec\path)}$. Every node $v$ in the reverse direction reads the cost value from the control message and, for each file $i \in \catalog$, computes the quantity
    \begin{align}
        h^v_{(i, \vec \path)} = r_{t, (i, \vec\path)} \sum^{k_*}_{k = k_{\vec \path(v)}}  \weight_{\left(\path_k,\path_{k+1}\right)} = r_{i, (i, \vec\path)} \sum^{|\vec\path|-1}_{k = k_{\vec \path(v)}}  \weight_{\left(\path_k,\path_{k+1}\right)} \mathds{1}_{\{ \sum^k_{k'=1}x^{\path_{k'}}_{i} <  1\}}
    \end{align}
    \item
    Node $v$ can then compute $g_{t,i}^v$ in Eq.~\eqref{eq:subgradient_expression} as follows
    \begin{align}
    \nonumber
        g^v_{t,i}=  \sum_{(i, \vec\path ) \in \requestSet_i} h^v_{(i, \vec \path)}.
    \end{align}
\end{enumerate}


\subsection{Regret Analysis for Generic Mirror Maps}
\label{sec:cn_regret_analysis}
In order to establish the regret guarantee of \AlgoName{}, we make a set of assumptions on the local mirror maps $\Phi^v$ at every node $v \in \vertices$:
\begin{enumerate}[label=(A\arabic*)]
    \item The map $\Phi^v: \domainPhi^v\to \reals^{\catalog}$ is a valid mirror map (see Sec.~\ref{section:OMD}).\label{asp:first_assumption}
    \item The mirror map $\Phi^v$ is $\theta^v$-strongly convex w.r.t a norm $d^v:\reals^\catalog \to \reals_+$ over $\statesSetFrac^v \cap \domainPhi^v$.
    \item The dual norm of $d^v:\reals^\catalog \to \reals_+$ is $d^{*v}:\reals^\catalog \to \reals_+$.
    \item Any local subgradient $\vec g^v$ at node $v \in \vertices$ of subgradient $\vec g$ of $G_{\vec r}(\x)$ at point $\x \in \statesSetFrac$ and request batch $\vec r \in \setRequestBatch$ is bounded under the dual norm $d^{*v}:\reals^\catalog \to \reals_+$ by $L^v_{\max}$, i.e., $d^{*v}(\vec g^v)\leq L^v_{\max}$. 
    \item The Bregman divergence $D_{\Phi^v} (\x^v,\x^v_1)$ is upper bounded by $D^v_{\max}$ for every node $v \in \vertices$ and $\x^v \in \statesSetFrac^v \cap \domainPhi^v$ for any $v \in \vertices$, where $\x^v_1 = \arg\min_{\x^v \in \statesSetFrac^v\cap\domainPhi^v} \Phi^v(\x^v)$ (line 2 in Algorithm~\ref{algo:cn_online_mirror_ascent}).
    \item The $l_1$ norm is upper bounded by $d^v(\,\cdot\,)$ where   $\norm{\,\cdot\,}_1 \leq M^v d^v(\,\cdot\,)$ for every $v \in \vertices$. \label{asp:upperbound_norm}
\end{enumerate}
The set of assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm} are satisfied when the mirror maps $\Phi^v$ are selected to be neg-entropy or the Euclidean mirror map for any $v \in \vertices$ (see Appendix~\ref{appendix:cn_properties_mp}). Table~\ref{tab:cn_constants} provides the constants for which the assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm} are satisfied for the neg-entropy and Euclidean mirror maps.
\begin{table}[t]
\[
\begin{array}{l|llllll}
\toprule
\text{Mirror map } \Phi^v(\x^v) & \theta^v & d^v(\,\cdot\,) & d^{*v}(\,\cdot\,) & L^v_{\max} & D^v_{\max} & M^v \\
\hline
\frac{1}{2} \norm{\x^v}^2_2 & 1 & \norm{\,\cdot\,}_2 & \norm{\,\cdot\,}_2 & R \max\{\sum^{|\vec\path|-1}_{k=k_{\vec\path} (v)} w_{(p_k, p_{k+1})}: \vec\path \in \pathSet\} & k/2 (1 - k/N)& \sqrt{N}\\
\sum_{i \in \catalog} x^v_i \log(x^v_i) & 1/k^v & \norm{\,\cdot\,}_1 & \norm{\,\cdot\,}_{\infty} & R \max\{\sum^{|\vec\path|-1}_{k=k_{\vec\path} (v)} w_{(p_k, p_{k+1})}: \vec\path \in \pathSet\}& k^v \log(N/k^v) & 1\\
\bottomrule
\end{array}
\]
 \caption{The constants for which  the neg-entropy and Euclidean mirror maps satisfy assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm} in Sec.~\ref{sec:cn_regret_analysis}.}
 \label{tab:cn_constants}
\end{table}



The following theorem establishes an upper bound on the regret of \AlgoName{} for fractional caching networks.
\begin{theorem}
When the local policy \LocalAlgoName{} in Algorithm~\ref{algo:cn_online_mirror_ascent} at every node $v \in \vertices$ is configured with the mirror map $\Phi^v$ (satisfying assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm}) and learning rate $\eta^v = \frac{1}{L^v_{\max}} \sqrt{\frac{2 \theta^v D^v_{\max}}{T}}$, the regret~\eqref{eq:cn_fractional_regret} satisfies:
\begin{align}
       \mathrm{Regret}_{T, \statesSetFrac}(\mathrm{OMA}_{\Phi^{\vertices}}) \leq \left(\sum_{v \in \vertices} L^v_{\max} \sqrt{\frac{2 D^v_{\max}}{\theta^v} }\right) \sqrt{T}\label{eq:cn_regret_bound},
\end{align}
\label{theorem:cn_regret_fractional}
\end{theorem}
The proof is given in Appendix~\ref{proof:cn_regret_fractional}.



We also provide in the following theorem an upper bound on the extended regret of \AlgoName{} for fractional caching networks.
% By selecting the learning rate $\eta^v =\sqrt{\frac{D^v_{\max} \theta^v}{\left( L^v_{\max}/2 + M^v w'^v_{\max}\right) L^v_{\max} T} }$ for every $v \in \vertices$ that gives the tightest upper bound, we finally get
% \begin{align}
%         \widehat{\text{Regret}}_{T, \statesSetFrac}(\mathcal{A})  \leq  \left( \sum_{v \in \vertices} L^v_{\max}\sqrt{\frac{2D^v_{\max} \left( 1 + 2 M^v w'^v_{\max} / L^v_{\max} \right) }{\theta^v}}\right) \sqrt{T}.
 \begin{theorem}
 When the local policy \LocalAlgoName{} in Algorithm~\ref{algo:cn_online_mirror_ascent} at every node $v \in \vertices$ is configured with the mirror map $\Phi^v$ (satisfying assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm}) and learning rate $\eta^v = \sqrt{\frac{D^v_{\max} \theta^v}{\left( L^v_{\max}/2 + M^v w'^v_{\max}\right) L^v_{\max} T}}$, the extended regret~\eqref{eq:cn_fractional_regret} satisfies:
 \begin{align}
     \widehat{\text{Regret}}_{T, \statesSetFrac}(\mathrm{OMA}_{\Phi^{\vertices}})  \leq  \left( \sum_{v \in \vertices} L^v_{\max}\sqrt{\frac{2D^v_{\max} \left( 1 + 2 M^v w'^v_{\max} / L^v_{\max} \right) }{\theta^v}}\right) \sqrt{T}.
 \end{align}
 \label{theorem:cn_extended_fractional_regret}
 \end{theorem}
 The proof is provided in Appendix~\ref{proof:cn_extended_fractional_regret}.
 \subsection{Offline Problem}
 \label{sec:cn_offline_problem}
  The static caching network allocation problem can be formulated as finding the caching network state $\vec x^* \in \statesSetFrac$ that maximizes the time-averaged gain  over the time horizon $T$, i.e., 
\begin{align}
  \vec x_*  \in \underset{\vec x \in \statesSetFrac}{\arg\max}\left( G_{T}(\x) \triangleq \frac{1}{T} \sum^T_{t=1} G_{\vec r_t}( \vec x)\right).
  \label{eq:cn_static_gain_fractional}
\end{align}


 We show in the following theorem that \AlgoName{} can be used a numerical solver for the offline problem when considering the subgradients (line 5 in Algorithm~\ref{algo:cn_online_mirror_ascent}) are taken from the fixed gain function $G_T$ in Eq.~\eqref{eq:cn_static_gain_fractional}. 
 \begin{theorem}
  Let $\bar \x$ be the average fractional caching network state $\bar \x \triangleq \frac{1}{K} \sum^K_{k=1} \x_i $ obtained by running \LocalAlgoName{} at every node $v \in \vertices$ (satisfying assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm}) for $K$ iterations, where $\x_k$ is the fractional state obtained at iteration $k$. When the   subgradients (line 5 in Algorithm~\ref{algo:cn_online_mirror_ascent}) are computed from  the fixed gain function $G_T$ in Eq.~\eqref{eq:cn_static_gain_fractional}, then by selecting the learning rates $\eta^v$ at every node $v \in \vertices$, the gain of $\bar \x$ satisfies:
      \begin{align}
    G_T(\bar\x)   \geq  G_T(\x_*)  - \left(\sum_{v \in \vertices} L^v_{\max} \sqrt{\frac{2 D^v_{\max}}{\theta^v} }\right) \frac{1}{\sqrt{K}}.
  \end{align}
  \label{theorem:cn_fractional_offline_problem}
 \end{theorem}
 The proof is provided in Appendix~\ref{proof:cn_fractional_offline_problem}.
 
\section{Integral Caching Networks}
\label{s:fractional_marginal}
In this section, we turn our attention to the scenario of integral caching networks where caching states can no longer be fractional, and files must be stored in their entirety. In  Proposition~\ref{proposition:deterministic_worst_case_regret}, we showed that any deterministic policy that operates over integral caching decisions have worst case regret, so we are only interested in randomized policies in this section. We denote by $\z^v_t$ the random integral caching state of node $v \in \vertices$ in the set of valid integral caching states given by 
\begin{align}
    \statesSetInt^v \triangleq \statesSetFrac^v \cap \{0,1\}^\catalog.
\end{align}
Naturally, we can also define the random integral caching network state at time slot $t$ as $\vec z = [z^v_i]_{(i,v) \in \catalog \times \vertices}$ in the set $\statesSetInt \triangleq \bigtimes_{v \in \vertices} \statesSetInt^v$. 

The random state  $\vec z^v_t$ of a cache node $v\in \vertices$ can be fully described by a distribution $p^v_t$ with support $\statesSetInt^v$, but it is unfeasible in practice to keep track of a distribution that is exponential in size $|\statesSetInt^v| = {N\choose k^v}$. We instead restrict ourselves to work with the first moment of such distribution given as $\x^v_t = \mathbb{E} [\z^v_t]$, where $x^v_{t,i}$ is the marginal probability that file $i \in \catalog$ is stored at cache node $v \in \vertices$ during timeslot $t$.

In Proposition~\ref{p:cn_moments}, we show that by restricting a policy to maintain only the first moment representation of the random cache states, although we lose a great amount of information about the original distribution, we can reconstruct a distribution $\tilde{p}^v_t$ with support $\tilde{\statesSetInt}^v \subset \statesSetInt$ that is  polynomial in size $|\tilde{\statesSetInt}^v|\leq N$; moreover, the cache states sampled from the new distribution $\tilde{p}^v_t$ yield the same expected caching gain as the cache states sampled from the original distribution $p^v_t$ as long as they are sampled independently for the different nodes $v \in \vertices$.


\noindent\textbf{Online Integral Caching Networks Algorithms and Regret.} 
Since the offline problem is NP-Hard, then the regret of an online policy $\mathcal{A}$ is measured as the gain loss in comparison to the best static allocation in hindsight discounted by a factor $\psi = 1 - \frac{1}{e}$. The regret against an $\psi$-approximation of the static optimum is denoted by $\psi$-regret~\cite{krause2014submodular}, and formally defined as 
\begin{align}
\psi\text{-Regret}_{T, \statesSetInt}(\mathcal{A}) = \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{B}^T}{\sup} \left\{ \psi\sum^T_{t=1} G_{\vec r_t}(\vec{z}_*)- \mathbb{E} \left[\sum^T_{t=1} G_{\vec{r}_t}(\vec{z}_t) \right]\right\}, 
\label{eq:cn_regret}
\end{align}
where the expectation is taken over the random cache states $\vec z_t$; moreover, we can extend the regret definition to account  for the update cost~\eqref{eq:cn_update_cost}, so we define the extended regret as
\begin{align}
    \psi\text{-}\widehat{\text{Regret}}_{T, \statesSetInt}(\mathcal{A}) = \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{B}^T}{\sup} \left\{ \sum^T_{t=1} G_{\vec r_t}(\z_*)- \mathbb{E} \left[\sum^T_{t=1} G_{\vec{r}_t}(\z_t)  - \sum^T_{t=1} \sum_{v \in \vertices} \updatecost^v(\z^v_t, \z^v_{t+1})\right]\right\}.
    \label{eq:cn_psi_regret_extended}
\end{align}

\subsection{Regret Guarantees Transfer}
In this section, we show that the regret of any fractional caching network policy $\mathcal{A}$ with fractional states $\{\x_t\}^T_{t=1}$ can be transferred to the integral setting when the integral caching states are generated by \CoupledRounding{} with fractional caching state input $\x^v_t$ and random variable $\xi^v$  for every node $v \in \vertices$ and timeslot $t \in [T]$.
\begin{theorem}
\label{theorem:regret_generic_policy}
When  the random integral caching states $\z^v_t$ are  generated by \CoupledRounding{} with the fractional cache state input $\x^v_t$ for every $v\in\vertices$ and $t\in[T]$, then the $\psi$-regret guarantee over the random integral caching states satisfies:
\begin{align}
        \psi\mathrm{-Regret}_{T, \statesSetInt}(\mathcal{A})  \leq \psi \cdot   \mathrm{Regret}_{T, \statesSetFrac}(\mathcal{A}).
\end{align}
\end{theorem}
The proof is provided in Appendix~\ref{proof:regret_generic_policy}.

We provide the upper bound of the extended regret of \AlgoName{} for integral caching networks  in the following theorem.

\begin{theorem}
\label{theorem:cn_extended_psi_regret}
 When  the random integral caching states $\z^v_t$ are  generated by \CoupledRounding{} with the fractional cache state input $\x^v_t$, and the local policy \LocalAlgoName{} in Algorithm~\ref{algo:cn_online_mirror_ascent} is configured with the mirror map $\Phi^v$ (satisfying assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm}) and learning rate $\eta^v = \sqrt{\frac{2 D^v_{\max} \theta^v}{ \left( L^v_{\max} +2 kNM^v w'^v_{\max} / L^v_{\max} \right) L^v_{\max} T} }$ for every $v \in \vertices$ and $t \in [T]$, then the regret~\eqref{eq:cn_fractional_regret} satisfies:
 \begin{align}
     \widehat{\text{Regret}}_{T, \statesSetFrac}(\mathcal{A})  \leq  \left( \sum_{v \in \vertices} L^v_{\max}\sqrt{\frac{2D^v_{\max} \left( 1 + 2 kN M^v w'^v_{\max} / L^v_{\max} \right) }{\theta^v}}\right) \sqrt{T}.
 \end{align}
\end{theorem}
The proof is provided in Appendix~\ref{proof:cn_extended_psi_regret}.
\subsection{Offline Problem}
As in Sec.~\ref{sec:cn_offline_problem}, we seek $\vec z^* \in \statesSetInt$ that maximizes the aggregate gain~\eqref{eq:cn_static_gain_fractional} over the time horizon $T$, i.e., 
\begin{align}
  \vec z_*  \in \underset{\vec z \in \statesSetInt}{\arg\max}\,\, G_{T}(\z).
  \label{eq:cn_static_gain_integral}
\end{align}
In this integral setting  determining the best static allocation $\z_*$ is NP-Hard, and the problem admits at best a $1-\frac{1}{e}$ approximation in polynomial time~\cite{ioannidis2016adaptive}. We show in Corollary~\ref{corollary:cn_integral_offline_problem} that we can also use \AlgoName{} as a numerical solver to find a $1-\frac{1}{e}-\epsilon$ approximation of the static optimum in \BigO{\frac{1}{\epsilon^2}} iterations. 
\begin{corollary}
  Let $\bar \x$ be the average fractional caching network state $\bar \x \triangleq \frac{1}{K} \sum^K_{k=1} \x_k $ obtained by running \LocalAlgoName{} at every node $v \in \vertices$ (satisfying assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm}) for $K$ iterations, where $\x_k$ is the fractional state obtained at iteration $k$. When the   subgradients (line 5 in Algorithm~\ref{algo:cn_online_mirror_ascent}) are computed from  the fixed gain function $G_T$ in Eq.~\eqref{eq:cn_static_gain_fractional}, then by selecting the learning rates $\eta^v$ at every node $v \in \vertices$, the gain of $\bar \z$ sampled using \CoupledRounding{} with input $\bar \x$ satisfies:
      \begin{align}
    \mathbb{E}\left[G_T(\bar\z) \right]   \geq \psi G_T(\z_*)  - \psi \left(\sum_{v \in \vertices} L^v_{\max} \sqrt{\frac{2 D^v_{\max}}{\theta^v} }\right) \frac{1}{\sqrt{K}}.
  \end{align}
  \label{corollary:cn_integral_offline_problem}
 \end{corollary}
 The proof is provided in Appendix~\ref{proof:cn_integral_offline_problem}.






==> backups__zipped_project_/0._Symbols_Def.tex <==
\usepackage{mathtools}
\usepackage{eqparbox}
\usepackage{optidef}
\usepackage{appendix}
\usepackage{etoolbox,xspace}

\BeforeBeginEnvironment{appendices}{\clearpage}



% Operators

\newcommand{\CoupledRounding}{\textsc{Online Coupled Rounding}}
\newcommand{\OptTransport}{\textsc{Optimal Transport LP}}
\newcommand{\OMDNEG}{$\OMD_\negent$}
\newcommand{\conv}[1]{\mathrm{conv}\left(#1\right)}
\newcommand\vGroup[2]{\underset{#2}{\underbrace{#1} } }
\newcommand{\deriv}[2]{	\frac{\partial #1}{\partial #2}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcolumntype{C}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcommand{\card}[1]{\left|#1\right|}
\newcommand{\given}{\;\middle\vert\;}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\BigO}[1]{\ensuremath{\operatorname{\mathcal O}\left(#1\right)}}
\newcommand{\BigOmega}[1]{\ensuremath{\operatorname{\Omega}\left(#1\right)}}

\newcommand{\commentAlg}[1]{\textit{\small{#1}}}
\newcommand{\commentAlgspaced}[1]{\tabto {5cm}\textit{\small{#1}}}
\newcommand{\commentAlgspacedcm}[1]{\tabto {.5cm}\textit{\small{#1}}}
\newcommand{\commentAlgspacedccm}[1]{\tabto {1cm}\textit{\small{#1}}}
\newcommand{\argmin}{\mathop{\arg\min}}
\newcommand{\old}[1]{\textbf{\textcolor{red}{#1}}}
\newcommand{\new}[1]{\textbf{\textcolor{blue}{#1}}}
\newcommand{\why}[1]{\textbf{\textcolor{orange}{#1}}}
\newcommand{\fix}[1]{\textbf{\textcolor{red}{#1}}}
\newcommand{\Regret}{\ensuremath{\mathrm{Regret}}}
\newcommand{\OMD}{\ensuremath{\mathrm{OMD}}}
\newcommand{\OGD}{\ensuremath{\mathrm{OGD}}}
\newcommand{\nrm}{\ensuremath{\text{-}\mathrm{norm}}}
\newcommand{\negent}{\ensuremath{\mathrm{NE}}}
\newcommand{\updatecost}{\ensuremath{\mathrm{UC}}}
\newcommand{\supp}{\mathop{\ensuremath{\mathrm{supp}}}}
\renewcommand{\vec}[1]{\bm{\mathbf{#1}}}




% Symbols
\renewcommand{\vec}[1]{\pmb{#1}}
\newcommand{\statesSetFrac}{\mathcal{X}}
\newcommand{\statesSetInt}{\mathcal{Z}}
\newcommand{\naturals}{\mathbb N}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\capacity} {k}
\newcommand{\catalogSize}{N}
\newcommand{\timeHorizon}{T}
\newcommand{\catalog}{\mathcal{N}}
\newcommand{\x}{\vec{x}}
\newcommand{\y}{\vec{y}}
\newcommand{\z}{\vec{z}}
\newcommand{\requestSet}{\mathcal{R}}
\newcommand{\fractionalState}{x}
\newcommand{\randomState}{z}
\newcommand{\integralState}{\zeta}
\newcommand{\maxRequests}{R}
\newcommand{\maxMultiplicity}{h}
\newcommand{\learningrate}{\eta}
\newcommand{\updateCostWeight}{w}
\newcommand{\projectSymbol}{\Pi}
\newcommand{\request}{r}
\newcommand{\policy}{\mathcal{A}}
\newcommand{\domainMirrorMap}{\mathcal{D}}
\newcommand{\roundingScheme}{\Xi}
\newcommand{\couplingRandomVariable}{\xi}

\newcommand{\Rounding}{\textsc{Online Rounding}\xspace}









==> backups__zipped_project_/1._Abstract.tex <==
\begin{abstract}
We study an online caching problem in which requests can be served by a local cache to avoid retrieval costs from a remote server. The cache can update its state after a batch of requests and store an arbitrarily small fraction of each content. We study no-regret algorithms based on Online Mirror Descent (OMD) strategies. We show that the optimal OMD strategy depends on the request diversity present in a batch. We also prove that, when the cache must store the entire content, rather than a fraction, OMD strategies can be coupled with a randomized rounding scheme that preserves regret guarantees.
\end{abstract}

==> backups__zipped_project_/1._Introduction.tex <==
\section{Introduction}
Caches are deployed at many different levels in computer systems: from CPU hardware caches to operating system memory caches, from application caches at clients to CDN caches deployed as physical servers in the network or as cloud services like Amazon's ElastiCache~\cite{amazonElastiCache}. They aim to provide a faster service to the user and/or to reduce the computation/communication load on other system elements, like hard disks, content servers, etc.

The ubiquity of caches has motivated extensive research on the performance of existing caching policies, as well as on the design of new policies with provable guarantees. To that end, most prior work has assumed that caches serve requests generated according to a stochastic process, ranging from the simple, memory-less independent reference model~\cite{coffman1973operating}  to more complex models trying to capture temporal locality effects and time-varying popularities (e.g., the shot-noise model~\cite{traverso13}).
%
An alternative modeling approach is to consider an \emph{adversarial} setting. Assuming that the sequence of requests is generated by an adversary, an online caching policy can be compared to the optimal offline policy that  views the sequence of requests in advance. 
Caching was indeed one of the first problems studied by Sleator and Tarjan in the context of the  competitive analysis of online algorithms~\cite{sleator85}.  In competitive analysis, the metric of interest is the \emph{competitive ratio}, i.e., the worst-case ratio between the costs incurred by the online algorithm  and the  optimal offline \emph{dynamic} algorithm. 
This line of work led to the study of metrical task systems~\cite{borodin92}, a popular research area in the algorithms community~\cite{koutsoupias09}. 

Recently, Paschos et al.~\cite{PaschosLearningToCache}  proposed studying caching  as an online convex optimization (OCO) problem~\cite{Hazanoco2016}. OCO considers again an adversarial setting, but the metric of interest is the \emph{regret}, i.e., the difference between the costs incurred over a time horizon $T$ by the algorithm and by the optimal offline \emph{static} solution. Online algorithms whose regret grows sublinearly with  $T$ are called \emph{no-regret} algorithms, as their time-average regret becomes negligible for large $T$.
% \new{; although in practice, classifying sublinear regret policies as good policies must be  made ``within reason'', since the constants appearing in the regret are of importance when targeting performance guarantees for a finite horizon $T$, e.g., applying naively learning from expert advice~\cite{Hazanoco2016} over the exponentially sized universe of cache configurations (each configuration is an expert) yields directly a sublinear regret policy, but with large regret constants, which makes it futile for finite horizons.}
Paschos et al.~proposed a no-regret caching policy based on the classic online gradient descent method ($\OGD$),  
under the assumption that (a) the cache can store arbitrarily small fractions of each content (the so-called fractional setting), and (b) the cache state is updated after each request.

In this paper, we extend and generalize the analysis of Paschos et al.~in three different directions:
\begin{enumerate}
    \item We assume the cache can update its state after  processing a batch of $R \ge 1$ requests. This is of interest both in high-demand settings, as well as in cases when updates are infrequent, because they are costly w.r.t.~either computation or communication.  %This is a  it may happen when updates are particularly costly in terms of computation or communication; 
    \item We consider a broad family of caching policies based on online mirror descent ($\OMD$); $\OGD$ can be seen as  a special instance of this family. 
    \item We also depart from the fractional setting, extending our analysis to the case when the cache can only store entire files (the integral setting).
\end{enumerate}

Our contributions are summarized as follows.
First, we show that  caching policies based on $\OMD$ enjoy $\BigO{\sqrt T}$ regret in the fractional setting. Most importantly, we show that  bounds for the regret crucially depend on the diversity of the request process. In particular, the regret depends on the \emph{diversity ratio} $R/h$, where $R$ is the size of the batch, and $h$ is the maximum multiplicity of a request in a given batch.
%
Second, we characterize the optimality of OMD caching policies w.r.t.  regret under different diversity regimes. %and different cache sizes (normalized with respect to the catalog size). 
We observe that, for a large region of possible values of the diversity ratio, the optimum is either $\OGD$ or $\OMD$ with a neg-entropy mirror map ($\OMD_{\negent}$). In particular, $\OGD$ is optimal in the \emph{low diversity} regime, while $\OMD_{\negent}$ is optimal in the \emph{high diversity} regime. 
%
Third, $\OMD$ algorithms include a gradient update followed by a projection to guarantee that the new solution is in the feasible set (e.g.,  it does not violate the cache capacity constraints). The projection is often the most computationally expensive step of the algorithm. We show that efficient polynomial algorithms exist both for $\OGD$ (slightly improving the algorithm in~\cite{PaschosLearningToCache}) and for $\OMD_{\negent}$.
%
Finally, $\OMD$ algorithms work in a continuous space, and are therefore well-suited for the fractional setting originally studied by Paschos et al.  Still, we show that, if coupled with opportune rounding techniques, they can also be used when the cache can only store a content in its entirety, while preserving their regret guarantees.

The remainder of this paper is organized as follows. After an overview of the related work in Sec.~\ref{sec:related}, we introduce our model assumptions in Sec.~\ref{s:system} and provide  technical background on gradient algorithms in Sec.~\ref{sec:grad}. Section~\ref{sec:OMDanalysis} presents our main results on the regret of $\OMD$ caching policies and their computational complexity. A discussion about extending the model to include cache update costs, in Sec.~\ref{sec:movement}, is required to introduce the integral setting in Sec.~\ref{sec:rounding}.
Finally, numerical results are presented in Sec.~\ref{sec:experiments}.


==> backups__zipped_project_/2._Related_Work.tex <==
\section{Related work}
\label{sec:related}
% Classical caching and what is done up to now.

The caching problem has been extensively studied in the literature under different assumptions on the request process.  When the requests occur according to a given stochastic process, 
the analysis leads usually to complex formulas even in simple settings. For example, even the hit ratio of a single cache managed by the LRU eviction policy under the  independent reference model %(at any time a request is for file $i$ with probability $p_i$ independently from the past), and the metric of interest is the miss ratio
is hard to precisely characterize~\cite{king72,flajolet92}.
 The characteristic time approximation (often referred to as Che's approximation)  significantly simplifies this analysis by assuming that a file, in absence of additional requests for it, stays in the cache for a random time %$\tau$
 sampled independently from requests for other files. %(but the distribution of $\tau$ depends on the request process). 
 %To the best of our knowledge, it was 
 First proposed by Fagin~\cite{fagin77} and later rediscovered and popularized by~Che et al
~\cite{che02}, the approximation has been justified formally by several works ~\cite{Jele99,fricker2012,jiang18}
%The characteristic time approximation 
and has allowed the study of a large number of existing~\cite{garetto16} and new~\cite{gast2017ttl,leonardi18jsac} caching policies. It also applies to   networked settings~\cite{choungmo14,berger2014exact,alouf2016performance,chu18}
%In particular, new caching policies have been designed to optimize 
and to  more general utilities beyond the hit ratio~\cite{dehghan19,neglia18ton}, all under  stochastic requests. 

Online caching policies based on gradient methods have also been studied in the stochastic request setting, leading to Robbins-Monro/stochastic approximation algorithms (see, e.g., \cite{ioannidis2010distributed,ioannidis2016adaptive}). Though related to OCO, guarantees are very different than the regret metric we study here.
 %
 Many works have also explored the offline, network-wide static allocation of contents, presuming demand is known~\cite{borst2010distributed,shanmugam13,poularakis2016exploiting}.
%
We differ from the work above, as we consider adversarial requests.

%%%%%%%%%%% Adversarial, compare to dynamic optimum 
Caching under adversarial requests has been studied since Sleator and Tarjan's seminal paper~\cite{sleator85} through the competitive ratio metric. An algorithm is said to be $\alpha$-competitive when its competitive ratio is bounded by $\alpha$ over all possible input sequences. The problem has been generalized by Manasse et al.~\cite{manasse88}~under the name \emph{$k$-server problem}, and further generalized  by Borodin et al.~under the name \emph{metrical task systems (MTS)}~\cite{borodin92}. The literature on both the $k$-server and MTS problems is vast.
A recent trend is to apply continuous optimization techniques to solve these combinatorial problems. Bansal et al.~\cite{bansal12}  study the $k$-server problem on a weighted star metric space. In the same spirit, Bubeck et al.~\cite{bubeck_kserver_2018} use the framework of continuous online mirror descent to provide an $o(k)$-competitive algorithm for the $k$-server problem on  hierarchically separated trees. 
% \new{The competitive ratio approach is well understood for paging, and it is considered practically too pessimistic to provide a good classification of policies---e.g., LRU and any marking policy have the highest competitive ratio ~\cite{borodin2005online,PaschosLearningToCache}.} 
In this paper, we focus on regret rather than competitive ratio as main performance metric.
%
Andrew et al.~\cite{taleoftwometrics} give a formal comparison between competitive ratio and regret and 
%competitive analysis and  OCO/no-regret algorithms.  
prove that there is an intrinsic incompatibility between the two: no algorithm can have both sub-linear regret and a constant competitive ratio. At the same time, they propose an algorithm with sub-linear regret and slowly increasing competitive ratio.

Online convex optimization (OCO)  was first proposed by Zinkevich~\cite{Zinkevich2003}, who showed that projected gradient descent attains sublinear regret bounds in the online setting. OCO generalizes previous online problems like the experts problem ~\cite{littlestone94}, and has become widely influential in the learning community~\cite{Hazanoco2016, ShalevOnlineLearning}.  
To the best of our knowledge, Paschos et al.~\cite{PaschosLearningToCache} were the first to apply the OCO framework to caching. Beside proposing OGD for the single cache, they extended it to a simple networked scenario, where users have access to a set of parallel caches that store pseudo-random linear combinations of the files.  They proposed  no-regret algorithms in both settings. Bhattacharjee et al.~ \cite{FundamentalLimits} extended this work proving tighter lower bounds for the regret and proposing new caching policies for the networked setting that do not require content coding;  Mukhopadhyay and Sinha~\cite{mukhopadhyay2021online} accounted for switching costs due to file retrievals. We depart from these works in considering OMD algorithms, a more general request process, and allowing for integral cache states obtained through randomized rounding.





==> backups__zipped_project_/3._System_Description.tex <==
\section{System description}
\label{s:system}
\begin{table}[t!]

  \caption{{Notation Summary } }
  \vspace{-1em}
\begin{center}
    \begin{tabular}{C{.17\textwidth}C{.50\textwidth}}
    \hline
    \hline
    &\textbf{Notational Conventions} \\
    \hline  
    $[n]$& Set of integers $\{1,2, \dots, n\}$ \\
    \hline
    &\textbf{Caching } \\
    \hline  
    $\mathcal{N}$ & Catalog set with size $\card{\catalog} = N$\\
    $k$ & Cache capacity\\
	$\mathcal{X}$ & Set of fractional cache states \\ 
	$\mathcal{X}_\delta = \mathcal{X} \cap [\delta, 1]^N$ & The $\delta$-interior of $\mathcal{X}$ \\
	$\mathcal{Z} =  \mathcal{X} \cap \{0,1\}^N$ & Set of integral cache states\\
	$\vec{x}_t$ & Fractional cache state at timeslot $t$ in $\mathcal{X}$ \\
	$\vec \zeta_t$ & Integral cache state at timeslot $t$ in $\mathcal{Z}$\\
	$\vec z_t$ & Random integral cache state at timeslot $t$ in $\mathcal{Z}$\\
	$\vec{x}_*$ & Optimal cache allocation in hindsight in $\mathcal{X}$\\
	$R$ & The number of files' requests in a batch\\
	$h$ & The maximum multiplicity of any file in a batch of request \\
	$\mathcal{R}_{R,h}$ & Set of possible adversarial requests \\
	$\vec{r}_t$ & Batch of request arriving at timeslot $t$ in $\mathcal{R}$ \\ 
	$f_{\vec{r}_t}$ & Cost received at timeslot $t$ \\
	$\updatecost_{\vec{r}_t}$ & Update cost of the cache when $\vec{r}_t$ is received at timeslot $t$ \\
	$\vec{w}$ / $\vec{w}'$  & Service / update costs in $\mathbb{R}_+^N$, $w_i$ / $w_i'$ is the cost for file $i$\\
	\hline  
    &\textbf{Online Learning } \\
    \hline  
    $T$ & The time horizon \\
    $\eta$ & Learning rate \\
    $\updatecost_{\vec{r}_t} (\vec{x}_{t}, \vec{x}_{t+1} ) $ & Update cost at timeslot $t$ \\
	Regret$_T(\mathcal{A})$ & Regret of policy $\mathcal{A}$ over $T$\\
	$\mathrm{E\mbox{-}Regret}_T(\mathcal{A}, \Xi) $ & Extended regret of policy $\mathcal{A}$ over $T$ \\ 
	$\Phi(\vec{x})$ & Mirror map with domain $\mathcal{D}$ and co-domain $\mathbb{R}$ \\
	$D_\Phi(\vec{x},\vec{y})$ & Bregman divergence between $\vec{x}$ and $\vec{y}$ associated to the map $\Phi$\\ 
	$\Pi^{\Phi}_\mathcal{B}(\vec{y})$ & The projection of $\vec{y}$ onto $\mathcal{B}$ under the Bregman divergence associated to $\Phi$\\
  \hline
  \hline
  
\end{tabular}
\end{center}
\end{table}
\noindent\textbf{Remote Service and Local Cache.} We consider a system in which requests for files are served either remotely or by an intermediate cache of finite capacity. A cache miss incurs a file-dependent remote retrieval cost. Our goal is to study online caching algorithms that attain sublinear regret. Formally, we consider a stream of requests for files of equal size from a catalog $\mathcal{N}=\{1,2,\dots, N\}$.  These requests can be served by a remote server at cost $w_i \in \mathbb{R}_+$  per request for file $i\in\mathcal{N}$. This cost could be, e.g., an actual monetary cost for using the network infrastructure, or a quality of service cost incurred  due to fetching latency. Costs may  vary across files, as each file may be stored at a different remote location. We denote by %The cost of serving these files is summarized by a cost weight 
$\vec{w}=[w_i]_{i \in \mathcal{N}}\in \mathbb{R}_+^N$ the vector of costs %where $w_i \in \mathbb{R}_+$ is the cost of serving  file $i \in \mathcal{N}$. We assume that weights 
and assume that $\vec{w}$ is known.

 A local cache of finite capacity is placed in between the source of requests and the remote server(s). The local cache's role is to reduce the costs incurred by satisfying requests locally. We denote by $k \in \{1,2,\dots,N\}$ the capacity of the cache. The cache is allowed to store fractions of files (this assumption will be removed in Sec.~\ref{sec:rounding}).  We assume that time is slotted, and  denote by $x_{t,i}\in[0,1]$  the fraction of file $i \in \mathcal{N}$ stored in the cache at  timeslot $t \in \{1,2,\dots,T\}$.  The cache state is then given by vector $\vec{x}_t=[x_{t,i}]_{i\in \mathcal{N}}\in \mathcal{X}$, where $\mathcal{X}$ is the capped simplex  determined by the capacity constraint, i.e.: \begin{align}\mathcal{X} = \left\{ \vec{x} \in [0,1]^N : \sum^N_{i=1} x_i = k \right\}.\end{align}

\noindent\textbf{Requests.} We assume that a batch of multiple requests may arrive within a single timeslot. Moreover, a file may be requested multiple times (e.g., by different users, whose aggregated requests form the stream reaching the cache) within a single timeslot. We denote by $r_{t,i} \in \mathbb{N}$  the number of requests---also called multiplicity---for file $i \in \mathcal{N}$ at time $t$, and by $\vec{r}_t=[r_{t,i}]_{i\in\mathcal{N}} \in \mathbb{N}^N$ the vector of such requests, representing the entire batch. We assume that the number of requests (i.e., the batch size) at each timeslot is given by $R \in \mathbb{N}$. We also assume that  the maximum multiplicity of a file in a batch is bounded  by $h \in \mathbb{N}$. As a result, $\vec{r}_t$ belongs to set: 
\begin{align}\mathcal{R}_{R,h} = \left\{\vec{r} \in \{0,\dots, h\}^N : \sum^N_{i=1} r_i = R \right\}.\end{align}

Intuitively, the ratio $\frac{R}{h}$ defines the diversity of request batches in a timeslot. For example, when $\frac{R}{h} = 1$, requests are concentrated on a single content. When $\frac{R}{h} = N$, requests are spread evenly across the catalog $\mathcal{N}$. In general, $\frac{R}{h}$ is a lower bound for the number of distinct files requested in the batch. For that reason, we refer to $\frac{R}{h}$ as the \emph{diversity ratio.} This definition of diversity is consistent with other notions of diversity, such as, e.g., the entropy; indeed the diversity ratio provides a lower bound on the entropy of the normalized batch vector $\frac{\vec{r}_t}{R}$, %\in \Delta_N$,
as $E\left(\frac{\vec{r}_t}{R}\right) \geq \log\left(\frac{R}{h}\right)$ \cite[Lemma 3]{lin2013diversity},
where $E(\vec p) = -\sum_i p_i \log(p_i)$ is the entropy function. %Nevertheless, we adopt $\frac{R}{h}$ as a measure of diversity as, as we will see, it better characterizes system performance (see Thms.~\ref{xxx}-\ref{yyy}). 
%
We note that our request model
generalizes the setting  by Paschos et al. ~\cite{PaschosLearningToCache}, which can be seen as the case $R = h = 1$ under our request model. 
We make no additional assumptions on the request arrival process; put differently, we operate in the adversarial online setting, where a potential adversary may select an arbitrary request sequence in $\mathcal{R}_{R,h}$ to increase system costs.

\noindent\textbf{Service Cost Objective.} When a request batch  $\vec{r}_t$ arrives, the cache incurs the following cost:
\begin{align}
\label{e:cost}
f_{\vec{r}_t}(\vec{x}_t) = \sum^N_{i=1} w_i r_{t,i}(1 - x_{t,i}).\end{align}
In other words, for each file $i\in\mathcal{N}$, the system pays a cost proportional to the file fraction $(1-x_{t,i})$ missing from the local cache, weighted by the file cost $w_i$ and by the number of times $r_{t,i}$ file~$i$ is requested in the current batch $\vec{r}_t$.


The cost objective \eqref{e:cost} captures several possible real-life settings. First, it can be interpreted as a QoS cost paid by each user for the additional delay to retrieve part of the file from the server.  Second, assuming that the $R$ requests arrive and are served individually (e.g., because they are spread-out within a timeslot),  Eq.~\eqref{e:cost} can represent the load on  the servers or on the network to provide the missing part of the requested files.
Our model also applies when all requests for the same file are aggregated and served simultaneously  by a single fetch operation. In this case, $r_{t_i}$ in Eq.~\eqref{e:cost} should be the interpreted as the indicator variable denoting if file $i$ was requested; correspondingly, $R$ then indicates the total number of distinct files requested, and $h=1$.

\noindent\textbf{Online Caching Algorithms and Regret.} Cache content is determined online as follows. %: that is,
The cache has selected a state $\vec{x}_t \in \mathcal{X}$ at the beginning of a timeslot.  The request batch $\vec{r}_t$ arrives, and the linear cost $f_{\vec{r}_t}(\vec{x}_t) : \mathcal{X} \to \mathbb{R}_+$ is incurred; the state is subsequently updated to $\vec{x}_{t+1}$. Formally, the  cache state is determined by an online policy $\mathcal{A}$, i.e.,  a sequence of mappings  $\{\mathcal{A}_t\}^{T-1}_{t=1}$, where for every $t \geq 1$, $\mathcal{A}_t : (\mathcal{R}_{R,h} \times \mathcal{X})^{t} \to \mathcal{X}$ maps the sequence of the request batches and previous decisions $\{(\vec{r}_s, \vec{x}_s)\}^{t}_{s=1}$ to the next state $\vec{x}_{t+1}\in \mathcal{X}$. We assume that the policy is initialized with a feasible state $\vec{x}_1\in \mathcal{X}$. 

 We measure the performance of an online algorithm $\mathcal{A}$ in terms of regret, i.e., the difference between the total cost experienced by a policy $\mathcal{A}$ over a time horizon $T$ and that of the best static state $\vec{x}_*$ in hindsight. Formally,
\begin{align}
\text{Regret}_T(\mathcal{A}) = \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{R}^T_{R,h}}{\sup} \left\{ \sum^T_{t=1} f_{\vec{r}_t}(\vec{x}_t)- \sum^T_{t=1} f_{\vec{r}_t}(\vec{x}_*) \right\}, 
\label{eq:regret}
\end{align}
where
$\vec{x}_*=\argmin_{\vec{x} \in \mathcal{X}}\sum^T_{t=1} f_{\vec{r}_t}(\vec{x})$ 
 is the optimal static cache state (in hindsight). 
Note that, by taking the supremum in Eq.~\eqref{eq:regret}, we indeed measure regret in the adversarial setting, i.e., against an adversary that potentially picks requests in $\mathcal{R}_{R,h}$ trying to jeopardize  cache performance.

% \old{
% {Reviewer 3: My other big concern is that the regret function itself from (4) is defined relative to a single "optimal cache state", rather than a T-dimensional one, which would express the true regret relative to the "optimal cache states".}
% {Ideally, we could compare the online policy $\mathcal{A}$ to a dynamic optimum and in this setting, we should take into account the movement costs. The competitive ratio approach is well understood for paging, and it is practically too pessimistic to provide a good classification of policies---e.g., LRU and any marking policy has the highest competitive ratio ~\cite{PaschosLearningToCache,borodin2005online}}.
% }


 %We are interested in the worst possible regret that can be incurred by $\mathcal{A}$:
%\begin{align}\text{Regret}_T(\mathcal{A}) = \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{R}^T_{R,h}}{\sup} \left\{ \sum^T_{t=1} f_{\vec{r}_t}(\vec{x}_t)-\underset{x_* \in \mathcal{X}}{\min} \sum^T_{t=1} f_{\vec{r}_t}(\vec{x}_*) \right\}. \end{align}

% \why{Reviewer 1: The negative side of the paper, in my opinion, is the lack of sufficient conceptual novelty in contrast to existing work. On the methodological end, the analysis and the algorithm involving OMD used here are standard in the learning literature. For instance, the proof of the main theorem relies on standard analysis from Bubeck's book, and the $\BigO{\sqrt{T}}$ regret is also what one typically sees in online convex optimization. }

% \new{A cache configuration lives in a universe $\mathcal{U}$, that has cardinality  $ N \choose k$. When applying naively online community results, such as the expert problem, we indeed obtain  sub-linear regret of the order $\mathcal{O}(\log(|\mathcal{U}|)T )$. This has two disadvantages: \emph{(i)} the algorithm requires an exponentially sized data structure, and \emph{(ii)} the regret bound, although sublinear, it depends on the dimension $N$, that can be very large $N \gg k$. Thus, careful attention to regret constants and practicality (time-complexity) of policies should be made. }



\noindent\textbf{Update Costs.} An online algorithm $\mathcal{A}$ updating the cache state at timeslot $t$ may require moving a portion of a file from a remote server to the cache to implement this update. The update cost of the online algorithm is  not explicitly modeled in our cost  and  regret (Eqs.~\eqref{e:cost} and~\eqref{eq:regret}, respectively).
% This happens for two reasons. 
% First, the gradient-based algorithms we consider (see Sec.~\ref{sec:grad}) adapt the state by fetching fractions of files scaled by a gain $\eta=\BigO{{1}/{\sqrt{T}}}$; hence, when the time horizon is large,    file retrievals  satisfying requests would dominate this term.
% These small costs are  be fully eliminated in practice. 
We postpone the discussion of such cost in Sec.~\ref{sec:movement}. For the moment we observe that updates come ``for free'' for files requested in the current timeslot. For example, increasing the fraction $x_{t,i}$ for some file~$i$ such that $r_{t,i}>0$, can be performed by recovering the additional part
%a small ($\BigO{\eta}$) fraction 
out of the  ($1-x_{t,i}$) missing fraction that needs to be retrieved to serve the file; updates can thus ``free-ride'' on regular traffic, at no additional cost.
%This is because updates come ``for free'' for files requested in the current timeslot. 
%For example, increasing a coordinate $x_{t,i}$ for some file $i$ such that $r_{t,i}>0$, can be performed by recovering a small ($\BigO{\eta}$) fraction out of the overall ($1-x_i$) missing part of the file at the time of its retrieval; updates can thus ``free-ride'' on regular traffic, at no additional cost. 
% As we discuss in Sec.~\ref{sec:movement}, 
We prove in Theorem~\ref{prop:free_updates} that both main algorithms studied in this paper ($\OGD$ and $\OMD_{\negent}$) are in this regime, as  \emph{they only increase current state coordinates corresponding to files requested in the previous timeslot}; as such, for both algorithms, the update costs can be considered to be zero. 
% \old{There can be cases however where update costs cannot be ignored; we revisit this issue in Secs.~\ref{sec:movement} and~\ref{sec:rounding}, where we account for update costs explicitly.} 
% \new{ The same argument, unfortunately, cannot be transferred to the setting where  the fractional states are interpreted as probabilities of storing a given file; we revisit this issue in Secs.~\ref{sec:movement} and~\ref{sec:rounding}, where we account for update costs explicitly. In what follows, we consider deterministic cache states.}



==> backups__zipped_project_/4._Fractional_Caching_-_Gradient-Based_Algorithms.tex <==
\section{Fractional Caching and  Gradient-based Algorithms}\label{sec:grad}
% Any policy that updates the cache state by deterministic evictions and insertions of files in their entirety is too weak against an adversary and has worst case regret (see Proposition~\ref{proposition:deterministic_worst_case_regret}); therefore, classical policies, such as LRU, LFU, FIFO, etc., are all rendered obsolete in this setting. This observation, suggests that policies with low regret can only emerge from policies employing  fractional caching, or  randomization. 

 
 Inspired by offline minimization, it is natural to design a policy that, upon seeing $\vec{r}_t$,  selects as $\vec{x}_{t+1}$ the state that would have minimized (on hindsight) the aggregate cost up to time $t$ (i.e., $\sum_{t'=1}^{t}f_{\vec{r}_{t'}}(\vec{x})$). Unfortunately, such policy has poor regret: 
 \begin{proposition}
\label{proposition:aggregate_cost_policy}
The aggregate cost minimization policy is a policy $\policy$ that selects for every timeslot $t \in [T-1]$ the state $\x_{t+1} = \argmin_{\x \in \statesSetFrac} \sum_{t'=1}^{t}f_{\vec{r}_{t'}}(\vec{x})$. This policy has linear (worst-case) regret, i.e.,
\begin{align}
    \Regret(\policy) = \BigOmega{T}.
\end{align}
\end{proposition}
We provide a proof in Appendix~\ref{proof:aggregate_cost_policy}. 

A more conservative approach, that indeed leads to sublinear regret, is to take gradient steps, moving in the direction of a better decision according to the latest cost; we discuss in this section algorithms of this nature that employ fractional caching.



% \subsection{Gradient-based Algorithms}

\subsection{Online Gradient Descent (OGD)}
\label{section:OGD}
In OGD, introduced by Paschos et al. \cite{PaschosLearningToCache} for  online caching, the cache  is  initialized with a feasible state $\vec{x}_1\in \mathcal{X}$ and updated as follows.  Upon receiving a request batch $\vec{r}_t$, the cost $f_{\vec{r}_t}(\vec{x}_t)$ is incurred and the next state becomes:
\begin{align} \vec{x}_{t+1} = \Pi_\mathcal{X} \left(\vec{x}_t - \eta \nabla f_{\vec{r}_t}(\vec{x}_t)\right), \quad\text{for all}~t \in [T-1],\label{eq:ogd}\end{align}
where $\Pi_\mathcal{X}(\,\cdot\,)$ is the Euclidean projection onto $\mathcal{X}$, that ensures feasibility, and $\eta\in \mathbb{R}_+$ is called the learning rate. %OGD 
%The caching decision $\vec{x}_t$ is updated by an $\eta$ movement. We take a step in the direction of the gradient $\nabla f_{\vec{r}_t} (\vec{x}_t)$ at time $t$. Since this update step could lead to an invalid caching configuration, we are required to find the closest point $\vec{x}_{t+1}$ in the decision set $\mathcal{X}$. We use the Euclidean projection to obtain a feasible point, where $\Pi_\mathcal{X}(.)$ is the Euclidean projection onto $\mathcal{X}$. 
Note that the state $\vec{x}_{t+1}$ obtained according Eq.~\eqref{eq:ogd}  is indeed a function of  $\{(\vec{r}_{t}, \vec{x}_{t})\} \subset \{(\vec{r}_{s}, \vec{x}_{s})\}^{t}_{s=1} $ for every $t \geq 1$; hence, OGD is indeed an online caching policy as defined in Sec.~\ref{s:system}. Paschos et al. \cite{PaschosLearningToCache}, show that OGD attains sub-linear regret when $R=h=1$; more specifically, the following holds: %The cache performs as well as the best fixed caching decision as $T\to \infty$, even with the presence of an adversary.
\begin{theorem}%Paschos et al.~\cite{PaschosLearningToCache}]%
\!\!\!{\protect\textrm{(\cite[Theorem 2]{PaschosLearningToCache})}}
\label{theorem:pascos_regret}
When $R = h = 1$,   the regret of OGD is bounded as follows:
\begin{equation}
    \Regret_T(\OGD) \leq \norm{\vec w}_\infty \sqrt{ \min(2k ,2(N-k)) T}.
\end{equation}
\end{theorem}
% There are different ways we could project back to the decision set besides the Euclidean projection and perhaps more efficiently, for instance, one could take advantage of the geometry of $\mathcal{X}$. Furthermore, the OGD algorithm is unaware of the sparsity of cost gradients that could be used as an advantage to take better decisions, this is why focus our attention on the class of Online Mirror Descent (OMD) strategies described in section \ref{section:OMD}.

In other words, OGD attains an $\BigO{\sqrt{T}}$ regret when $R=h=1$. In this paper, we study a broader class of gradient descent algorithms that include OGD as a special case.  As we will see below (see Thm.~\ref{theorem:optimalq_q1}), the regret attained by OGD is not necessarily the tightest possible when $R\neq 1 \neq h$; broadening the  class  of algorithms we consider  allows us to improve upon this bound. 
%In the next section, we present a generalization of the OGD Algorithm. We show that we can obtain stronger regret guarantees, with this larger space of algorithms.
\subsection{Online Mirror Descent (OMD)}
\label{section:OMD}
%The class of OMD strategies contains the OGD algorithm as a particular instance, and OMD provides a generalization and the flexibility to adapt a strategy depending on the geometry of the constraint set and the boundedness of the loss gradients,

\begin{algorithm}[!t]
	\begin{algorithmic}[1]
		\Procedure {OnlineMirrorDescent}{$\vec{x}_1 \gets \underset{\vec{x} \in \mathcal{X} \cap \mathcal{D}}{\arg\min} \,\Phi(\vec{x}) , \eta$}
		\For{$t \gets 1,2,\dots,T$}\Comment{{ Incur a cost $f_{\vec{r}_t}(\vec{x}_t)$, and receive a gradient  $  \nabla f_{\vec{r}_t}(\vec{x})$}}
		\State
		$\hat{\vec{x}}_t\gets \nabla \Phi (\vec{x}_t)$\Comment{{ Map primal point to dual point}}
		\State
		$\hat{\vec{y}}_{t+1}   \gets \hat{\vec{x}}_t - \eta \nabla f_{\vec{r}_t}(\vec{x}_t)$\Comment{{ Take gradient step in the dual}}
		\State
		$\vec{y}_{t+1}   \gets \left(\nabla \Phi\right)^{-1}(\hat{\vec{y}}_{t+1})$\Comment{{ Map dual point to a primal point}}
		\State
		$\vec{x}_{t+1}\gets \Pi_{\mathcal{X} \cap \mathcal{D}}^\Phi(\vec{y}_{t+1})$\Comment{{ Project new point onto feasible region}}
		\EndFor
		\EndProcedure
	\end{algorithmic}
	\caption{Online mirror descent ($\text{OMD}_\Phi$)}
	\label{algo:online_mirror_descent}
\end{algorithm}
OMD \cite[Sec.~5.3]{Hazanoco2016} is the online version of the mirror descent (MD) algorithm \cite{beck2003mirror} for convex optimization of a fixed, known function. The main premise behind mirror descent is that variables and gradients live into two distinct spaces: the \emph{primal space}, for variables, and the \emph{dual space}, for gradients. The two are linked via a function known as a \emph{mirror map}. Contrary to standard gradient descent, updates using the gradient occur on the dual space; the mirror map is used to invert this update to a change on the primal variables. For several constrained optimization problems of interest, mirror descent leads to faster convergence compared to gradient descent \cite[Sec. 4.3]{bubeck2015convexbook}. OMD arises by observing that MD is agnostic to whether the gradients are obtained from a \emph{fixed} function, or a sequence revealed adversarially.

\noindent\textbf{OMD for Caching.} Applied to our caching problem, OMD takes the form summarized in Algorithm~\ref{algo:online_mirror_descent}. %performs a gradient descent update, similarly to OGD. However, the decision variable is mapped to a \emph{dual space}, before performing the gradient descent step. The resulting dual point is mapped to the \emph{primal space}. Since this point can lie outside of $\mathcal{X}$, we also require a projection step. 
In our case, both the primal and dual spaces are $\mathbb{R}^N$. To disambiguate between the two, we denote primal points by $\vec{x}, \vec{y} \in \mathbb{R}^N$   and dual points by  $\hat{\vec{x}},\hat{\vec{y}} \in \mathbb{R}^N$, respectively.   Formally, OMD is parameterized by (a) a fixed learning rate $\eta\in \mathbb{R}_+$, and (b) a  differentiable map $\Phi : \mathcal{D} \to \mathbb{R}$, strictly convex over $\mathcal D$ and $\rho$-strongly convex over $\mathcal{X} \cap \mathcal{D}$, where $\mathcal{X}$ is included in the closure of $\mathcal{D}$; that is %$\mathcal{X} \subseteq \mathrm{closure}(\mathcal{D})$. 
\begin{align}\mathcal{X} \subseteq \mathrm{closure}(\mathcal{D}).\label{eq:closure} \end{align}
Function $\Phi$ is called the \emph{mirror map}, that links the primal to the dual space.  

Given $\eta$ and $\Phi$, an OMD iteration proceeds as follows. After observing  the request batch $\vec{r}_t$ and incurring the cost $f_{\vec{r}_t}(\vec{x}_t)$, the current state $\vec{x}_t$ is first mapped from the primal  to the dual space via: 
\begin{align}\label{eq:mapstep}\hat{\vec{x}}_{t} = \nabla \Phi(\vec{x}_t).\end{align} Then, a regular gradient descent step is performed \emph{in the dual space} to obtain an updated dual point: \begin{align}\hat{\vec{y}}_{t+1}   = \hat{\vec{x}}_t - \eta \nabla f_{\vec{r}_t}(\vec{x}_t). \end{align} This updated dual point is then mapped back to the primal space using the inverse  of mapping $\nabla \Phi$, i.e.:
\begin{align}\label{eq:invstep}\vec{y}_{t+1} = \left(\nabla \Phi\right)^{-1}\!(\hat{\vec{y}}_{t+1}).\end{align}
The resulting primal point $\vec{y}_{t+1}$ may lie outside the constraint set $\mathcal{X}$. To obtain the final feasible point $\vec{x}_{t+1}\in \mathcal{X}$, a projection is made using the Bregman divergence associated with the mirror map~$\Phi$; that is, instead of the orthogonal projection used in OGD, the final cache state becomes:
\begin{align}\label{eq:bregprojstep}
\vec{x}_{t+1}= \Pi_{\mathcal{X} \cap \mathcal{D}}^\Phi(\vec{y}_{t+1}),
\end{align}
where $\Pi_{\mathcal{X} \cap \mathcal{D}}^\Phi(\,\cdot\,)$ is the Bregman projection, which we define formally below, in Definition~ \ref{def:Bregman_projection}. %instead of the Euclidean distance. 

Together, steps \eqref{eq:mapstep}-\eqref{eq:bregprojstep} define OMD. Note that, as it was the case for OGD, $\vec{x}_{t+1}$ is a function of $\{(\vec{r}_{t}, \vec{x}_{t})\} \subset \{(\vec{r}_{s}, \vec{x}_{s})\}^{t}_{s=1} $, hence OMD is indeed an online algorithm.
Two additional technical assumptions on $\Phi$ and $\mathcal{D}$ must hold for steps \eqref{eq:invstep} and \eqref{eq:bregprojstep} to be well-defined.\footnote{All hold for the algorithms we consider in Sec.~\ref{sec:OMDanalysis}.}
First, the gradient of~$\Phi$ must diverge at the boundary of $\mathcal{D}$; this, along with strict convexity, ensures the existence and uniqueness of the Bregman projection in~\eqref{eq:bregprojstep}. Second, the image of $\mathcal{D}$ under the gradient of $\Phi$ should take all  possible values, that is $\nabla\Phi(\mathcal{D}) = \mathbb{R}^N$; this, along again with strict convexity, ensures that $\nabla\Phi$ is one-to-one and onto, so its inverse exists and Eq.~\eqref{eq:invstep} is well-defined.

%We can see that OMD for every $t\geq 2$, 
We observe that setting $\Phi(\vec{x}) = \frac{1}{2} \norm{\vec{x}}^2_2$ and $\mathcal{D} = \mathbb{R}^N$ yields the identity mapping $\nabla \Phi(\vec{x}) = \vec{x},$ for all $\vec x \in \mathcal{D}$. Furthermore, the Bregman divergence associated with this map is just the Euclidean distance $D_\Phi (\vec{x}, \vec{y}) = \frac{1}{2}\norm{\vec{x} -\vec{y}}^2_2 $. Thus, this Euclidean version of OMD is equivalent to OGD, and OMD can be seen as a generalization of the OGD to other mirror maps.

%\noindent\textbf{Bregman Projection.} 
To conclude our description of OMD, we define the Bregman projection \cite{kiwiel1997proximal}.
\begin{definition}
\label{def:Bregman_projection}
    The Bregman projection denoted by $\Pi^{\Phi}_{\mathcal{X} \cap \mathcal{D}}:\mathbb{R}^N\to\mathcal{X} \cap \mathcal{D}$, is defined as
    \begin{align}
        \Pi^{\Phi}_{\mathcal{X} \cap \mathcal{D}}(\vec{y}) &= \underset{\vec{x} \in {\mathcal{X} \cap \mathcal{D}}}{\arg\min}\,D_\Phi (\vec{x},\vec{y}), & \text{where}& &  D_\Phi(\vec{x},\vec{y}) = \Phi(\vec{x}) - \Phi(\vec{y}) - \nabla {\Phi(\vec{y})}^T (\vec{x} - \vec{y})
    \end{align}
 is the Bregman divergence associated with the mirror map $\Phi$. 
\end{definition}

%The mapping $\vec{x} \to D_\Phi(\vec{x},\vec{y})$ is strictly convex, and locally increasing at the boundary of $\mathcal{D}$, this implies the existence and the uniqueness of this projection. 

\subsection{Analysis of Online Mirror Descent Algorithms}\label{sec:OMDanalysis}

We present our main results regarding the application of  OMD under several different mirror maps to the online caching problems. 
%We present our main results regarding the application of different OMD algorithms to the online caching problems. 
%To that end, we discuss the performance of OMD under several different mirror maps. 
We will be concerned with both (a) the regret attained, and (b)~computational complexity issues, particularly pertaining to the associated Bregman projection. 

As we will see, our major observation is that regret of different algorithms is significantly influenced by the diversity of the demand, as captured by the diversity ratio $\frac{R}{h}$. In particular, our analysis allows us to characterize regimes of the diversity ratio in which OGD outperforms other mirror maps, and vice versa.


\subsection{$q$-Norm Mirror Maps}
\label{subsection:q-norm-mirror-maps}
A natural generalization of the OGD algorithm to a broader class of OMD algorithms is via $q$-norm mirror maps, whereby: 
\begin{align}
     \Phi(\vec{x}) = \frac{1}{2}\norm{\vec{x}}^2_q, \quad\text{where }q \in (1,2],~\text{and }   \quad \mathcal{D}&=\mathbb{R}^N.
\label{eq:qnorm_mirrormap}
\end{align}
It is easy to verify that $\Phi$ and $\mathcal{D}$, defined as above, satisfy all technical requirements set in Sec.~\ref{section:OMD} on a mirror map and its domain.
We define $\OMD_{q\nrm}$ to be the OMD Algorithm $\ref{algo:online_mirror_descent}$ with $\Phi$ and $q$ given by Eq.~\eqref{eq:qnorm_mirrormap}.
Note that this map generalizes OGD, which corresponds to the special case $q=2$. 
In what follows, we denote by $\|\cdot\|_p$ the dual norm of $\|\cdot\|_q$. Then, $p \in [2, \infty)$ is such that $\frac{1}{p} + \frac{1}{q} = 1$. Note that sometimes $\OMD_{q\nrm}$
% OMD strategies generated by this class of $q$-norm mirror maps 
is referred to as  a \emph{$p$-norm algorithm}~\citep{ShalevOnlineLearning}. %, where $p= \frac{1}{1 - 1/q} \in [2, \infty)$~

% Note that for $q=1$, the mirror map is undefined because it is not strictly convex w.r.t. $\norm{\,\cdot\,}_1$
% We note that restricting $q\in (1,2]$ ensures that $\Phi(\vec{x})$ is strongly convex w.r.t the norm $\norm{\,\cdot\,}_q$~\cite{Shalev2007}.
% G: removed to gain space
%This class of $q$-norm mirror maps generates OMD strategies known as $p$-norm algorithms with 
%$p= \frac{1}{1 - 1/q} \in [2, \infty)$~\citep{Gentile_pnorm}.
%$p \geq [2, \infty)$ \cite{Gentile_pnorm}.   
 %$\OMD_{q\nrm}$ algorithms   interpolate between the additive-update algorithm OGD ($q=2$) and the multiplicative-update algorithm  resulting from OMD with a neg-entropy map we describe in Section~\ref{sec:neg_entropy}.

%as $q$ converges to $1$ \cite{Gentile_pnorm}.  Though the mirror map is not defined for $q=1$, as the resulting $\Phi$ is \emph{not} differentiable, the limiting algorithm as $q$ converges to $1$ is equivalent to the so-called neg-entropy map over the simplex (capped simplex with $k=1$), and have the same multiplicative update rule with a scaling factor over a general setting of the capped simplex. We prove this result in Theorem~\ref{theorem:equivalent_1norm_negentropy}, and we elaborate in great detail in Sec.~\ref{sec:neg_entropy}.


 %OMD with a neg-entropy map amounts to a multiplicative update rule (see Eq.~\eqref{eq:multi}). Intermediate values of $q\in(1,2]$ thus establish a continuum \cite{Gentile_pnorm} between a multiplicative-update algorithm  (OMD with a neg-entropy map) and an additive-update algorithm (OGD).


%Furthermore, we allow $\text{OMD}_{1\text{-norm}}$ to be included in the definition, by taking the limit $q\to1$.

\subsubsection{Regret Analysis} We begin by providing a regret bound for $\OMD_{q\nrm}$   algorithms in the context of online caching:
\begin{theorem}
\label{theorem:qnorm_regret}
% $\eta = \sqrt{\frac{(q-1) k^2 \left(k^{-\frac{2}{p}}  - N^{-\frac{2}{p}}\right)}{\norm{\vec w}^2_\infty h^2 \left(\frac{R}{h}\right)^{\frac{2}{p}} T}}$%
For $\eta = \sqrt{\frac{(q-1) k^2 \left(k^{-\frac{2}{p}}  - N^{-\frac{2}{p}}\right)}{\norm{\vec w}^2_\infty h^2 \left(\frac{R}{h}\right)^{\frac{2}{p}} T}}$, the regret of $\OMD_{q\nrm}$  over $\mathcal{X}$ satisfies:
\begin{equation}
    \Regret_T(\OMD_{q\nrm}) \leq \norm{\vec w}_\infty h k \left(\frac{R}{h}\right)^{\frac{1}{p}}\sqrt{\frac{1}{q-1}  \left(k^{-\frac{2}{p}} - N^{-\frac{2}{p}}\right) T}.
    \label{eq:qnorm_regret}
\end{equation}
\end{theorem}
\noindent The proof can be found in Appendix \ref{proof:qnorm_regret}. We use an upper bound on the regret of general OMD from %Bubeck 
\cite[Theorem 4.2]{bubeck2015convexbook} and relate it to our setting; in doing so, we  bound the diameter of~$\mathcal{X}$ w.r.t. Bregman divergence under $\Phi$ as well as the dual-norm $\norm{\,\cdot\,}_p$ of the gradients $\nabla f_{\vec{r}_t}(\vec{x}_t)$. %The mirror map is strongly convex w.r.t the norm $\norm{.}_q$, and the Bregman divergence of $\vec{x}_1$ and $\vec{x}_*$ is bounded under $\Phi$. 

Comparing Theorem~\ref{theorem:qnorm_regret} to Theorem~\ref{theorem:pascos_regret}, we see that both attain an $\BigO{\sqrt{T}}$ regret. A natural question to ask when comparing the two bounds is whether there are cases where $\OMD_{q\nrm}$ with $q\neq 2$ outperforms OGD (i.e.,  $\OMD_{2\nrm}$).  The constants in the r.h.s.~of Eq.~\eqref{eq:qnorm_regret} depend on the diversity ratio $\frac{R}{h}$; this, in turn, affects  which is the optimal $q$, i.e., the one that minimizes the bound in Eq.~\eqref{eq:qnorm_regret}. 

%In particular, given a diversity ratio $\frac{R}{h}$, we can use the r.h.s.~of Eq.~\eqref{eq:qnorm_regret} to determine the optimal $q$, i.e, the $q^*\in [1,2]$ that minimizes the upper bound on the regret. 
Let $q^*=\mathop{\arg\inf}_{q\in (1,2]} \mathtt{ub}(q)$ be the optimal $q$, where $\mathtt{ub}:(1,2] \to \reals_+$ is the upper bound in Eq.~\eqref{eq:qnorm_regret}. Note that $q^* \in  [1,2]$. Figure \ref{fig:diversity_regimes} shows $q^*$ as a function of the diversity ratio, for different values of cache capacity $k$.  We observe that OGD ($q=2$) is optimal for lower diversity regimes and larger caches; as diversity increases or cache size decreases, values $q<2$ become optimal. We note also that the transition from $q^*=2$ to $q^*=1$ is sharp, and becomes sharper as $k$ increases. 
\begin{figure}[!t]
    \centering
    \includegraphics[width = 130pt]{graphical_res/Aug/optimal_q.pdf}
    \caption{Numerical characterization of  $q^*\in [1,2]$  as a function of the diversity ratio $R/h$, for different cache capacities $k$ expressed as fractions of the catalog size ($N=100$). Given $R/h$, the optimal $q^*$ is determined as the value in $[1,2]$ that minimizes the upper-bound in Eq.~\eqref{eq:qnorm_regret}. Higher values of $R/h$ represent more diverse requests. Under small diversity, OGD is optimal; as diversity increases, mirror maps for which $q<2$ attain a more favorable upper bound than OGD.}
    \label{fig:diversity_regimes}
\end{figure}
\subsubsection{Optimality Regimes.}\label{sec:optregimes}
Motivated by these observations, we turn our attention to formally characterizing the two regimes under which optimality transitions from $q^*=2$ to $q^*=1$.
We begin by characterizing the upper bound on the regret for these two regimes. Indeed,
by setting $q=2$ in Theorem~\ref{theorem:qnorm_regret}, we obtain an upper bound of the regret of OGD, generalizing Theorem~\ref{theorem:pascos_regret} to the case $R/h > 1$:
\begin{corollary}
\label{corollary:regret_qnorm_q2}
For $\eta  = \textstyle \sqrt{\frac{k \left(1 - \frac{k}{N}\right)}{ \norm{\vec w}^{2}_\infty  h R T}}$ the regret of OGD, satisfies:
\begin{equation}
\Regret_T(\OGD) \leq \norm{\vec{w}}_\infty\sqrt{ hR k \left(1 - \frac{k}{N}\right) T}.
\label{eq:regret_qnorm_q2}
\end{equation}
\end{corollary}
\noindent This a direct consequence of Theorem~\ref{theorem:qnorm_regret}; the proof can be found in Appendix \ref{proof:regret_qnorm_q2}. 
We note that, in this result, we improve upon the bound of Paschos et al.~\cite{PaschosLearningToCache}: for $R=h=1$, the bound in Eq.~\eqref{eq:regret_qnorm_q2} is smaller than  the one in Theorem~\ref{theorem:pascos_regret} by  at least a $\sqrt{2}$ factor.

%The fact that $\text{OMD}_{q\text{-norm}}$ interpolates between additive and multiplicative algorithms for $q=2$ and $q\to1$ respectively, motivates us to provide the other bound for the case of $\text{OMD}_{1\text{-norm}}$. We will further demonstrate why the two corner settings of $\text{OMD}_{q\text{-norm}}$ are of importance in our analysis in Sec. \ref{sec:diversity_and_regret}.

We also characterize the limiting behavior of $\OMD_{q\nrm}$ as $q$ converges to $1$. 
\begin{corollary}
\label{corollary:regret_qnorm_q1}
As $q$ converges to $1$, the upper bound on $\OMD_{q\nrm}$ regret given by Eq.~\eqref{eq:qnorm_regret} converges to:
\begin{equation}
\norm{\vec w}_\infty h k \sqrt{ 2\log\left(\frac{N}{k}\right) T}.
\label{eq:regret_qnorm_q1}
\end{equation}
\end{corollary}
%\noindent The regret bound in Eq. \eqref{eq:qnorm_regret} is not defined for $q=1$. Taking the limit $q$ converges to $1$, this gives the desired result. 
The proof can be found in Appendix \ref{proof:regret_qnorm_q1}. As we show below, this  limit is precisely the bound on the regret attained under the neg-entropy mirror map (see Theorem~\ref{theorem:regret_negentropy}). Armed with Corollaries~\ref{corollary:regret_qnorm_q2} and~\ref{corollary:regret_qnorm_q1}, we can formally characterize the regimes in which either of the two strategies become dominant.
%\subsection{Diversity and regret tightness}
%\label{sec:diversity_and_regret}
%We provide analytical regimes of the optimal $q^*$. Theorem \ref{theorem:optimalq_q2} specifies the regime where $q=2$ should be selected to obtain the tightest regret in the class of $q$-norm mirror maps OMD, and in Theorem \ref{theorem:optimalq_q1}, we give the regime where $q\to1$ should be picked instead. 
In particular, the following result holds:
\begin{theorem}
\label{theorem:optimalq_q2}
OGD, i.e., $\OMD_{q\nrm}$ for $q=2$, is optimal in the class of $\OMD_{q\nrm}$ algorithms when $\frac{R}{h} \leq k$.
\end{theorem}
In other words, when the diversity ratio is smaller than the cache size, it is preferable to update the cache via OGD. The proof, in Appendix \ref{proof:optimalq_q2}, establishes that the upper bound in Eq.~\eqref{eq:qnorm_regret} is monotonically decreasing w.r.t $q$ in the specified interval. 
%This is achieved by showing that the first derivative of Eq.~\eqref{eq:qnorm_regret} is upper-bounded by a negative factor.
Our next result characterizes then the neg-entropy ($q$ converges to $1$) mirror map outperforms OGD:
\begin{theorem}
\label{theorem:optimalq_q1}
The limit, as $q$ converges to $1$, of the  $\OMD_{q\nrm}$ regret bound in Eq.~\eqref{eq:regret_qnorm_q1} is smaller than the corresponding bound for 
%tighter than , yields a tighter regret than  
OGD ($\OMD_{q\nrm}$ with $q=2$) when $\frac{R}{h} > 2 \sqrt{N k}$.
\end{theorem}
The proof is provided in Appendix \ref{proof:optimalq_q1}. 
%G: REMOVED TO GAIN SPACE. ALSO WHAT WE SAY IS QUITE TRIVIAL
%The result is obtained by relaxing the regret bound in Eq.~\eqref{eq:regret_qnorm_q1} using a sharp upper bound, which is subsequently compared to Eq.~\eqref{eq:regret_qnorm_q2}. 
We stress that Theorem~\ref{theorem:optimalq_q1} implies the sub-optimality of OGD in the regime $\frac{R}{h} > 2 \sqrt{N k}$. The experiments in Fig.~\ref{fig:diversity_regimes} suggest the bound in Theorem~\ref{theorem:optimalq_q1} is quite tight: for example for $k=7$ the bounds suggest $q=1$ should be optimal when $R/h$ exceeds $2 \sqrt{100 \times 7} \approx 52.9$, while experiments show that it is optimal when $R/h$ exceeds $45$. On the contrary, we observe that the bound in  Theorem~\ref{theorem:optimalq_q2} seems to be loose and the transitions we observe in Fig.~\ref{fig:diversity_regimes} are sharper than what one would predict from the bounds.

\subsubsection{Dual-Primal Update and Bregman Projection}\label{sec:bregmanomdq}

Having characterized the regret of OMD algorithms, we turn our attention to implementation issues. 
The map to the dual space and back in
%is obtained by replacing 
Eq.~\eqref{eq:mapstep} and Eq.~\eqref{eq:invstep}  (Lines 3 and 5 in Algorithm~\ref{algo:online_mirror_descent}), have the following expression~\cite{Gentile_pnorm}, respectively: 
\begin{align}
\label{eq:q-norm-update}
& \hat{x}_{t,i} = \left(\nabla \Phi(\vec{x}_t)\right)_i = \text{sign} (x_{t,i})\frac{|x_{t,i}|^{q-1}}{\norm{\vec{x}_t}^{q-2}_q}, \quad\text{for all }~i \in \mathcal{N}, \\
%\end{align}
%and 
%\begin{align}
& {y}_{t+1,i} = \left( \left(\nabla \Phi\right)^{-1}(\hat{\vec{y}}_{t+1}) \right)_i = \text{sign} (\hat{y}_{t+1,i}) \frac{|\hat{y}_{t+1,i}|^{p-1}}{\norm{\hat{\vec{y}}_{t+1}}^{p-2}_p}, \quad\text{for all }~i \in \mathcal{N}.\end{align}
%G: GAIN SPACE
%The first update rule is obtained by taking the gradient of the mirror map, while the inverse mapping is the gradient of Legendre conjugate of $\Phi$, that is $\frac{1}{2}\norm{\vec{x}}^2_p$ (see Gentile and Littlestone \cite{Gentile_pnorm}).


Finally, for all $q\in (1,2]$ the Bregman projection in Eq.~\eqref{eq:bregprojstep} (Line 6 in Algorithm \ref{algo:online_mirror_descent}) involves solving a convex optimization problem, in general. For the OGD Algorithm however ($q=2$) the projection is the usual Euclidean projection, and can be performed in $\BigO{N^2}$ steps, using the projection algorithm by Wang and Lu \cite{wang2015projection}. Specifically when $\frac{R}{h} = 1$, only a single component of state is updated at each iteration, and Paschos et al. \cite{PaschosLearningToCache} provide an algorithm that performs the projection in $\BigO{N}$ time.\footnote{To be precise, the projection algorithm as presented in~\cite{PaschosLearningToCache} requires at each iteration a preliminary step with complexity $\BigO{N \log(N)}$ to sort a vector of size $N$, followed by $\BigO{N}$ steps. However, it is possible to replace sorting by $\BigO{\log(N)}$  binary search and insertion operations reducing the complexity to $\BigO{N}$ per iteration.}


%For $q$-norm mirror map OMD as $q\to1$ we provide an alternative mirror map that attains the same regret bound and overcomes the projection difficulty in \ref{sec:neg_entropy}, and in the next section we show why we emphasize on the corner cases $q=2$ and $q\to1$.

\subsection{Neg-Entropy Mirror Map}
\label{sec:neg_entropy}

To conclude this section, we turn our attention to the neg-entropy mirror map that, as discussed earlier, attains the same regret performance as $\OMD_{q\nrm}$ as $q$ converges to $1$.  Beyond its improved performance in terms of regret in the high diversity ratio regime, the neg-entropy mirror map comes with an additional computational advantage: the Bregman projection admits a highly efficient implementation.


Formally,  OMD under the neg-entropy mirror map uses: 
\begin{align}\label{eq:neg-entropy}
\Phi(\vec{x}) &= \sum^N_{i=1} x_i \log\left(x_i\right), \text{  and } \mathcal{D} = \mathbb{R}_{>0}^N.
\end{align}
Note that, as per the requirements  in Sec.~\ref{section:OMD},  $\mathcal{X}\subseteq\mathrm{closure}(\mathcal{D})$. Also, $\nabla\Phi$ indeed diverges at the boundary of $\mathcal{D}$, and $\nabla \Phi(\mathcal{D})=\mathbb{R}^N$, as
\begin{align}\label{eq:negrad}
  \deriv{\Phi(\vec{x})}{x_i}= 1+\log x_i, \quad \text{for all }i\in \mathcal{N}.
\end{align}
 We refer to the resulting algorithm as $\OMD_{\negent}$.

\subsubsection{Regret Analysis}

We first characterize the regret of $\OMD_\negent$:
\begin{theorem}
\label{theorem:regret_negentropy}
For $\eta = \sqrt{\frac{2 \log(N/k)}{\norm{\vec w}^{2}_\infty h^2 T}} $, the regret of $\OMD_{\negent}$ satisfies:
\begin{align}
\Regret_T(\OMD_{\negent}) \leq \norm{\vec w}_\infty hk \sqrt{ 2 \log (N/k)}.
\end{align}
\end{theorem}
\noindent The proof, in Appendix \ref{proof:regret_negentropy}, is similar to the proof of Theorem \ref{theorem:qnorm_regret}. Using again the general bound of the regret of OMD algorithms in Bubeck \cite[Theorem 4.2]{bubeck2015convexbook}, we bound the diameter of $\mathcal{X}$ w.r.t.~to the Bregman divergence as well as the dual norm $\norm{\,\cdot\,}_\infty$ of gradients $\nabla f_{\vec{r}_t}(\vec{x}_t)$. 

Crucially, we observe that $\OMD_{\negent}$ indeed attains the same regret bound as the one in Corollary~\ref{corollary:regret_qnorm_q1}, namely, the bound on $\OMD_{q\nrm}$ when $q$ converges to $1$. This immediately implies the advantage of $\OMD_\negent$ over OGD in high diversity ratio regimes, as described in Sec.~\ref{sec:optregimes} and Theorem~\ref{theorem:optimalq_q1}.

%as $q$ converges to $1$ \cite{Gentile_pnorm}.  Though the mirror map is not defined for $q=1$, as the resulting $\Phi$ is \emph{not} differentiable, the limiting algorithm as $q$ converges to $1$ is equivalent to the so-called neg-entropy map over the simplex (capped simplex with $k=1$), and have the same multiplicative update rule with a scaling factor over a general setting of the capped simplex. We prove this result in Theorem~\ref{theorem:equivalent_1norm_negentropy}, and we elaborate in great detail in Sec.~\ref{sec:neg_entropy}.


 %OMD with a neg-entropy map amounts to a multiplicative update rule (see Eq.~\eqref{eq:multi}). Intermediate values of $q\in(1,2]$ thus establish a continuum \cite{Gentile_pnorm} between a multiplicative-update algorithm  (OMD with a neg-entropy map) and an additive-update algorithm (OGD).


% \ref{theorem:equivalent_1norm_negentropy}

\subsubsection{Dual-Primal Update  and Bregman Projection}
As $\nabla \Phi(\vec{x})$ is given by Eq.~\eqref{eq:negrad}, the inverse mapping is given by $ \left( \left( \nabla \Phi\right)^{-1}(\hat{\vec{y}}_{t+1}) \right)_i = \mathrm{exp}(\hat{y}_{t,i} - 1)$. Hence, the map to the dual space and back in Eq.~\eqref{eq:mapstep}-Eq.~\eqref{eq:invstep}  (Lines 3--5 in Algorithm \ref{algo:online_mirror_descent}) can be concisely written as:
\begin{align}
	y_{t+1,i} & 
	= \exp\left(\hat{x}_{t,i} - \eta \deriv{f_{\vec{r}_t}(\vec{x}_t)}{x_i} - 1\right)
	          = \exp\left( \log({x}_{t,i}) - \eta \deriv{ f_{\vec{r}_t}(\vec{x}_t)}{x_i} \right)
	           = x_{t,i}\,e^{-\eta \deriv{f_{\vec{r}_t}(\vec{x}_t)}{x_i}}, \quad \text{for all}~i \in \mathcal{N}. \label{eq:multi}
\end{align}
In other words, OMD under the neg-entropy adapts the cache state via \emph{a multiplicative rule} (namely, the one implied by \eqref{eq:multi}), as opposed to the additive rule of OGD (see Eq.~\eqref{eq:ogd}).



\begin{algorithm}[!t]
	\caption{Neg-Entropy Bregman projection onto the capped simplex}
	\begin{algorithmic}[1]
		\Require $N$; $k$; $\norm{\vec{y}}_1$; $P$; Sorted $y_N \geq \cdots \geq y_{N-k+1} \geq y_{i}, \forall i \leq N-k$
		\Statex \Comment{ $\vec{y}$ is the intermediate cache state, and $P$ is  a scaling factor initialized to 1}

		\State $y_{N+1} \gets +\infty$
		\For{ b $\in \{N, \dots , N-k+1\}$ }
		\State $m_{b} \gets \frac{k+b-N}{\norm{\vec{y}}_1 - \sum_{i=b+1}^{N} {y_i P}}$
		\If {$y_{b} m_{b}P  < 1 \leq y_{b+1} m_{b} P$}\Comment{ Appropriate $b$ is found}
		\For {i $\geq$ b+1 }
		\State $y_i \gets \frac{1}{ m_{b} P}$
		\EndFor
		\State $P \gets m_b P$
		\State \Return $\vec{y} P$\Comment{ $\vec{y} P$ is the result of the projection }
		\EndIf
		\EndFor
	\end{algorithmic}
	\label{alg:bregman_divergence_projection}
\end{algorithm}

 Finally, the projection algorithm onto the capped simplex can be implemented in $\BigO{N + k \log(k)}$ time for arbitrary $R$ and $h$ values using a waterfilling-like algorithm. The full procedure is presented in Algorithm~\ref{alg:bregman_divergence_projection}.  The algorithm receives as input the top-$k$ elements of $\vec{y}$, sorted in a descending order. It then identifies via a linear search 
 which elements exceed an appropriate threshold and set them to one. The other elements
 %of which the highest-value value elements are set to one, and the remaining elements 
 are scaled by a constant factor to satisfy the capacity constraint.
%  by a different constant factor; which elements are deemed high and low value is determined via a linear search.
 The following theorem holds:
\begin{theorem}
\label{theorem:bregman_divergence}
Algorithm \ref{alg:bregman_divergence_projection} returns the projection $\Pi^{\Phi}_{\mathcal{X} \cap \mathcal{D}}(\vec{y})$ onto the capped simplex $\mathcal{X}$ under the neg-entropy $\Phi$. It requires
% $\BigO{k}$ steps per iteration.  This results in an overall time complexity of 
$\BigO{N + k \log(k)}$ operations per $\OMD_{\negent}$ iteration, for general values of ${R}$ and ${h}$, and only $\BigO{k}$ operations, when $\frac{R}{h} = 1$.
\end{theorem}
\noindent The proof is given in Appendix \ref{proof:bregman_divergence}. To prove this theorem, we characterize the KKT conditions of the minimization problem. Then we show that these conditions can be checked in $\BigO{k}$ time. Finally, we show how maintaining $\vec{y}$ in a partially sorted list across iterations leads to the reported complexity results.
% When $\frac{R}{h} = 1$, Alg.~1 leads to only a single state coordinate update. The projection step takes $\BigO{k}$,  and an extra $\BigO{\log(k)}$ to maintain top-$k$ components of $\vec{x}_t$ sorted online. This gives an overall time complexity of $\BigO{k}$ per iteration of OMD; we note that, in contrast, OGD requires $\BigO{N}$ per iteration in the $\frac{R}{h} = 1$ setting (see Sec.~\ref{sec:bregmanomdq}).
% When $\frac{R}{h} \neq  1$, a partial sort is to maintain top-$k$ components of $\vec{y}_t$ sorted; this can be done using partial sorting in $\BigO{N + k \log(k)}$  \citep{paredes2006optimal}. This gives an $\BigO{N + k \log(k)}$ time complexity per iteration; in contrast, OGD requires $\BigO{N^2}$ steps per iteration in this setting (see Sec.~\ref{sec:bregmanomdq}).

Theorem~\ref{theorem:bregman_divergence} implies that $\OMD_{\negent}$ has significant computational savings when compared to OGD (cf.~Sec.~\ref{sec:bregmanomdq}), both when $\frac{R}{h} = 1$ and for general values of $R$ and $h$. The per-iteration time complexity of $\OGD$ and $\OMD_\negent$ is summarised in Table~\ref{table:timecomplexity}.

%When $\frac{R}{h} = 1$, the overall time complexity is $\BigO{k}$ per iteration of $\OMD_{\negent}$;  in contrast, OGD requires $\BigO{N}$ steps per iteration in the same setting. Similarly, for general values of $R$ and $h$, $\OMD_{\negent}$ per-iteration complexity is $\BigO{N + k \log(k)}$, while OGD requires $\BigO{N^2}$ steps per iteration. The per-iteration time complexity of $\OGD$ and $\OMD_\negent$ is summarised in Table~\ref{table:timecomplexity}.

\begin{table}[t]
\[
\begin{array}{@{}l*{3}{c}@{}}
\toprule
\text{Diversity ratio} & \multicolumn{2}{c@{}}{\text{Policy}}\\
    \cmidrule(l){2-3}
    & \OGD & \OMD_\negent \\
\midrule
R/h=1 & \BigO{N}&  \BigO{k} \\
R/h > 1 & \BigO{N^2} & \BigO{ N + k \log(k) }\\
\bottomrule
\end{array}
\]
 \caption{Per-iteration time complexity of $\OGD$ and $\OMD_\negent$.}
 \label{table:timecomplexity}
\end{table}

==> backups__zipped_project_/5._Update_Cost.tex <==
\section{Update Cost}
\label{sec:movement}
The model presented in Sec.~\ref{s:system} can be extended by adding the  cost to update the cache state after the batch of $R$ requests has been served. This cost may quantify the additional load on the server or on the network. This update cost is often called  \emph{movement cost} \cite{bubeck2015convexbook} or \emph{switching cost} \cite{taleoftwometrics}.
As the state changes from $\vec x_t$ to $\vec x_{t+1}$, the cache evicts part of the file $i$ if $x_{t+1,i} < x_{t,i}$ and stores additional bytes of it if $x_{t+1,i} > x_{t,i}$.
We make the following assumptions:
\begin{enumerate}
    \item Evictions do not engender update costs, as the cache can perform them autonomously;
    \item Insertions of (part of) files which have been requested do not engender update costs, as these files have already been retrieved by the cache in their entirety to satisfy the requests.
    \item Insertions of (part of) files which have not been requested incur a cost proportional to the fraction of file retrieved. 
\end{enumerate}

We can then define the update cost at time slot $t$ as
\begin{align}
\label{eq:movement_fractional}
\updatecost_{\vec{r}_t} (\vec{x}_{t}, \vec{x}_{t+1} ) = \sum_{i \notin \supp(\vec{r}_t)} w_i' \max\left\{0, x_{t+1,i} - x_{t,i}\right\},
\end{align}
where $\supp(\vec{r}_t) = \left\{i \in \mathcal{N}: r_{t,i}  \neq 0\right\}$ denotes the support of $\vec{r}_t$, i.e., the set of files that have been requested during the $t$-th timeslot, and $w'_i$ is the cost to retrieve the whole file $i$, and can in general be different from the cost $w_i$ appearing in~\eqref{e:cost}.

If the update cost is introduced in the model, the \emph{extended} regret can be defined as follows:
% Call it extended regret in text.
\begin{align}
    \text{E-Regret}_T({\mathcal{A}}) &= \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{R}^T_{R,h}}{\sup} \left\{ \sum^T_{t=1} f_{\vec{r}_t}(\vec{x}_t) + \updatecost_{\vec{r}_t} (\vec x_{t}, \vec x_{t+1})-\sum^T_{t=1} f_{\vec{r}_t}(\vec{x_*}) \right\} \label{eq:regret_extended}\\
    &\le  \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{R}^T_{R,h}}{\sup} \left\{  \sum^T_{t=1} f_{\vec{r}_t}(\vec{x}_t) - \sum^T_{t=1} f_{\vec{r}_t}(\vec{x}_*) \right\} +  \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{R}^T_{R,h}}{\sup}\left\{ \sum^T_{t=1}  \updatecost_{\vec{r}_t} (\vec x_{t}, \vec x_{t+1})\right\}. \label{eq:rounding_regret_upper_bound}
\end{align}
Equation~\eqref{eq:rounding_regret_upper_bound} shows that the regret of an arbitrary online algorithm can be bounded by considering the regret we have derived so far (Eq.~\eqref{eq:regret}), ignoring update costs, and subsequently accounting for an additional term corresponding to the update. Note that the optimal static allocation does not incur any update cost.  Equation~\eqref{eq:rounding_regret_upper_bound} implies that any policy with $\BigO{\sqrt{T}}$ regret and  $\BigO{\sqrt{T}}$ update cost in expectation has also $\BigO{\sqrt{T}}$ extended  regret.

One of the reasons why we did not introduce directly the update cost is that, in the fractional setting, OMD update cost is zero both for the Euclidean (OGD) and the neg-entropy ($\OMD_{\negent}$) mirror maps. Formally, we have:
\begin{proposition}
\label{prop:free_updates}
For any request batch $\vec r_t$ received at time slot $t \in [T]$, the update of fractional cache state from $\x_t \in \mathcal{X}$ to $\x_{t+1} \in \mathcal{X}$ obtained by $\OMD_\negent$ or $\OGD$ has no cost, i.e.,
\begin{align}
    \updatecost_{\vec r_t} (\vec x_t, \vec x_{t+1}) = 0.
\end{align}
\end{proposition}
The proof is provided in Appendix~\ref{proof:free_updates}. In fact, the gradient step increases the fraction  $x_{t,i}$ only for files $i$  that have been requested, and the projection step reduces the fraction for all other files in order to satisfy the capacity constraint. It follows that $x_{t+1,i} - x_{t,i} > 0$ if and only if $i \in \supp(\vec r_t)$, and thus $\updatecost_{\vec{r}_t} (\vec{x}_{t}, \vec{x}_{t+1} )=0$. As a consequence, the $\BigO{\sqrt{T}}$ regret guarantees we proved in the previous sections for OGD and $\OMD_{\negent}$ hold also under the more general definition in~\eqref{eq:regret_extended}.
%
In the next section, we show that update costs cannot be neglected when the cache is forced to store a file in its entirety.

==> backups__zipped_project_/6._Integral_Caching.tex <==

\section{Integral Caching}
\label{sec:rounding}
In the previous sections, we assumed that the cache can store arbitrarily small chunks of a file, and this allowed us to design no-regret policies that employ fractional caching. However, this assumption can be too strong in some applications. For example, when the catalog is composed of small sized files, the discreteness of chunks sizes cannot be neglected;
% we are limited to only extract relatively big chunks and rounding such allocations can cause a significant performance drop;
moreover, the metadata needed for each chunk can cause memory and computational overheads.  These observations motivate us to study the case when the cache can only store the entire file. We refer to this setting as the \emph{integral} caching. Formally, we restrict the cache states to belong to the set 
\begin{align}
    \mathcal{Z} = \left\{\vec \zeta \in \{0,1\}^N: \sum_{i \in \mathcal{N}} \zeta_i = k\right\}.
\end{align}
Note that the set $\mathcal{Z}$ is a restriction of the set of fractional caching states $\mathcal{X}$ to its corners, i.e., $ \mathcal{Z} = \mathcal{X} \cap \{0,1\}^N$; thus, we maintain the same definition of the requests and the service cost objective in Sec.~\ref{s:system}.  In this setting, we allow policies to be randomized. This extension turns out to be necessary in order to have a sublinear regret policy; formally, we have:
\begin{proposition}
\label{proposition:deterministic_worst_case_regret}
Any deterministic policy restricted to select integral cache states in $\mathcal{Z}$ has the following lower bound on its regret
\begin{align}
      \Regret_T(\policy) \geq  k \left(1 - \frac{k}{N}\right)T.
\end{align}
\end{proposition}
To prove the proposition, we show that an adversary can exploit the deterministic nature of the policy by continuously requesting the files that are not stored in the cache. We provide the proof in Appendix~\ref{proof:deterministic_worst_case_regret}. 

We thus turn our attention to randomized policies. In particular, we focus on a special class of randomized policies, constructed by (a) a fractional online caching policy $\policy$, i.e., of the type we have studied so far (see Sec.~\ref{s:system}),   combined with (b)  a randomized rounding scheme $\Xi$, that maps fractional caching states to integral ones.  In particular, for every $t \geq 1$ the randomized rounding scheme $\Xi: \mathcal{X}^t \times \mathcal{Z}^{t-1} \times [0,1] \to \mathcal{Z}$ maps the previous fractional cache states $\{\x_{s}\}^{t-1}_{s=1} \in \mathcal{X}^{t-1}$, the current fractional cache state $\x_t \in \mathcal{X}$, the previous random cache states $\{\z_{s}\}^{t-1}_{s=1} \in \mathcal{Z}^{t-1}$, and a source of randomness $\xi_t \in [0,1]$ to a new random cache state $\z_t \in \mathcal{Z}$ where 
\begin{align}\label{eq:expectzt}\mathbb{E} [\z_t] = \x_t.\end{align}
Note that the rounding function takes into account not only the current fractional state $\x_t$, which determines its expectation, but also the past fractional and integral states ($\{(\z_{s},\x_{s})\}^{t-1}_{s=1}$); this is in fact instrumental in attaining a sublinear extended regret (see Theorems~\ref{theorem:rounding_independent} and~\ref{theorem:rounding_coupled} below).

We extend the definitions of the regret and the extended regret as follows:
\begin{align}
\mathrm
{Regret}_T(\policy, \Xi) = \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{R}^T_{R,h}}{\sup} \left\{ \mathbb{E} \left[ \sum^T_{t=1} f_{\vec{r}_t}(\vec{z}_t)\right]- \sum^T_{t=1} f_{\vec{r}_t}(\vec{z}_*) \right\}, 
\label{eq:integral_regret}
\end{align}
and 
\begin{align}
    \mathrm{E\mbox{-}Regret}_T(\policy, \Xi) &= \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{R}^T_{R,h}}{\sup} \left\{ \mathbb{E} \left[\sum^T_{t=1} f_{\vec{r}_t}(\vec{z}_t) + \updatecost_{\vec{r}_t} (\vec z_{t}, \vec z_{t+1})\right]-\sum^T_{t=1} f_{\vec{r}_t}(\vec{z}_*) \right\},
    \label{eq:integral_extendedregret}
\end{align}
where the expectation is taken over the random choices of the rounding scheme $\Xi$, and  \begin{align}\vec{z}_*=\argmin_{\vec{z} \in \mathcal{Z}}\sum^T_{t=1} f_{\vec{r}_t}(\vec{z})\end{align}
 is the optimal static integral cache state (in hindsight).  By restricting our focus to such randomized policies, we obtain a regret that is equal to the fractional caching policy's regret. Formally, we have:
  \begin{proposition}
\label{proposition:regret_transfer}
Any random integral caching states $\z_t \in \mathcal{Z}$, for $t\in[T]$, generated from fractional caching states of policy $\policy$ via a randomized rounding $\Xi$ that satisfies \eqref{eq:expectzt},  yield the same regret as $\policy$, i.e., $\Regret_T(\policy, \Xi) =\Regret_T(\policy)$, given by \eqref{eq:integral_regret} and \eqref{eq:regret}, respectively.
\end{proposition}
 The result follows from the linearity of the cost functions and the expectation operator; moreover, the static optimum can always be selected to be integral from the integrality of the capacity constraint and linearity of the objective function. The proof is provided in Appendix.~\ref{proof:regret_transfer}.

Proposition~\ref{proposition:regret_transfer} thus implies that regret guarantees for a fractional policy $\mathcal{A}$ readily transfer to the integral regime, when coupled with rounding $\Xi$. Unfortunately, when considering the extended regret  (Eq.~\eqref{eq:integral_extendedregret}) instead, na\"ive  rounding policies can arbitrary evict and fetch objects to the cache causing large update costs (see Theorem~\ref{theorem:rounding_independent}). Thus, unless rounding is carefully designed, we may fail to have sublinear regret guarantees when accounting for update costs. In the next section, we show how a randomized rounding scheme~$\Xi$ can be  selected to avoid incurring large update costs. 


\subsection{Rounding Schemes and Extended Regret} 
% \begin{align}\mathcal{Z} = {\left\{ \vec{\zeta} \in \{0,1\}^N: \sum^N_{i=1} \zeta_i = k\right\}}.\end{align}
%be the set of possible integral cache configurations.
% We are going to show that, by coupling OMD methods with opportune rounding techniques, the service-cost regret guarantees derived for the fractional setting transfer (in expectation) to the integral one. %
% A straightforward approach is to use OMD to update a fractional state $\vec{x}_t\in \mathcal{X}$ and then randomly sample an integral state $\vec z_t \in \mathcal{Z} $ after each round of requests so that $\mathbb{E}[\vec z_t] = \vec{x}_t$, for all $t\geq 1$. 
%\begin{align}\mathbb{E}[\vec z_t] = \vec{x}_t,\quad \text{for all}~t\geq 1.\end{align}

% S: describe formally randomized algos.




% In this section, we 

\subsubsection{Online Independent Rounding.}  If we consider a fractional caching state $\x_t \in \mathcal{X}$, then a random integral caching state $\vec z_t \in \mathcal{Z}$ with the marginal $\mathbb{E}[\z_t] = \x_t$ exists and can be sampled in polynomial time (see, e.g., \cite{geocaching2015, ioannidis2016adaptive}).  Thus, a rounding scheme $\Xi$ can be constructed with such strategy that takes as input the current fractional cache state $\x_t$ 
ignoring previous fractional cache states $\{\x_{s}\}^{t-1}_{s=1} \in \mathcal{X}^{t-1}$, and previous random cache states $\{\z_{s}\}^{t-1}_{s=1} \in \mathcal{Z}^{t-1}$.
%and ignores the previous cache state $\x_{t-1}$ and random cache state $\z_{t-1}$. 
We provide pseudocode for this procedure in Algorithm~\ref{algo:online_rounding}. Because at any time $t$ the random cache states are independent, we refer to this rounding as \emph{online independent sampling}. Unfortunately, when considering the extended regret~\eqref{eq:integral_extendedregret}, any caching policy coupled with this rounding scheme loses its $\BigO{\sqrt{T}}$ regret guarantee. Formally, we have the following:

\begin{theorem}
\label{theorem:rounding_independent}
% Consider a policy that adds $\eta$ fraction to the requested file and 
Any randomized caching policy constructed by an online policy $\policy$ combined with  online independent sampling as a randomized rounding scheme $\Xi$ has linear (worst-case) extended regret, i.e., 

\begin{align}
        \mathrm{E\mbox{-}Regret}_T(\policy, \Xi)  = \Omega (T).
\end{align}


% Online independent sampling incurs $\Omega(T)$ update cost in the worst case.
\end{theorem}
The proof is provided in Appendix~\ref{proof:rounding_independent}. Online independent sampling causes more frequent cache updates, as it samples a new state from $\z_t$ ignoring the previous state $\vec\zeta_{t-1}$ sampled from $\z_{t-1}$. Intuitively, imposing dependence (coupling) between the two consecutive random states may significantly reduce the expected update cost.


\begin{algorithm}[!t]
	\begin{algorithmic}[1]
% 	\State Sample $\xi$ u.a.r in the interval $[0,1]$ 
    % \State Assume that files' representations in $\mathcal{N}$ are assigned in increasing movement cost, such that $w'_i \geq w'_{i-1}$ for all $i \in \mathcal{N} \setminus \{1\}$. 
	\Procedure {\Rounding}{$\x \in \mathcal{X}$, $\xi \in [0,1]$}
    \State $\mathcal I_0 = \emptyset$
    \For {$i = 1,2,\dots, N$} 
    \State $\mathcal I_{i} \gets \begin{cases} \mathcal I_{i-1}\cup \{ i\} &\text{if}\quad \sum^i_{j=1} x_{j} \geq \xi + |\mathcal I_{i-1}|,\\ \mathcal I_{i-1} &\text{otherwise.} \end{cases}$
    %\State $I_{i} \gets  I_{i-1} \cup C_i$
    \EndFor
    \State \Return $\vec \z \gets \sum_{i \in I_N} \vec e_i $
	\EndProcedure
	\State  
\State $\triangleright$ In  \emph{online independent sampling},  \Rounding  is called with arguments ($\x_t$, $\xi_t$), where $\x_t$ are provided by algorithm $\mathcal{A}$ and $\{\xi_t\}_{t=1}^{T-1}$ are i.i.d., sampled u.a.r. from $[0,1]$.
\State $\triangleright$ In \emph{online coupled rounding}, a $\xi$ is sampled once u.a.r. from $[0,1]$; then,  \Rounding  is called with arguments ($\x_t$, $\xi$), i.e., using the same $\xi$ for all $\x_t$  provided by algorithm $\mathcal{A}$. 
\State $\triangleright$ Both return an integral r.v.~$\z_t$ s.t. $\mathbb{E}[\z_t]=\vec x_t$, with the expectation being over $\{\xi_t\}_{t=1}^{T-1}$ and $\xi$, respectively.
	\end{algorithmic}
	\caption{\Rounding. }
	\label{algo:online_rounding}
\end{algorithm}

\subsubsection{Online Coupled Rounding.}  To address this issue, our proposed \emph{online coupled rounding} scheme is  described also in Algorithm~\ref{algo:online_rounding}, using however the same randomization source across all timeslots. In particular, the coupling across states comes from the use of the same uniform random variable~$\xi$; the dependency on the previous random states (coupling) is possible when fixing the value of the random variable  sampled only once. 
%In that sense, %Algorithm~\ref{algo:online_rounding} is an adaptation of the random placement schemes proposed by~\cite{geocaching2015, ioannidis2016adaptive} with the main difference is for any time slot $t \in {T}$ the random variables $\vec z_t$ are implicitly constructed and coupled with $\vec z_{t-1}$. 
A consequence of this coupling is that 
%the computation of the next integral state is computationally efficient and requires only small movement costs. 
the next integral state can be computed efficiently and lead to small movement costs.
Note that Algorithm~\ref{algo:online_rounding} does not necessarily find an optimal coupling, but it is sufficiently conservative: overall, it yields a sublinear update cost, and thus preserves the sublinearity of the regret. This is formally expressed in the following Theorem: 
\begin{theorem}
\label{theorem:algorithm_rounding_coupled}
Consider an OMD policy configured with learning rate $\eta = \Theta{\left( \frac{1}{\sqrt{T}}\right)}$ that selects the states $\{\x_t\}^T_{t=1} \in \mathcal{X}^T$, and a uniform random variable $\xi$ with support $[0,1]$. At time $t$, the randomized rounding algorithm $\Xi$ in  Algorithm~\ref{algo:online_rounding} takes as input current cache state $\x_t$ and $\xi$ and outputs the random integral cache configurations $\vec z_{t} \in \mathcal{Z}$ satisfying $ \mathbb {E}_{\xi} [\vec z_t] = \x_t$. The expected movement cost of the random integral cache states is 
\begin{align}
  \mathbb E_\xi \left[\updatecost_{\vec r_t}\left(\vec z_{t}, \vec z_{t+1} \right)\right] = \BigO{\sqrt{T}},
\end{align}
when $\xi$ is sampled once u.a.r. from the interval $[0,1]$ and then fixed for $t \in [T]$. Moreover, the extended regret is sublinear 
\begin{align}
    \mathrm{E\mbox{-}Regret}_T(\policy, \Xi)  = \BigO {\sqrt{T}}.
\end{align}
\end{theorem}
We provide the proof in Appendix~\ref{proof:algorithm_rounding_coupled}. In summary, any OMD policy combined with online coupled rounding yields $\BigO {\sqrt{T}}$ extended regret in the integral caching setting. The computational complexity of online coupled rounding is \BigO{N}  (see also  Fig.~\ref{fig:online_coupled_rounding}).

\subsubsection{Online Optimally-Coupled Rounding.}
It is possible in general to reduce the update cost of online coupled rounding.
In particular, minimizing the expected update cost over all joint distributions of the random variables $\vec z_t$ and $\vec z_{t+1}$ leads to an optimal transport problem~\cite{peyre2019computational}.
%If we optimize over all the joint distributions of the random variables $\vec z_t$ and $\vec z_{t+1}$ seeking to minimize the expected update cost, then such objective is attained by solving an optimal transport problem~\cite{peyre2019computational}. 
For completeness, we describe this rounding scheme here, though (1) it does not reduce the extended regret guarantee attained by online coupled rounding (up to multiplicative constants), and (2) it has an increased computational cost.

Formally, at each time $t$ the random variables $\vec z_t$ with marginal $\vec x_t$ can be constructed by sampling from a distribution $\vec p_t$ with \BigO{N} support $\left \{\vec{\zeta}^1_t, \vec{\zeta}^2_t, \dots, \vec{\zeta}^{|\vec p_t|}_{t}\right\}$, where $p_{t,i} = \mathbb{P} (\vec z_t = \vec\zeta^i_t)$ for $i \in [\card{\vec p_t}]$. The decomposition can be performed in \BigO{k N \log(N)} steps~\cite{geocaching2015, ioannidis2016adaptive}. We denote the joint probability $\mathbb{P} \left (\vec z_{t+1} = \vec\zeta^j_{t+1} , \vec z_t = \vec\zeta^i_{t}\right)$ by the flow $f_{i,j}$ for all $(i,j) \in [|\vec p_t|] \times [|\vec p_{t+1}|]$. The optimal transport problem can be described by the following linear program:
\begin{align*}
\text{Minimize:}& \quad
\quad \mathbb{E}\left[ \updatecost\left(\z_t,\z_{t+1}\right)\right] = \sum^{|\vec p_t|}_{i=1} \sum^{|\vec p_{t+1}|}_{j=1}  \updatecost_{\vec r_t} \left(\vec \zeta^i_{t},\vec \zeta^j_{t+1}\right) f_{i,j}\\
\text{Subject to:}& \quad
\sum^{|\vec p_{t+1}|}_{j=1}f_{i,j} = p_{t,i}, & \forall i \in [|\vec p_t|],\\
\phantom{\text{Subject to:}}& \quad\sum^{|\vec p_{t}|}_{i = 1} f_{i,j} = p_{t+1, j}, & \forall j \in  [ |\vec p_{t+1}|],\\
\phantom{\text{Subject to:}}& \quad f_{i,j} \in [0,1], & \forall (i,j)\in  [|\vec p_t|] \times [|\vec p_{t+1}|].
\end{align*}
% where $\mathcal{C} (\vec F)$ is the expected update cost, given as
% \begin{align}
%     \mathcal{C} (\vec F) \triangleq \mathbb{E}\left[ \updatecost\left(\z_t,\z_{t+1}\right)\right] = \sum^{|\vec p_t|}_{i=1} \sum^{|\vec p_{t+1}|}_{j=1}  \updatecost_{\vec r_t} (\vec \zeta^i_{t},\vec \zeta^j_{t+1} ) f_{i,j}.
% \end{align}

We  solve the above linear program to obtain a minimum-cost flow $[f^*_{i,j}]_{(i,j)\in  [|\vec p_t|] \times [|\vec p_{t+1}|]}$. If the random state at time $t$ is $\vec \zeta^i_t$, then we select the new random state to be $\vec  \zeta^j_{t+1}$ with (conditional) probability $ \mathbb{P} \left( \vec z_{t+1} =\vec \zeta^j_{t+1} \given \vec z_t =\vec \zeta^i_t \right) = \frac{f^*_{i,j}}{p^t_i}$.
Such coupling ensures that the expected update cost is minimized. When we combine this rounding scheme with a no-regret fractional policy we obtain sublinear extended regret~\eqref{eq:integral_extendedregret}:
\begin{corollary}
\label{corollary:opt_coupling_sublinear_updatecost}
Consider an OMD policy configured with learning rate $\eta = \Theta{\left( \frac{1}{\sqrt{T}}\right)}$ combined with online optimally-coupled rounding $\Xi$. The obtained randomized integral caching policy has sublinear extended regret, i.e., 
\begin{align}
    \mathrm{E\mbox{-}Regret}(\policy, \Xi) = \BigO{\sqrt{T}}.
\end{align}
\end{corollary}
The corollary follows from Theorem~\ref{theorem:algorithm_rounding_coupled}, because online coupled rounding constructs a feasible transportation flow (see Fig.~\ref{fig:conditioned_implicit} for an illustration) that is not necessarily optimal but gives sublinear update costs, and the optimal flow can only have lower update cost.
% The proof is provided in Appendix~\ref{proof:opt_coupling_sublinear_updatecost}.

The na\"ive implementation of the optimal transport problem has $\BigO{N^3}$ time complexity, but several efficient approximations exist in the literature~\cite{peyre2019computational}. 

% Therefore, coupling the random states gives the following expected movement cost
% \begin{align}
%     \mathbb{E}_{\vec z_t}\left[ \mathbb{E}_{\vec z_{t+1} | \vec z_t }\left[\norm{\vec z_{t+1} - \vec z_t}_{1, \vec w'}\right]\right] &= \sum^{|\vec p_t|}_{i=1} \sum^{|\vec p_{t+1}|}_{j=1} \norm{\zeta^j_{t+1}-\zeta^i_{t}}_{1, \vec w'} \mathbb{P} ( \vec z_{t+1} =\zeta^j_{t+1} | \vec z_t =\zeta^i_t) \mathbb{P}(\vec z_t =\zeta^i_t) \\
%     &=  \sum^{|\vec p_{t+1}|}_{j=1} \norm{\zeta^j_{t+1}-\zeta^i_{t}}_{1, \vec w'} f^*_{i,j}.
% \end{align}

% The flow constructed by Algorithm~\ref{algo:online_coupled_rounding} (see Figure~\ref{fig:conditioned_implicit}) is a feasible solution of the above problem and satisfies the hypothesis of Theorem~\ref{theorem:rounding_coupled}. The optimal flow obtained by solving \OptTransport{} can only reduce the expected movement cost; thus, the online optimally-coupled rounding satisfies the hypothesis in Theorem~\ref{theorem:rounding_coupled} and preserves the sub-linearity of regret. 

% The update cost of the online optimally-coupled rounding is sublinear and preserves the sublinearity of the extended regret~\eqref{eq:regret_extended}.




% Unfortunately, when we consider the more general definition of regret including the update cost~\eqref{eq:regret_extended} such \emph{independent sampling} can incur linear update cost in the worst case and hence we no longer have the regret guarantee.

% In particular, 
% Caratheodory's theorem \cite{rockafellar1970convex} guarantees that, for any~$\vec x_t$, the support of $\vec z_t$ can be limited to at most $N$ cache configurations;  Warmuth and Kuzmin provided a practical algorithm \cite[Algorithm 2]{WarmuthRandomizedPCA}.
% When sampling occurs at each time $t$ independently from the past, we refer to this rounding scheme as \emph{independent sampling}.
% \subsection{Update Cost}

% Similarly to  Sec.~\ref{sec:movement}, we can introduce the update cost as
% \begin{align}
% \label{eq:movement_integer}
% \updatecost_{\vec{r}_t} (\vec\zeta_{t}, \vec\zeta_{t+1} ) = \sum_{i \notin \supp(\vec{r}_t)} w_i' \max(0, \vec\zeta_{t+1,i} - \vec\zeta_{t,i}),
% \end{align}
% and extend similarly the regret notion as in Eq.~\eqref{eq:regret_extended}. Unfortunately, the update cost \emph{cannot} be neglected under independent sampling: 





% \begin{theorem}
% \label{theorem:rounding_independent}
% Online independent sampling  has $\Omega(T)$ update cost in worst case.
% \end{theorem}
% The proof can be found in Appendix \ref{proof:rounding_independent}. This result implies that, when considering the more general definition of regret including the update cost, OMD coupled with independent sampling loses its $\BigO{\sqrt{T}}$ regret guarantee. 
%
% Independent sampling causes more frequent cache updates, as it samples $\z_{t+1}$ ignoring the current state $\vec\zeta_t$. Intuitively, coupling the two consecutive states may significantly reduce the expected update cost.
% Moreover,  if we manage to achieve $\BigO{\sqrt{T}}$ update cost in expectation, by the upper bound in Eq.~\eqref{eq:rounding_regret_upper_bound}  the generalized  regret will also be $\BigO{\sqrt{T}}$. 



% \subsection{Online Coupled Rounding}
% \label{sec:online_coupled_rounding}
% % Assume at time $t$ the random variable $\vec z_t$ with $\mathbb{E}[{\vec z_t}] = \vec{x}_t $ has been used to sample the integral state $\vec \zeta_t$ and that the a-priori probability to sample $\vec \zeta_t$ was $\mathbb P(\vec z_t = \vec  \zeta_t) = p_t$. 

% % Algorithm~\ref{algo:online_coupled_rounding} takes as input the fractional states $\vec{x}_{t}$ and $\vec{x}_{t+1}$, the integral state $\vec\zeta_t$ and its corresponding probability $p_t$. It implicitly constructs a new random variable $\vec z_{t+1}$ with $\mathbb{E}[\vec z_{t+1}] = \vec x_{t+1}$ and samples the new integral state $\vec \zeta_{t+1}$ from it. In more detail, the algorithm generates a sequence of random variables whose marginal distribution is progressively closer to $\vec{x}_{t+1}$. The marginal distributions of two consecutive random variables differ only for a $\delta_{i,j}$ mass moved from file $i$ to file $j$, i.e., the marginal distribution changes from $\vec x$ to $\vec x - \delta_{i,j} \vec e_i + \delta_{i,j} \vec e_j$. 
% % Each intermediate random variable is sampled through the procedure \textsc{Elementary $\delta$-movement} that is detailed in Algorithm~\ref{algo:elementary_movement} in Appendix~ \ref{app:online_rounding}.
% % Algorithm~\ref{algo:online_coupled_rounding} returns the new state $\vec \zeta_{t+1}$ and its corresponding probability $p_{t+1}$.  
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{graphical_res/Aug/algo.pdf}
%     \caption{The random integral cache configuration $\vec z_t$ obtained by calling \CoupledRounding{} on the fractional cache states $\x_t$. The catalog size is $N = 8$ and the cache size $k=3$.}
%     \label{fig:online_coupled_rounding}
% \end{figure}

%  Algorithm~\ref{algo:online_coupled_rounding} takes as input the fractional state $\vec{x}_{t}$ and it implicitly constructs a random variable $\vec z_{t}$ with $\mathbb{E}[\vec z_{t}] = \vec x_{t}$ and samples the new integral state $\vec \zeta_{t}$ from it in \BigO{N} operations (see Fig.~\ref{fig:online_coupled_rounding}). Note that the randomization in  Algorithm~\ref{algo:online_coupled_rounding} comes from the uniformly sampled random variable $\xi$, and the coupling part comes by fixing the value of the random variable once sampled; moreover, Algorithm~\ref{algo:online_coupled_rounding} is an adaptation of the random placement schemes proposed by  \cite{geocaching2015, ioannidis2016adaptive} with the main difference is for any time slot $t \in {T}$ the random variables $\vec z_t$ are implicitly constructed and coupled with $\vec z_{t-1}$. As a result, such adaptation is computationally efficient and produces random cache states with small movement costs.

% % G: REMOVED TO GAIN SPACE
% %Note that the algorithm does not keep track of the probability distribution of each random variable $\vec z_t$, but only of the probability such distribution assigns to the sampled state $\vec \zeta_t$.

% Starting then from an arbitrary random variable $\vec z_1$ with $\mathbb{E}_\xi[\vec z_{1}] = \vec{x}_{1}$, we can at each time slot use a policy $\mathcal A$ to generate the new fractional state $\vec{x}_{t+1}$ and then Algorithm~\ref{algo:online_coupled_rounding} is called to sample the integral cache state $\vec z_{t+1}$. 


% The proof can be found in Appendix \ref{proof:algorithm_rounding_coupled}. We show that the change from $\vec{x}_t$ to $\vec{x}_{t+1}$ can be decomposed in at most $N-1$ elementary operations (movement of $\delta_{i,j} \in \mathbb{R}_+$ mass from component $i \in \mathcal{N}$ to $j \in \mathcal{N}$), and that for each of them 
% the expected  $\vec{w}'$-weighted $l_1$-distance between the sampled integral configuration is of the order
% $\BigO{\delta_{i,j}}$.

% % Finally, we note that one can find the  joint probability distribution of  $\vec z_t$ and $\vec z_{t+1}$ by formulating an optimal transport problem \cite{peyre2019computational} to minimize $\mathbb E\left[\norm{\vec z_{t+1} - \vec z_t}_{1,\vec w'}\right]$. This approach may lead a smaller expected update cost, but it requires to explicitly consider all possible values of $\vec Z_t$ and $\vec Z_{t+1}$, that may be as many as $|\mathcal Z| = {N \choose k}$. Our algorithm instead efficiently builds the support of these random variables at each step to have size at most linear in $N$.


% \subsection{Online Optimally-Coupled Rounding}
% \label{sec:online_optimal_coupled_rounding}
% The coupling scheme given by \CoupledRounding{} in Algorithm~\ref{algo:online_coupled_rounding} for any time slot $t$ implicitly conditions the new random cache state with respect to the previously sampled random state as illustrated in Figure~\ref{fig:conditioned_implicit}; unfortunately, such coupling does not necessarily yield the smallest expected movement cost.  We can optimize over all the joint distributions of the random variables $\vec z_t$ and $\vec z_{t+1}$ seeking to minimize $\mathbb E\left[\norm{\vec z_{t+1} - \vec z_t}_{1,\vec w'}\right]$, and such objective is attained by solving an optimal transport problem~\cite{peyre2019computational}. For any time slot $t$ the random variables $\vec z_t$ with marginal $\vec x_t$ can be constructed by sampling from a distribution $\vec p_t$ with \BigO{N} support $\{\zeta^1_t, \zeta^2_t, \dots, \zeta^{|\vec Z_t|}_{t}\}$, where $p_{t,i} = \mathbb{P} (\vec z_t = \zeta^i_t)$. The decomposition can be performed using \cite[Algorithm 2]{ioannidis2016adaptive}.


% We denote the joint probability $\mathbb{P} (\vec z_{t+1} = \zeta^j_{t+1} , \vec z_t = \zeta^i_{t})$ by the flow $f_{i,j}$ for all $(i,j) \in [|\vec p_t|] \times [|\vec p_{t+1}|]$, then the optimal transport problem can be described by the following linear program:

% \begin{subequations}
% \begin{gather*}
% \OptTransport\end{gather*}
% \begin{mini}
% {}{\sum^{|\vec p_t|}_{i=1} \sum^{|\vec p_{t+1}|}_{j=1}  \norm{\zeta^j_{t+1}-\zeta^i_{t}}_{1, \vec w'} f_{i,j} }{}{}
% \addConstraint{\sum^{|\vec p_{t+1}|}_{j=1}}{f_{i,j} = p_{t,i},}{\quad i \in \{1,2, \dots, |\vec p_t|\}}
% \addConstraint{\sum^{|\vec p_{t}|}_{i = 1} }{ f_{i,j} = p_{t+1, j},}{\quad j \in \{1,2, \dots, |\vec p_{t+1}|\}}
% \addConstraint{}{f_{i,j} \in [0,1],}{\quad(i,j)\in \{1,2,\dots  |\vec p_t|\} \times \{1,2, \dots, |\vec p_{t+1}|\} }.
%     % \text{Subject to}& \nonumber \\
%     % &\sum^{|\vec p_{t+1}|}_{j=1} f_{i,j} = p_{t,i}, \forall i \in \{1,2, \dots, |\vec p_t|\} \\
%     % &\sum^{|\vec p_{t}|}_{i = 1} f_{i,j} = p_{t+1, j}, \forall i \in \{1,2, \dots, |\vec p_{t+1}|\} \\
%     % & 0 \leq f_{i,j} \leq 1, \forall (i,j)\in \{1,2,\dots  |\vec p_t|\} \times \{1,2, \dots, |\vec p_{t+1}|\} 
% \end{mini}
% \end{subequations}

% We solve \OptTransport{} to obtain a minimum cost flows $f^*_{i,j}$ for any $(i,j) \in \{1,2,\dots  |\vec p_t|\} \times \{1,2, \dots, |\vec p_{t+1}|\} $. If the random state at time $t$ is $\zeta^i_t$, then we select the new random state to be $\zeta^j_{t+1}$ with the conditional probability 
% \begin{align}
%     \mathbb{P} ( \vec z_{t+1} =\zeta^j_{t+1} | \vec z_t =\zeta^i_t) = \frac{f^*_{i,j}}{p^t_i}.
% \end{align}
% Therefore, coupling the random states gives the following expected movement cost
% \begin{align}
%     \mathbb{E}_{\vec z_t}\left[ \mathbb{E}_{\vec z_{t+1} | \vec z_t }\left[\norm{\vec z_{t+1} - \vec z_t}_{1, \vec w'}\right]\right] &= \sum^{|\vec p_t|}_{i=1} \sum^{|\vec p_{t+1}|}_{j=1} \norm{\zeta^j_{t+1}-\zeta^i_{t}}_{1, \vec w'} \mathbb{P} ( \vec z_{t+1} =\zeta^j_{t+1} | \vec z_t =\zeta^i_t) \mathbb{P}(\vec z_t =\zeta^i_t) \\
%     &=  \sum^{|\vec p_{t+1}|}_{j=1} \norm{\zeta^j_{t+1}-\zeta^i_{t}}_{1, \vec w'} f^*_{i,j}.
% \end{align}


% The flow constructed by Algorithm~\ref{algo:online_coupled_rounding} (see Figure~\ref{fig:conditioned_implicit}) is a feasible solution of the above problem and satisfies the hypothesis of Theorem~\ref{theorem:rounding_coupled}. The optimal flow obtained by solving \OptTransport{} can only reduce the expected movement cost; thus, the online optimally-coupled rounding satisfies the hypothesis in Theorem~\ref{theorem:rounding_coupled} and preserves the sub-linearity of regret. The naive implementation of the optimal transport problem has the time complexity of $\BigO{N^3}$, but several efficient approximations exist in the literature~\cite{peyre2019computational}. 



==> backups__zipped_project_/7.1._Experiments.tex <==
\section{Numerical Experiments}
\label{sec:experiments}

%We evaluate the performance of the different caching policies under synthetic traces and a real trace.  

\subsection{Experimental setup}


\subsubsection{Datasets.}
Throughout all experiments, we assume equal costs per file, i.e., $w_i = w'_i = 1, \forall i \in \mathcal{N}$. The learning rate $\eta^*$ denotes the learning rate value specified in Corollary~\ref{corollary:regret_qnorm_q2} and in Theorem~\ref{theorem:regret_negentropy} for $\OGD$ and $\OMD_\negent$, respectively. The learning rate is selected to be  $\eta^*$ unless otherwise mentioned. In what follows, we distinguish the number of batches  in the trace ($B$) and the time horizon ($T$). 

We generate the following synthetic datasets, summarized in Table~\ref{tab:traces}. 



\noindent\textbf{Fixed Popularity.}
Requests are i.i.d.~and sampled from a catalog of $N =200$ files according to a \emph{Zipf} distribution with exponent $\alpha = 0.8$. 
%This distribution represents the popularity of the files.
Each batch counts a single request ($R=1$). We set set the time horizon as $T = 10^5$.  The cache capacity is $k = 100$.
Note that the total number of requests is equal to the product of the requests in each batch ($R$) and the number of batches (both reported in Table~\ref{tab:traces}).


\noindent\textbf{Batched Fixed Popularity}.
Request are generated as above from a Zipf distribution with exponent $\alpha$, but are now grouped in batches of $R=5 \times 10^3$ requests.
We take different exponents $\alpha \in \{0.1, 0.2, 0.7\}$ for  traces \emph{Batched Fixed Popularity} (1), (2), and (3), respectively, in Table \ref{tab:traces}.
The parameter $\alpha$ controls the diversity of the files in the request batches. If $\alpha = 0$, then each file is requested with equal probability, %of each file to be requested,
corresponding to $\frac{R}{h} \to N$ (high diversity). As we increase $\alpha$, the requests become more concentrated; this corresponds to $\frac{R}{h} \to 1$ (low diversity). Table~\ref{tab:traces} shows the value of $h$ observed in each trace. In all cases, we select catalog size $N = 10^4$, cache size $k \in \{25,125,250\}$,  and time horizon $T = 10^4$. 

\noindent\textbf{Transient Popularity}. We also generate two non-stationary request traces. In these traces, we reset the popularity distribution periodically.


In the first scenario (\emph{Partial Popularity Change} traces), we still have batches of $R=5 \times 10^3$ requests sampled from a catalog of $N=10^4$ files according to a Zipf distribution with parameter $\alpha \in \{0.1, 0.3,0.4\}$ for traces (1), (2), and (3), respectively. But now the popularities of a subset of files is modified every $10^3$ time slots. In particular the 5\% most popular files become the 5\% least popular ones and vice versa. 
We want to model a situation where the cache knows the timescale over which the request process changes and which files are affected (but not how their popularity changes). Correspondingly, the time horizon is also set to $T=10^3$ and, at the end of each time horizon, the cache redistributes uniformly the cache space currently allocated by those files. The cache size is $k=50$.


%the content provider periodically refreshes its library, and both catalog changes and the periods of stationarity are known (even though the popularity values are not).
%In every period of $10^3$ timeslots, the  we change the popularity of 10\% of the catalog  as follows: the popularities of most 5\% popular files are randomly assigned to the 
%least 5\% popular files, and vice versa.
 
% From the algorithmic perspective,
%we set the targeted time horizon to be equal to the (known) period of stationarity; i.e., $T=10^3$. 
%That is, when implementing OGD and OMD, we set the time horizon $T$ (used to determine $\eta$) to be equal to this period; at the end of each period $T$, we reset the caching decision of each algorithm, by spreading the mass uniformly among the files affected by this popularity change. %We set the period of stationarity to $T=10^3$. 
% This happens 5 times, resulting in a total of 5T batches in the entire trace. We  again generate different diversity regimes, with exponents $\alpha \in \{0.1, 0.4,0.7\}$, batch size $R=5 \times 10^3$, cache size $k =5$, catalog size $N = 500$. This gives traces \emph{Partial Popularity Change} (1), (2) and (3), corresponding to the different exponents, respectively.
 
In the second scenario (\emph{Global Popularity Change} trace) each batch counts only a single request ($R=1$) sampled from a catalog of $N=10^4$ files according to a {Zipf} distribution with exponent $\alpha=0.8$. Every $5\times 10^4$ time slots (or requests in this case) the popularity of each files change: file $i \in \{1, \dots, N\}$ assumes the popularity of file $j=(1+ (i + N/4) \! \mod N$). The cache size is $k=200$.  We also generate the \emph{Downscaled Global Popularity Change} trace as  a downscaled version of \emph{Global Popularity Change} trace, where the catalog size is reduced to $N = 25$, the cache size to $k=4$, and the number of requests to $ 9 \times 10^3$. The learning rate is set to $\eta = 0.01$.


%each content we perform a circular shift by a step $50$ to the components of the popularity distribution vector. Hence,  the popularity profile of the requests changes significantly from one timeslot to the next. This gives the \emph{Global Popularity Change} trace, with a total duration (total number of batches) of $15 \times 10^4$.


\noindent\textbf{Akamai Trace.}
We consider also a real file request from the Akamai CDN provider~\cite{akamaiGiovanni}. The trace spans 1 week, and we extract from it about $8.5 \times 10^7$ requests for the $N=10^3$ most popular files. We consider re catalog is truncated to  the $10^3$ most popular files. We group requests in batches of size $R = 5 \times 10^3$, and we consider a time horizon $T = 100$ time slots corresponding roughly to 1 hour. %($5 \times 10^5$ individual file requests). 
The cache size is $k=25$.
% 


\begin{table}[!t]
%\centering
  \caption{Trace Summary}
  \label{tab:traces}
  \begin{tabular}{llllll}
    \hline
    Trace  & \# Batches &$T$ &$N$& $R$ & $h$ \\
    \hline
    Fixed Popularity & $1.5  \times 10^5$ & $1.5  \times 10^5$& $10^4$ &1 & 1\\
    Batched Fixed Popularity  (1) & $10^4$ & $10^4$&$  10^4$& $5\times10^3$  & 2\\
    Batched Fixed Popularity  (2) & $10^4$ & $10^4$&$ 10^4$& $5\times10^3$  & 5\\
    Batched Fixed Popularity (3) & $10^4$ & $10^4$&$ 10^4$& $5\times10^3$  & 87\\
    Partial Popularity Change  (1)  & $5 \times 10^3$ & $10^3$&$10^4$& $5\times10^3$ & 2\\
    Partial Popularity Change  (2)  &  $5 \times 10^3$ & $10^3$&$10^4$& $5\times10^3$ & 6\\
    Partial Popularity Change  (3) &  $5 \times 10^3$  & $10^3$&$10^4$& $5\times10^3$ & 10\\
    Global Popularity Change & $1.5 \times 10^5$ & $1.5 \times 10^5$& $10^4$&1 & 1\\
    Downscaled Global Popularity Change & $9 \times 10^3$ & $9 \times 10^3$& $25$&1 & 1\\
    CDN Trace & $1.7\times 10^4$ & $10^2$ & $10^3$ & $5 \times 10^3$ & $380$ \\
    \hline
\end{tabular}
\end{table}

\subsubsection{Online Algorithms.} Starting with the gradient based algorithms, we implemented $\OMD_\negent$ with the projection defined in Algorithm \ref{alg:bregman_divergence_projection}. We implemented two different projection algorithms for $\OGD$: the one by Paschos et al. \cite{PaschosLearningToCache} for the setting $\frac{R}{h} = 1$, and the one by Wang and Lu  \cite{wang2015projection} for the general setting $\frac{R}{h} > 1$. 

In addition, we implemented four caching eviction policies: LRU, LFU, W-LFU, and FTPL. LRU and LFU evict the least recently used and least frequently used file, respectively. While LFU estimates file popularities considering all requests seen in the past, W-LFU~\cite{karakostas2002exploitation} is an LFU variant that only considers requests during a recent time window $W$, which we set equal to $T \times R$ in our experiments. The policies LRU, LFU, and W-LFU are allowed to process individual requests.  FTPL is a no-regret policy proposed by Mukhopadhyay and Sinha~\cite{mukhopadhyay2021online} that is practically a LFU policy with Gaussian perturbation. 
Finally, we define \emph{Best Static} to be the optimal static allocation $\vec{x}^*
$, i.e., the configuration storing the $k$ most popular files as we consider $w_i = 1, \forall i \in \mathcal{N}$. We also define \emph{Best Dynamic} to be the caching policy that stores the $k$ most popular files at any time for the synthetic traces (for which the instantaneous popularity is well defined). The optimality of such policy is formally studied in~\cite{panigrahy21}.



\subsubsection{Online Rounding.}
We also implemented the three rounding policies described in~Sec.~\ref{sec:rounding}: (a) the online independent sampling algorithm, (b) the online coupled rounding described 
in Algorithm \ref{algo:online_rounding}, and (c) the online optimally-coupled rounding described in Sec~\ref{sec:online_optimal_coupled_rounding}.
We tested them with  $\OGD$ with learning rate $\eta = 0.01$ and the \emph{Downscaled Global Popularity Change} trace.


\subsubsection{Performance Metrics.} We measure performance  w.r.t.~four metrics  defined in Table~\ref{tab:performance_metrics}. The Normalized Average Cost $\mathrm{NAC}(\mathcal{A}) \in [0,1]$ corresponds to the time-average cost over the first $t$ time slots, normalized by the batch size $R$.  The Normalized Moving Average Cost  $\mathrm{NMAC}(\mathcal{A}) \in [0,1]$ is computed similarly, using a moving average instead over a time window $\tau > 0$; we use $\tau = 500$ in our experiments.  We also consider the Time Average Regret $\mathrm{TAR} (\mathcal{A}) \in [0, R]$, which is precisely the time average regret over the first $t$ time slots. Finally, when studying rounding algorithms, we also measure and report the Cumulative Update Cost $\mathrm{CUC}(\mathcal{A}) \in [0, \infty)$.

% %\centering
%   \caption{Performance Metrics}
%   \label{tab:performance_metrics}
%   \begin{tabular}{llll}
%     \hline
%     Performance metric & Definition & Range & Objective\\
%     \hline
%     Normalized Average Cost (NAC) & $ \displaystyle\mathrm{NAC} (\mathcal{A}) =  \frac{1}{R t} \sum^t_{s = 0 }f_{\vec{r}_s}(\vec{x}_s)$ & $[0,1]$ & $\downarrow$\\
%     Normalized Moving Average Cost (NMAC) &  $\displaystyle\mathrm{NMAC} (\mathcal{A}) =  \frac{1}{R \min(\tau,t)} \sum^t_{s = t-\min(\tau,t) }f_{\vec{r}_s}(\vec{x}_s)$& $[0,1]$ & $\downarrow$\\
%     Time Average Regret (TAR)& $\displaystyle\mathrm{TAR} (\mathcal{A}) = \frac{1}{t}\left(\sum^t_{s=1} f_{\vec{r}_s}(\vec{x}_s)- \sum^t_{s=1} f_{\vec{r}_s}(\vec{x_*}) \right)  $ & $[0,R]$ & $\downarrow$\\
%     Cumulative Update Cost (CUC) & $\displaystyle\mathrm{CUC} (\mathcal{A}) = \sum^t_{s=1} \updatecost_{\vec{r}_s} (\vec{x}_{s}, \vec{x}_{s+1} )$ & $ [0, \infty]$ & $\downarrow$\\
%     \hline
% \end{tabular}
% \end{table}

\begin{table}[!t]
%\centering
  \caption{Performance Metrics. All are better if lower.}
  \label{tab:performance_metrics}
  %\begin{small}
  \begin{tabular}{lll}
    \hline
    Performance metric & Definition & Range \\
    \hline
    Normalized Average Cost  & $ \mathrm{NAC} (\mathcal{A}) =  \frac{1}{R t} \sum^t_{s = 0 }f_{\vec{r}_s}(\vec{x}_s)$ & $[0,1]$\\
    Normalized Moving Average Cost  &  $\mathrm{NMAC} (\mathcal{A}) =  \frac{1}{R \min(\tau,t)} \sum^t_{s = t-\min(\tau,t) }f_{\vec{r}_s}(\vec{x}_s)$& $[0,1]$ \\
    Time Average Regret& $\mathrm{TAR} (\mathcal{A}) = \frac{1}{t}\left(\sum^t_{s=1} f_{\vec{r}_s}(\vec{x}_s)- \sum^t_{s=1} f_{\vec{r}_s}(\vec{x_*}) \right)  $ & $[0,R]$ \\
    Cumulative Update Cost & $\mathrm{CUC} (\mathcal{A}) = \sum^t_{s=1} \updatecost_{\vec{r}_s} (\vec{x}_{s}, \vec{x}_{s+1} )$ & $ [0, \infty]$ \\
    \hline
\end{tabular}
%\end{small}
\end{table}

%When comparing different policies, the static optimum incurs the same cost for all policies. Therefore it is enough to compare using the NAC metric instead of the regret. While in the real trace we use NMAC metric, to better capture the variability in real traces by averaging over the time window $\tau$, and we take $\tau = 500$.



%\subsubsection{Stationary requests under different diversity regimes}

%\subsubsection{Robustness to changing popularity requests}
% We first consider the scenario, where we have a partial popularity change. The supplier of the files is aware of the catalog change. Therefore, the targeted time horizon is the period of stationarity, this is take to be $T = 10^3 $. We reset the caching decision of each algorithm, by spreading the mass uniformly among the files affected by this popularity change. We generate different diversity regimes, with exponents $\alpha \in \{0.1, 0.4,0.7\}$, batch size $R=5 \times 10^3$, cache size $k =5$, catalog size $N = 500$. The popularity changes every $10^3$ requests, and we change 10\% of the catalog 5 times. Hence, $T= 5 \times 10^3$ is the total number of request batches. The change is a random shuffling of the popularity of the most 5\% popular files with least 5\% popular files. This gives the trace \emph{Partial popularity change trace} (1), (2) and (3) corresponding to the different exponents respectively.

  




==> backups__zipped_project_/7.1._Experiments1.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate the performance of the different caching policies under synthetic traces and a real trace.  

\subsection{Experimental setup}


\subsubsection{Datasets.}
Throughout all experiments, we assume equal costs per file, i.e., $w_i = w'_i = 1, \forall i \in \mathcal{N}$. We generate the following synthetic datasets, summarized in Table~\ref{tab:notations_definitions}:


\noindent\textbf{Fixed Popularity.}
In this setting, we sample independently at any time individual requests from \emph{Zipf} distribution with exponent $\alpha = 0.8$. This distribution represents the popularity of the files.
We set the catalog size to $N =200$ and time horizon $T = 10^5$.  The cache capacity is $k = 10$, and the learning rate $\eta^*$ is the optimal learning rates corresponding to each algorithm.

\noindent\textbf{Batched Fixed Popularity}.
Similar to the above setting, we sample independently at any time individual requests from a \emph{Zipf} distribution. Except that the generated requests are grouped into batches of size $R = 5\times 10^3$. We take different exponents $\alpha$, this parameter controls the diversity of the files in the request batches. If $\alpha = 0$, then each file is requested with equal probability, %of each file to be requested,
corresponding to $\frac{R}{h} \to N$ (high diversity). As we increase $\alpha$, the requests become more concentrated; this corresponds to $\frac{R}{h} \to 1$ (low diversity). We consider exponents $\alpha \in \{0.1, 0.2, 0.7\}$, which  give  traces \emph{Batched Fixed Popularity} (1), (2), and (3), respectively, in Table \ref{tab:notations_definitions}. In all cases, we select catalog size $N = 200$, cache size $k \in \{2,5,10\}$, batch size $R = 5 \times 10^3$ and time horizon $T = 10^4$. 

\noindent\textbf{Transient Popularity}. We also generate two non-stationary request traces. In these traces, we reset the popularity distribution periodically.


In the first scenario, 
we consider a partial popularity change. Intuitively, we aim to model a situation where the supplier of the contents periodically refreshes its library, and both catalog changes and the periods of stationarity are known (even though the popularity values are not).
  In every period of $10^3$ timeslots, the  we change the popularity of 10\% of the catalog  as follows: the popularities of most 5\% popular files are randomly assigned to the 
 least 5\% popular files, and vice versa.
 From the algorithmic perspective,
we set the targeted time horizon to be equal to the (known) period of stationarity; i.e., $T=10^3$. 
That is, when implementing OGD and OMD, we set the time horizon $T$ (used to determine $\eta$) to be equal to this period; at the end of each period $T$, we reset the caching decision of each algorithm, by spreading the mass uniformly among the files affected by this popularity change. %We set the period of stationarity to $T=10^3$. 
 This happens 5 times, resulting in a total of 5T batches in the entire trace. We  again generate different diversity regimes, with exponents $\alpha \in \{0.1, 0.4,0.7\}$, batch size $R=5 \times 10^3$, cache size $k =5$, catalog size $N = 500$. This gives  traces \emph{Partial Popularity Change} (1), (2) and (3), corresponding to the different exponents, respectively.
 

In the second scenario, we sample individual requests independently from a \emph{Zipf} distribution with exponent $\alpha=0.8$. Then, these individual requests are grouped into request batches. After every $5\times 10^4$ time slots we perform a circular shift by a step $50$ to the components of the popularity distribution vector. Hence,  the popularity profile of the requests changes significantly from one timeslot to the next. This gives the trace \emph{Changing Popularity}, with a total duration (total number of batches) of $15 \times 10^4$.


\noindent\textbf{CDN Trace.}
We use a real file request trace collected from a major Content Delivery Network (CDN). We only consider 1 week of the CDN trace, and the catalog is truncated to  the $10^3$ most popular files. The requests arrive in batches of size $R = 5 \times 10^3$, and we target the time horizon to be the average number of batch requests collected in as single hour $ T = 100 $ ($5 \times 10^5$ individual file requests). The policies LRU, LFU and 2-LFU are allowed to process individual requests. We take the refresh periodicity of 2-LFU to be $T \times R$ requests. 



\begin{table}[!t]
%\centering
  \caption{Trace Summary}
  \label{tab:notations_definitions}
  \begin{tabular}{llllll}
    \hline
    Trace  & \# Batches &$T$ &$N$& $R$ & $h$ \\
    \hline
    Fixed Popularity & $10^5$ & $10^5$& 200&1 & 1\\
    Changing Popularity  & $15 \times 10^4$ & $15 \times 10^4$& 200&1 & 1\\
    Batched Fixed Popularity  (1) & $10^4$ & $10^4$&200& $5\times10^3$  & 40\\
    Batched Fixed Popularity  (2) & $10^4$ & $10^4$&200& $5\times10^3$  & 53\\
    Batched Fixed Popularity (3) & $10^4$ & $10^4$&200& $5\times10^3$  & 346\\
    Partial Popularity Change  (1)  & $5 \times 10^3$ & $10^3$&500& $5\times10^3$ & 40\\
    Partial Popularity Change  (2)  &  $5 \times 10^3$ & $10^3$&500& $5\times10^3$ & 169\\
    Partial Popularity Change  (3) &  $5 \times 10^3$  & $10^3$&500& $5\times10^3$ & 473\\
    CDN Trace & $1.7\times 10^4$ & $10^2$ & $10^3$ & $5 \times 10^3$ & $380$ \\
    \hline
\end{tabular}
\end{table}

\subsubsection{Online Algorithms.} Starting with the gradient based algorithms, we implement $\OMD_\negent$ with the projection defined in Algorithm \ref{alg:bregman_divergence_projection}. We implement $\OGD$  using two implementations of the projection algorithm, one by Paschos et al. \cite{PaschosLearningToCache} for the setting $\frac{R}{h} = 1$, and one by Wang and Lu  \cite{wang2015projection} for the general setting $\frac{R}{h} \neq 1$. 

In addition, we implement the classical caching policies LRU, LFU and 2-LFU. LRU (least recently used) and LFU (least frequently used) are the classic caching policies. The 2-LFU is a Window-LFU \cite{karakostas2002exploitation}, where the time window is selected to be $W = T \times R$.  
Finally, we define \emph{Best Static} to be $\vec{x}^*
$, i.e. the state  storing the most $k$ popular files that is optimal when $w_i = 1, \forall i \in \mathcal{N}$. We also define \emph{Best Dynamic} to be the cache that stores the most $k$ popular files at any time for the synthetic traces. 

\noindent\textbf{Randomized Rounding.}
We also implement two rounding policies. To do so, we  generate fractional caching decisions by running $\OGD$ with learning rate $\eta = 0.01$. We round these both via (a) the independent sampling algorithm, and (b) the online coupled rounding 
in Algorithm \ref{algo:online_coupled_rounding}.


\subsubsection{Performance Metrics.} We measure performance  w.r.t.~four metrics  defined in Table~\ref{tab:performance_metrics}. The Normalized Average Cost $\mathrm{NAC}(\mathcal{A}) \in [0,1]$ corresponds the time-average fraction of cache misses up to time slot $t$, normalized by the batch size $R$.  The Normalized Moving Average Cost  $\mathrm{NMAC}(\mathcal{A}) \in [0,1]$ is computed similarly, using a moving average instead over a time window $\tau > 0$; we use $\tau = 500$ in this case.  We also consider the Time Average Regret $\mathrm{TAR} (\mathcal{A}) \in [0, R]$, which is precisely regret upto time slot $t$, scaled by $t$. Finally, when studying rounding algorithms, we also measure and report the Cumulative Update Cost $\mathrm{CUC}(\mathcal{A}) \in [0, \infty)$.

% \begin{table}[!t]
% %\centering
%   \caption{Performance Metrics}
%   \label{tab:performance_metrics}
%   \begin{tabular}{llll}
%     \hline
%     Performance metric & Definition & Range & Objective\\
%     \hline
%     Normalized Average Cost (NAC) & $ \displaystyle\mathrm{NAC} (\mathcal{A}) =  \frac{1}{R t} \sum^t_{s = 0 }f_{\vec{r}_s}(\vec{x}_s)$ & $[0,1]$ & $\downarrow$\\
%     Normalized Moving Average Cost (NMAC) &  $\displaystyle\mathrm{NMAC} (\mathcal{A}) =  \frac{1}{R \min(\tau,t)} \sum^t_{s = t-\min(\tau,t) }f_{\vec{r}_s}(\vec{x}_s)$& $[0,1]$ & $\downarrow$\\
%     Time Average Regret (TAR)& $\displaystyle\mathrm{TAR} (\mathcal{A}) = \frac{1}{t}\left(\sum^t_{s=1} f_{\vec{r}_s}(\vec{x}_s)- \sum^t_{s=1} f_{\vec{r}_s}(\vec{x_*}) \right)  $ & $[0,R]$ & $\downarrow$\\
%     Cumulative Update Cost (CUC) & $\displaystyle\mathrm{CUC} (\mathcal{A}) = \sum^t_{s=1} \updatecost_{\vec{r}_s} (\vec{x}_{s}, \vec{x}_{s+1} )$ & $ [0, \infty]$ & $\downarrow$\\
%     \hline
% \end{tabular}
% \end{table}

\begin{table}[!t]
%\centering
  \caption{Performance Metrics. All are better if lower.}
  \label{tab:performance_metrics}
  %\begin{small}
  \begin{tabular}{lll}
    \hline
    Performance metric & Definition & Range \\
    \hline
    Normalized Average Cost  & $ \displaystyle\mathrm{NAC} (\mathcal{A}) =  \frac{1}{R t} \sum^t_{s = 0 }f_{\vec{r}_s}(\vec{x}_s)$ & $[0,1]$\\
    Normalized Moving Average Cost  &  $\displaystyle\mathrm{NMAC} (\mathcal{A}) =  \frac{1}{R \min(\tau,t)} \sum^t_{s = t-\min(\tau,t) }f_{\vec{r}_s}(\vec{x}_s)$& $[0,1]$ \\
    Time Average Regret& $\displaystyle\mathrm{TAR} (\mathcal{A}) = \frac{1}{t}\left(\sum^t_{s=1} f_{\vec{r}_s}(\vec{x}_s)- \sum^t_{s=1} f_{\vec{r}_s}(\vec{x_*}) \right)  $ & $[0,R]$ \\
    Cumulative Update Cost & $\displaystyle\mathrm{CUC} (\mathcal{A}) = \sum^t_{s=1} \updatecost_{\vec{r}_s} (\vec{x}_{s}, \vec{x}_{s+1} )$ & $ [0, \infty]$ \\
    \hline
\end{tabular}
%\end{small}
\end{table}

%When comparing different policies, the static optimum incurs the same cost for all policies. Therefore it is enough to compare using the NAC metric instead of the regret. While in the real trace we use NMAC metric, to better capture the variability in real traces by averaging over the time window $\tau$, and we take $\tau = 500$.



%\subsubsection{Stationary requests under different diversity regimes}

%\subsubsection{Robustness to changing popularity requests}
% We first consider the scenario, where we have a partial popularity change. The supplier of the files is aware of the catalog change. Therefore, the targeted time horizon is the period of stationarity, this is take to be $T = 10^3 $. We reset the caching decision of each algorithm, by spreading the mass uniformly among the files affected by this popularity change. We generate different diversity regimes, with exponents $\alpha \in \{0.1, 0.4,0.7\}$, batch size $R=5 \times 10^3$, cache size $k =5$, catalog size $N = 500$. The popularity changes every $10^3$ requests, and we change 10\% of the catalog 5 times. Hence, $T= 5 \times 10^3$ is the total number of request batches. The change is a random shuffling of the popularity of the most 5\% popular files with least 5\% popular files. This gives the trace \emph{Partial popularity change trace} (1), (2) and (3) corresponding to the different exponents respectively.

  




==> backups__zipped_project_/7.2._Experiments.tex <==

\subsection{Results}
\subsubsection{Stationary Requests}
Figures \ref{fig:performance_stationary} (a) and \ref{fig:performance_stationary} (b) show the performance w.r.t.~$\mathrm{NAC}$ of OGD and $\OMD_\negent$,  respectively, under different learning rates $\eta$ on the \emph{Fixed Popularity} trace. We observe that  both algorithms  converge slower under small learning rates, but reach a final lower cost, while  larger learning rates lead to faster convergence, albeit to higher final cost. This may motivate the adoption of 
%motivates choosing  
a diminishing learning rate, 
%as also indicated by our theory (see Theorems~\ref{theorem:optimalq_q1} and \ref{theorem:optimalq_q2}): 
that combines the best of the two options, starting large to enable fast convergence, and enabling eventual fine-tuning. We show one curve corresponding to a diminishing learning rate both for $\OGD$ and $\OMD_\negent$, and indeed they achieve the smallest costs. The  learning rate denoted by $\eta^*$ is the learning rate that gives the tightest worst-case regrets for $\OGD$ and $\OMD_\negent$, as stated in Theorems~\ref{corollary:regret_qnorm_q2} and \ref{theorem:regret_negentropy}). While this learning rate is selected to protect against any (adversarial) request sequence, it is not too pessimistic: Figures \ref{fig:performance_stationary} (a) and \ref{fig:performance_stationary}(b) show it performs well when  compared to other learning rates. 
%(\fix{see Theorems~\ref{theorem:optimalq_q1} and \ref{theorem:optimalq_q2}}):%


Figure \ref{fig:performance_stationary} (c) shows the time-average regret $\mathrm{TAR}$ of OGD and $\OMD_\negent$  over the \emph{Fixed Popularity} trace. As both algorithms have sub-linear regret, their time average regret goes to $0$ for $T \to \infty$.
Note how instead LRU exhibits a constant time average regret.
%We observe that both converge to the static optimum cost; this confirms also the sub-linearity of the regret, which implies the time average regret goes to 0 for $T\to \infty$. We also observe that the two algorithms provide a cost reduction of 20\% compared to LRU.

\begin{figure}[!t]
\centering
  \subcaptionbox{$\mathrm{NAC}$ of OGD}{
    \includegraphics[width=.25\textwidth]{graphical_res/Aug/fixed_ogd.pdf}\!\!
  }%
  \subcaptionbox{$\mathrm{NAC}$ of $\OMD_\negent$}{
     \centering
    \includegraphics[width=.25\textwidth]{graphical_res/Aug/fixed_omd.pdf}\!\!
  }%
  \subcaptionbox{Time-Average Regret}{
    \includegraphics[width=.25\textwidth]{graphical_res/Aug/fixed_average_regret.pdf}
  }
  \caption{NAC of the different caching policies over the \emph{Fixed Popularity} trace. Subfigures (a) and (b) show the performance of OGD and $\OMD_\negent$ respectively under different learning rates. For small learning rates the algorithms both converge slower but more precisely, while for larger learning rates they converge faster, but to a higher cost. Subfigure (c) shows the time average regret of the two gradient algorithms. Since the regret is sub-linear, the time average regret converges to $0$ as $T \to \infty$.  }
  \label{fig:performance_stationary}
\end{figure}

\begin{figure}[!t]
  \centering

  \subcaptionbox{ $k = 25, \alpha =0.1$}{
  \includegraphics[width=.2\linewidth]{graphical_res/Aug/diversity_regime_4_1_25.pdf}
  }
  \subcaptionbox{$k = 125, \alpha =0.1$}{
  \includegraphics[width=.2\linewidth]{graphical_res/Aug/diversity_regime_4_1_125.pdf}
  }
  \subcaptionbox{$k = 250, \alpha =0.1$}{
  \includegraphics[width=.2\linewidth]{graphical_res/Aug/diversity_regime_4_1_250.pdf}
  }
  \\
  \subcaptionbox{$k = 25, \alpha =0.2$}{
  \includegraphics[width=.2\linewidth]{graphical_res/Aug/diversity_regime_5_2_25.pdf}
  }
  \subcaptionbox{$k = 125, \alpha =0.2$}{
  \includegraphics[width=.2\linewidth]{graphical_res/Aug/diversity_regime_5_2_125.pdf}
  }
  \subcaptionbox{$k = 250, \alpha =0.2$}{
  \includegraphics[width=.2\linewidth]{graphical_res/Aug/diversity_regime_5_2_250.pdf}
  }
  \\
    \subcaptionbox{$k = 25, \alpha =0.7$}{
  \includegraphics[width=.2\linewidth]{graphical_res/Aug/diversity_regime_87_7_25.pdf}
  }
  \subcaptionbox{$k = 125, \alpha =0.7$}{
  \includegraphics[width=.2\linewidth]{graphical_res/Aug/diversity_regime_87_7_125.pdf}
  }
  \subcaptionbox{$k = 250, \alpha =0.7$}{
  \includegraphics[width=.2\linewidth]{graphical_res/Aug/diversity_regime_87_7_250.pdf}
  }
  \caption{NAC of $\OMD_\negent$ and OGD evaluated under different cache sizes and diversity regimes. We use  traces \emph{Batched Fixed Popularity} (1), (2), and (3) corresponding to different diversity regimes. Figures from left to right correspond to  different cache sizes $ k \in \{25,125,250\}$, while figures from top to bottom correspond to  different exponent values $\alpha \in \{0.1, 0.2, 0.7\}$. $\OMD_\negent$ outperforms OGD in diverse regimes and small cache sizes, while OGD outperforms for large cache sizes and concentrated requests.}
  \label{fig:diversity_regimes_stationary}
\end{figure}


\subsubsection{Effect of Diversity.}
Figure \ref{fig:diversity_regimes_stationary} shows the $\mathrm{NAC}$ performance of $\OMD_\negent$ and OGD on the traces \emph{Batched Fixed Popularity} (1), (2), and (3) under different cache capacities $k$ and  exponent values $\alpha$. We observe that  $\OMD_\negent$ outperforms OGD in the more diverse regimes ($\alpha \in \{0.1, 0.2\}$). This is more apparent for smaller cache sizes $k$. In contrast, OGD outperforms $\OMD_\negent$ when requests are less diverse  ($\alpha =0.7$); again, this is more apparent for larger cache size $k$. These observations agree with Theorems~\ref{theorem:optimalq_q1} and \ref{theorem:optimalq_q2} in Sec. \ref{sec:optregimes}, which postulated that high diversity and small cache sizes favors $\OMD_\negent$.


\subsubsection{Robustness to Transient Requests.}
Figure \ref{fig:performance_partial_popularity_change} shows the normalized average cost of $\OMD_\negent$ and OGD over the \emph{Partial Popularity Change} traces,  evaluated under different diversity regimes. Dashed lines indicate the projected performance in the stationary setting (if request popularities stay fixed). 
% The diversity regimes are selected to provide different performance: in (a) $\OMD_\negent$ outperforms OGD, in (b) $\OMD_\negent$ has similar performance to OGD, and in (c) $\OMD_\negent$ performs worse than OGD.
 
 Across the different diversity regimes, we find the $\OMD_\negent$ is more robust to popularity changes. In (a), (b) and (c) $\OMD_\negent$ outperforms OGD in the non-stationary popularity setting: we observe a wider performance gap as compared to the stationary setting.
%  In (c), the algorithms exhibit similar performance.
 
 Figure \ref{fig:performance_changing} (a) and (b) show the normalized average cost over the  \emph{Global Popularity Change} trace for the policies OGD and $\OMD_\negent$, respectively. We observe in Figure \ref{fig:performance_changing} (b) the NAC of $\OMD_\negent$ performance degrades after each popularity change. This is a limitation due to the multiplicative nature of $\OMD_\negent$. When the algorithm learns that a file, say it $i$, is not important, it can set $x_{t,i}$ arbitrarily close to $0$. If, suddenly, this content becomes popular, then $\OMD_\negent$ adapts slowly, due to its multiplicative nature--remember Eq.~\eqref{eq:multi}. This is shown in Figure~\ref{fig:performance_changing} (b). We can overcome this limitation by requiring all state variables to be larger than some small $\delta>0$; $\OMD_\negent$ is then limited to  $\mathcal{X}_\delta$, the $\delta$ interior of the capped simplex $\mathcal{X}$. More precisely, the $\delta$ interior of the capped simplex is defined as  $\mathcal{X}_\delta \triangleq  \mathcal{X} \cap [\delta, 1]^N $. In Figure~\ref{fig:performance_changing} (c), we use $\delta = 10^{-4}$. This parameter indeed prevents the algorithm from driving the fractional allocations 
 %make caching decisions 
 arbitrary close to 0, improving its adaptability. Both algorithms outperform competitors (Fig.~\ref{fig:performance_changing} (d)). 
\begin{figure}[!t]
  \centering
  \subcaptionbox{$\alpha = 0.1$}{
  \includegraphics[width=.27\linewidth]{graphical_res/Aug/robustness_regime1.pdf}
  }
  \subcaptionbox{$\alpha = 0.3$}{
  \includegraphics[width=.27\linewidth]{graphical_res/Aug/robustness_regime2.pdf}
  }
  \subcaptionbox{$\alpha = 0.4$}{
  \includegraphics[width=.27\linewidth]{graphical_res/Aug/robustness_regime3.pdf}
  }
  \caption{NAC of OGD and $\OMD_\negent$ evaluated under different diversity regimes when $10\%$ of the files change popularity over time. We use traces \emph{Partial Popularity Change} (1), (2), and (3) corresponding to the different diversity regimes. The diversity regimes are selected, such that, in the stationary setting (dashed line): (a) $\OMD_\negent$ outperforms OGD, (b) $\OMD_\negent$ has similar performance to OGD and (c) $\OMD_\negent$ performs worse than OGD. We observe that $\OMD_\negent$ is consistently more robust to partial popularity changes than OGD.
  }
  \label{fig:performance_partial_popularity_change}
\end{figure}

\begin{figure}[!t]
  \centering
  %NAC of OGD%
  \subcaptionbox{NAC of OGD}{
    \includegraphics[width=.23\linewidth]{graphical_res/Aug/dynamic_ogd.pdf}
  }
  %NAC of $\OMD_\negent$%
  \subcaptionbox{NAC of $\OMD_\negent$}{
    \includegraphics[width=.23\linewidth]{graphical_res/Aug/dynamic_omd.pdf}
  }
  %NAC of $\delta-\OMD_\negent$%
  \subcaptionbox{NAC of $\delta$-$\OMD_\negent$}{
    \includegraphics[width=.23\linewidth]{graphical_res/Aug/dynamic_somd.pdf}
  }
  \subcaptionbox{NAC of FTPL}{
    \includegraphics[width=.23\linewidth]{graphical_res/Aug/ftpl_changing.pdf}
  }
  
  %NAC  of gradient algorithms best candidate vs classical policies LRU, LFU and W-LFU%
    \subcaptionbox{NAC of the different policies, LRU, Best static and Best dynamic.}{
    \includegraphics[width=.40\linewidth]{graphical_res/Aug/compare_changing.pdf}
  }
  \caption{NAC of the different caching policies evaluated on the \emph{Global Popularity Change} trace. The popularity of the requests changes sharply at fixed periods.  In (b), $\OMD_\negent$, operating over  the constraint set $\mathcal{X}$, adapts slowly, because multiplicative updates make it ``stuck'' in a corner configuration; in contrast, in (a), OGD adapts more seamlessly to  popularity changes. In (c), we see that modifying $\OMD_\negent$ to operate over the $\delta$-interior of $\mathcal{X}$ resolves this issue,  the cache states are bounded away from zero. Finally, both policies outperform competitors, as shown in (d).}
  \label{fig:performance_changing}
\end{figure}
\begin{figure}
    \centering
     \subcaptionbox{$R/h = 1$}{
    \includegraphics[width=.3\linewidth]{graphical_res/Aug/complexity_nonbatched.pdf}
  }
  \subcaptionbox{$R/h > 1$}{
    \includegraphics[width=.3\linewidth]{graphical_res/Aug/complexity_batched.pdf}
  }
    \caption{Runtime per iteration of $\OMD_\negent$ and $\OGD$. Subfigure (a) shows the runtime per 500 iterations over the \emph{Fixed Popularity} trace.  Subfigure (b) shows the runtime per 50 iterations over the \emph{Batched Fixed Popularity (2)} trace.   }. 
    \label{fig:time_complexity}
\end{figure}


\subsubsection{CDN Trace}
 Figure~\ref{fig:cdn_trace} shows that  the two gradient algorithms, $\OMD_\negent$ and OGD, perform similarly  over the CDN trace w.r.t. NMAC; OGD is slightly better in parts of the trace. Overall, these algorithms consistently outperform LRU, LFU, and W-LFU. Note that these caching policies process requests individually, while  gradient algorithms adapt slower, \emph{freezing} their state for the entire batch size ($R=5000$). Nevertheless, gradient algorithms still perform better.
\begin{figure}[!t]
    \centering
    \includegraphics[width=.45\linewidth]{graphical_res/Aug/CDN.pdf}
    \caption{NMAC of the different caching policies evaluated on the \emph{CDN Trace}. $\OMD_\negent$ and OGD provide consistently the best performance compared to W-LFU, LRU and LFU. OGD performs slightly better than OMD in some parts of the trace.}
    \label{fig:cdn_trace}
\end{figure}
\subsubsection{Randomized Rounding}
Figure \ref{fig:rounding_costs} shows the cumulative update cost for the online independent sampling, the online coupled rounding, and the online optimally-coupled rounding algorithms over the \emph{Downscaled Global Popularity Change} trace. All the rounding algorithms exhibit the same service cost in expectation. The update cost of online coupled rounding and the online optimally-coupled rounding is small, in the order of  the learning rate $\eta$; moreover, we observe that online optimally-coupled rounding yields lower update costs than the online coupled rounding. In contrast, online independent sampling incurs a significantly larger update cost.

Figure \ref{fig:rounding_caching_decisions} shows the fractional and (rounded) integral cache states  under \emph{Downsampled Global Popularity Change} trace when the cache size is $k=4$.   Independent sampling indeed leads to more frequent updates than  coupled rounding, while the latter maintains a more stable cache configuration by coupling the consecutive states and avoiding unnecessary updates.

\subsubsection{Computational Cost}
Figure~\ref{fig:time_complexity} shows the time taken by both policies OMD and \OMDNEG{} to perform 500 iterations over the \emph{Fixed Popularity} trace (Fig.~\ref{fig:time_complexity} (a)), and the time taken to perform 50 iterations over  the \emph{Batched Fixed Popularity (2)} trace (Fig.~\ref{fig:time_complexity} (b)). We observe that \OMDNEG{} is at least 15 times faster in computing cache states on average.
% ---80 times higher than coupled rounding.


\begin{figure}[!t]
  \centering
  \subcaptionbox{Normalized average cost}{
  \includegraphics[width=.32\linewidth]{graphical_res/Aug/rounding_nac.pdf}
  }%\hspace{5mm}
%   \subcaptionbox{NAC of independent sampling}{
%   \includegraphics[width=.22\linewidth]{graphical_res/rounding_independent_service_cost.png}
%   }
    \subcaptionbox{Cumulative update cost}{
  \includegraphics[width=.32\linewidth]{graphical_res/Aug/rounding_cuc.pdf}
  }%\hspace{5mm}
%   \subcaptionbox{CUC of independent sampling}{
%   \includegraphics[width=.22\linewidth]{graphical_res/rounding_independent_movement_cost.png}
%   }
  \caption{Costs associated with the rounded integral caching over the \emph{Downscaled Global Popularity Change} trace. The normalized average costs shown in (a) are the same for the online independent sampling, the online coupled rounding and the online optimally-coupled rounding. The cumulative update cost of the online coupled rounding and online optimally-coupled rounding in (b) is of the same order as in the fractional setting, while the online independent rounding in (b) gives a much higher update cost. The reported values are averaged over 20 experiments, and the blue shaded area represents 10\% scaling of the standard deviation. }
  \label{fig:rounding_costs}
\end{figure}


\begin{figure}[!t]
  \centering
  \subcaptionbox{Fractional cache states}{
  \includegraphics[width=.3\linewidth]{graphical_res/Aug/states_frac.pdf}
  }
     \subcaptionbox{Online independent sampling}{
  \includegraphics[width=.3\linewidth]{graphical_res/Aug/states_ind.pdf}
  }
  \\
  \subcaptionbox{Online coupled rounding}{
  \includegraphics[width=.3\linewidth]{graphical_res/Aug/states_coup.pdf}
  }
 \subcaptionbox{Online optimally-coupled rounding}{
  \includegraphics[width=.3\linewidth]{graphical_res/Aug/states_coup_opt.pdf}
  }
  \caption{Online rounding of fractional caching states. Visually, we see that the online independent rounding has more frequent updates than the online coupled rounding. This leads to large update costs. The online coupled rounding and the online optimally-coupled rounding  prevents the cache to perform unnecessary updates.  }
  \label{fig:rounding_caching_decisions}
\end{figure}




==> backups__zipped_project_/8._Conclusion.tex <==
\section{Conclusions}

We studied no-regret caching algorithms based on OMD with $q$-norm  and neg-entropy mirror maps.  Our analysis indicates that batch diversity impacts regret performance; a key finding is that OGD is optimal in low-diversity regimes, while $\OMD_\negent$ is optimal under high diversity. With an appropriately designed  rounding scheme, our $\BigO{\sqrt{T}}$ bound on the regret for general OMD algorithms extends to  integral caches as well, despite the need to account for update costs in this setting. 

Our numerical experiments indicate that the gap between the regimes in which OGD and $\OMD_\negent$ are optimal, w.r.t. the diversity ratio, is narrow; this suggests that our characterization of the two regimes can be further improved. Proving the optimality of $\OMD_\negent$ within the $q$-norm mirror map class, as opposed to merely its domination over OGD, is also open. Finally, devising strongly polynomial, efficient algorithms for the Bregman projection when $q\in(1,2)$, and characterizing update costs in this setting, also remain open problems.

==> backups__zipped_project_/acm-original-files/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> backups__zipped_project_/backup/S11-Related_work1.tex <==
Classical analysis techniques are based on the Time-to-Live (TTL) Caches. These cache models are used to encapsulate several caching policies such as LRU, FIFO and RND policies, this is analysed exactly by Berger et al. \cite{berger2014exact}, and approximately in the work of Gast and Houdt \cite{gast2017ttl}. The utility, or hit ratio are used as metrics to evaluate the performance of the different policies. 

Networks of caches found many applications in practice. This motivated several works to study the performance of cache networks. This is studied by Alouf et al. \cite{alouf2016performance} and Borst et al. \cite{borst2010distributed} for hierarchical network structures, e.g., the Domain Name Server (DNS) network architecture. More generally the work of Fong et al. \cite{fong1997}, Dehghan et al. \cite{dehghan2016complexity}, Ioannidis et al. \cite{ioannidis2010distributed} and Poularakis et al. \cite{poularakis2016exploiting} study distributed caching in networks.



%%%%%%%%%%% Adversarial, compare to dynamic optimum 
Caching under adversarial requests is a setting, in which the requests could potentially be generated by an adversary. A classical performance metric is to compare the performance of the cache relative to a dynamic optimum that is aware of the adversary's plan. This is classically studied under the name \emph{k-server} problem, this problem was introduced by Fiat et al. \cite{fiat1994competitive}. The performance metric is the bounded ratio between the cost experienced by a policy relative to a dynamic optimum. This ratio is called the \emph{competitive ratio}. More recently, Bubeck et al. \cite{bubeck_kserver_2018}, uses the framework of continuous online mirror descent to provide $o(k)$-competitive algorithm, that is independent of the underlying hierarchical separated tree (HST) metric.

%%%%%%%%%%% Adversarial, compare to fixed optimum
Recently, Paschos et al. \cite{PaschosLearningToCache} frame the caching problem as an online convex optimization problem. This setting also considers adversarial requests, with the distinction, that the performance metric is the difference between the cost experienced by a policy and the static optimum, this is called $regret$. They also give an online gradient descent policy that attains sub-linear regret. Bhattacharjee et al. \cite{FundamentalLimits} study the fundamental limits of this formulation.

% Regret vs Competitive ratio
Andrew et al.~\cite{taleoftwometrics} show that there is an intrinsic incompatibility between Regret and the competitive ratio, so that it is not possible for an algorithm to have both sub-linear regret and a constant competitive ratio. 

==> backups__zipped_project_/backup/S2-System_description1.tex <==
\section{System description}
\label{s:system}
\noindent\textbf{Remote Service and Local Cache.} We consider a system in which requests for files are served either remotely or by an intermediate cache of finite capacity. A cache miss incurs a file-dependent remote retrieval cost. Our goal is to study online algorithms for determining cache contents that attain sublinear regret. Formally, we consider stream of requests for  files of equal size from a catalog $\mathcal{N}=\{1,2,\dots, N\}$ .  These requests can be served by a remote server at cost $w_i \in \mathbb{R}_+$  per request for file $i\in\mathcal{N}$. This cost could be, e.g., an actual monetary cost for using the network infrastructure, or a quality of service cost incurred  due to fetching latency. Costs may  vary, as each file may be stored at a different remote location. We denote by %The cost of serving these files is summarized by a cost weight 
$\vec{w}=[w_i]_{i \in \mathcal{N}}\in \mathbb{R}_+^N$ the vector of costs %where $w_i \in \mathbb{R}_+$ is the cost of serving  file $i \in \mathcal{N}$. We assume that weights 
and assume that $\vec{w}$ is known.

 A local cache of finite capacity is placed in between the source of requests and the remote service. The local cache's role is to reduce the cost paid by the remote server, by satisfying requests locally. We denote by $k \in \{1,\dots,N\}$ the capacity of the cache. The cache is allowed to store fractions of files.  We assume that time is slotted, and  denote by $x_{t,i}\in[0,1]$  the fraction of file $i \in \mathcal{N}$ stored in the cache at  time slot $t \in \{1,2,\dots,T\}$.  The cache state is then given by vector $\vec{x}_t=[x_{t,i}]_{i\in \mathcal{I}}\in \mathcal{X}$, where $\mathcal{X}$ is the capped simplex  determined by the capacity constraint, i.e.: \begin{align}\mathcal{X} = \left\{ \vec{x} \in [0,1]^N : \sum^N_{i=1} x_i = k \right\}.\end{align}

\noindent\textbf{Requests.} We assume that a batch of multiple requests may arrive within a single time slot. Moreover, a file may be requested multiple times (e.g., by different users, whose aggregated requests form the stream reaching the cache) within a single time slot. We denote by $r_{t,i} \in \mathbb{N}$  the number of requests for file $i \in \mathcal{N}$ at time $t$, and by $\vec{r}_t=[r_{t,i}]_{i\in\mathcal{N}} \in \mathbb{N}^N$ the vector of such requests, representing the entire batch. We assume that the number of requests (i.e., the batch size) at each timeslot is given by $R \in \mathbb{N}$. We also assume that  the maximum multiplicity of a file in a batch is bounded by $h \in \mathbb{R}$. As a result, $\vec{r}_t$ belongs to set: 
\begin{align}\mathcal{R}_{R,h} = \left\{\vec{r} \in \{0,\dots, h\}^N : \sum^N_{i=1} r_i = R \right\}.\end{align}

Intuitively, the ratio $\frac{R}{h}$ defines the diversity of request batches in a timeslot. For example, as $\frac{R}{h} \to 1$, requests are concentrated on a single content. As $\frac{R}{h} \to N$, requests are spread evenly across the catalog $\mathcal{N}$. We note that this
generalizes Paschos et al.~\cite{PaschosLearningToCache}; their setting can be seen as the case $R = h = 1$ under our request model. 
We note that we make no prior assumptions on the stochasticity of request arrivals; put differently, we operate in the adversarial online setting, where a potential adversary may select an arbitrary request sequence in $\mathcal{R}_{R,h}$ to increase system costs.

\noindent\textbf{Service Cost Objective.} When a request batch  $\vec{r}_t$ arrives, the cache incurs the following cost:
\begin{align}
\label{e:cost}
f_{\vec{r}_t}(\vec{x}_t) = \sum^N_{i=1} w_i r_{t,i}(1 - x_{t,i}).\end{align}
In other words, for each file $i\in\mathcal{N}$, the remote server pays a cost proportional to the file fraction $(1-x_{t,i})$ missing from the local cache, weighted by the file cost $w_i$ and by the number of times $r_{t,i}$ that $i$ is requested in the current batch $\vec{r}_t$.


The cost objective \eqref{e:cost} captures several possible real-life settings. For example, assuming that each of the $R$ requests in the batch arrive and are served individually (e.g., either because they are spread-out within a timeslot, or because the fetching/QoS cost is paid separately for each user), leads to precisely the formulation in Eq.~\eqref{e:cost}. If, on the other hand, all requests are aggregated and served simultaneously, so that multiple requests for the same file are served by a single fetch operation, this can be captured by Eq.~\eqref{e:cost} with $h=1$ (so that the multiplicity of each file is at most 1, irrespective of how many users request it).

\noindent\textbf{Online Caching Algorithms and Regret.} Cache contents are determined online: that is, the cache has selected a state $\vec{x}_t \in \mathcal{X}$ at the beginning of a time slot.  The request batch $\vec{r}_t$ arrives, and the linear cost $f_{\vec{r}_t}(\vec{x}_t) : \mathcal{X} \to \mathbb{R}_+$ is incurred; the state is subsequently updated to $\vec{x}_{t+1}$. Formally, the  cache state is determined by an online policy $\mathcal{A}$, i.e.,  a sequence of mappings  $\{\mathcal{A}_t\}^{T-1}_{t=1}$, where for every $t \geq 1$, $\mathcal{A}_t : (\mathcal{R}_{R,h} \times \mathcal{X})^{t} \to \mathcal{X}$ maps the sequence of the request batches and previous decisions $\{(\vec{r}_s, \vec{x}_s)\}^{t}_{s=1}$ to the next state $\vec{x}_{t+1}\in \mathcal{X}$. We assume that the policy is initialised with a feasible state $\vec{x}_1\in \mathcal{X}$. 

 We measure the performance of an online algorithm $\mathcal{A}$ in terms of regret, i.e., the difference between the total cost experienced by a policy $\mathcal{A}$ over a time horizon $T$ and that of the best static state $\vec{x}_*$ in hindsight. Formally,
\begin{align}\text{Regret}_T(\mathcal{A}) = \underset{\{\vec{r}_1, \dots, \vec{r}_t\} \in \mathcal{R}^T_{R,h}}{\sup} \left\{ \sum^T_{t=1} f_{\vec{r}_t}(\vec{x}_t)- \sum^T_{t=1} f_{\vec{r}_t}(\vec{x_*}) \right\}. \label{eq:regret}\end{align}
where
$\vec{x_*}=\argmin_{\vec{x} \in \mathcal{X}}\sum^T_{t=1} f_{\vec{r}_t}(\vec{x})$ 
 is the optimal cache state (in hindsight). 
Note that, by taking the supremum in Eq.~\eqref{eq:regret}, we indeed measure regret in the adversarial setting, i.e., against an adversary that potentially picks requests in $\mathcal{R}_{R,h}$ trying to jeopardize  cache performance.
 
 %We are interested in the worst possible regret that can be incurred by $\mathcal{A}$:
%\begin{align}\text{Regret}_T(\mathcal{A}) = \underset{\{\vec{r}_1, \dots, \vec{r}_t\} \in \mathcal{R}^T_{R,h}}{\sup} \left\{ \sum^T_{t=1} f_{\vec{r}_t}(\vec{x}_t)-\underset{x_* \in \mathcal{X}}{\min} \sum^T_{t=1} f_{\vec{r}_t}(\vec{x_*}) \right\}. \end{align}

\noindent\textbf{Update Costs.} An online algorithm $\mathcal{A}$ updating the cache state at timeslot $t$ may require moving a portion of a file from a remote server to the cache. This is  not modeled in the cost (Eq.~\eqref{e:cost}) and, consequently, the regret (Eq.~\eqref{eq:regret}). This is indeed reasonable. First, the gradient-based algorithms we consider (see Sect.~\ref{sec:grad}) adapt the state by fetching fractions of files scaled by a gain $\eta\ll 1$; hence, by decreasing $\eta$, these update can be made arbitrarily small and, in particular, negligible compared to  file retrievals  satisfying requests, which are  accounted for in Eq.~\eqref{e:cost}. Second, even these negligible updates come for free for files requested in the previous timeslot. For example, increasing the $x_{i}$ for such a file $i$  can be performed by storing the small ($O(\eta)$) fraction of the ($1-x_i$) missing part of the file at the time of its retrieval. For these two reasons, we ignore this update cost in our analysis in  Sec.~\ref{sec:OMDanalysis}. In Sec.~\ref{xxx}, we revisit this issue, accounting also for update costs.   

==> backups__zipped_project_/backup/S4-Online_rounding.tex <==

\section{Online Rounding}
\label{sec:rounding}
In the previous sections, we assumed that the cache can store arbitrarily small chunks of a file. In practice the cache needs to store some metadata for each chunk and this overhead prevents the cache from splitting small files. These observations motivate us to study the case when the cache can only store the entire file, and the cache state consequently needs to be integral.

\subsection{Integral Caches} We denote the \emph{integral} cache configuration at time $t$ as $\boldsymbol{\zeta}_t$. It belongs to the set
%clearly a file can only have a finite number of chunks, and this can introduce application specific errors, e.g., rounding heuristics or the overhead cost caused by the chunks metadata, and these errors can be made more significant when the contents are small. To overcome these practical challenges, we are motivated to work with integral caching decisions. Let 
\begin{align}\mathcal{Z} = {\left\{ \boldsymbol{\zeta} \in \{0,1\}^N: \sum^N_{i=1} \zeta_i = k\right\}}.\end{align}
%be the set of possible integral cache configurations.

We are going to show that, by coupling OMD methods with opportune rounding techniques, the service-cost regret guarantees derived for the fractional setting transfer (in expectation) to the integral one. %
A straightforward approach is to use OMD to update a fractional state $\vec{x}_t\in \mathcal{X}$ and then randomly sample an integral state $\boldsymbol{Z}_t \in \mathcal{Z} $ after each round of requests so that $\mathbb{E}[\boldsymbol{Z}_t] = \vec{x}_t$, for all $t\geq 1$. 
%\begin{align}\mathbb{E}[\boldsymbol{Z}_t] = \vec{x}_t,\quad \text{for all}~t\geq 1.\end{align}
A random variable $\boldsymbol Z_t$ with the above marginals indeed exists, and can be sampled in polynomial time (see, e.g., \cite{geocaching2015, ioannidis2016adaptive}). In particular, 
Caratheodory's theorem \cite{rockafellar1970convex} guarantees that, for any~$\boldsymbol x_t$, the support of $\boldsymbol Z_t$ can be limited to at most $N$ cache configurations;  Warmuth and Kuzmin provided a practical algorithm \cite[Algorithm 2]{WarmuthRandomizedPCA}.

When sampling occurs independently from the past, we refer to this rounding scheme as \emph{independent sampling}.
The expected service cost incurred through independent sampling is, by the linearity of $f_{\vec{r}_t}$: 
\begin{align}
  \mathbb{E} \left[\sum^T_{t=1} f_{\vec{r}_t} (\boldsymbol Z_t)\right] &=\sum^T_{t=1} \mathbb{E} \left[f_{\vec{r}_t} (\boldsymbol Z_t)\right] =\sum^T_{t=1} f_{\vec{r}_t} \left(\mathbb{E} \left[\boldsymbol Z_t\right]\right) = \sum_{t=1}^T f_{\vec{r}_t} (\vec{x}_t).
\end{align}
The best static configuration $\vec{x}_*$ in the fractional setting can always be selected to be integral; this is because the objective and constraints are linear, so integrality follows from the fundamental theorem of linear programming. Hence, the expected regret for the service cost coincides with the regret of the fractional caching policy.


\subsection{Update Cost} Similarly to  Sec.~\ref{sec:movement}, we can introduce the update cost as
\begin{align}
\label{eq:movement_integer}
\updatecost_{\vec{r}_t} (\boldsymbol\zeta_{t}, \boldsymbol\zeta_{t+1} ) = \sum_{i \notin \supp(\vec{r}_t)} w_i' \max(0, \boldsymbol\zeta_{t+1,i} - \boldsymbol\zeta_{t,i}),
\end{align}
and extend similarly the regret notion as in Eq.~\eqref{eq:regret_extended}. Unfortunately, the update cost \emph{cannot} be neglected in this integral setting: 
\begin{theorem}
\label{theorem:rounding_independent}
Online independent sampling can incur an extra update cost that is $\Omega(T)$ in expectation.
\end{theorem}
The proof can be found in Appendix \ref{proof:rounding_independent}. This result implies that, when considering the more general definition of regret including the update cost, OMD coupled with independent sampling loses its $\BigO{\sqrt{T}}$ regret guarantee. 
%
Independent sampling causes more frequent cache updates, as it samples $\boldsymbol\zeta_{t+1}$ ignoring the current state $\boldsymbol\zeta_t$. Intuitively, coupling the two consecutive states may significantly reduce the expected update cost. Moreover,  if we manage to achieve $\BigO{\sqrt{T}}$ update cost in expectation, by the upper bound in Eq.~\eqref{eq:rounding_regret_upper_bound}  the generalized  regret will also be $\BigO{\sqrt{T}}$. The following theorem provides a sufficient condition relating the expected update cost to the weighted $l_1$ norm of the fractional change $\vec x_{t+1} - \vec x_t$. The weighted $l_1$ norm is defined as
\begin{align}\norm{\vec{z}}_{1, \boldsymbol w'} :=  \sum^N_{i=1} w_i' |z_i|.\end{align}
%We observe that $\text{MC}_{\vec{r}_t} (\zeta_{t}, \zeta_{t+1} ) \le \norm{\zeta_{t+1} - \zeta_t}_{1, \boldsymbol w'}$.
We observe that $\updatecost_{\vec{r}_t} (\boldsymbol\zeta_{t}, \boldsymbol\zeta_{t+1} ) \le \norm{\boldsymbol\zeta_{t+1} - \boldsymbol\zeta_{t}}_{1,\boldsymbol w'}$.
\begin{theorem}
\label{theorem:rounding_coupled}
Consider an OMD Algorithm and a joint distribution of $(\boldsymbol Z_t,\boldsymbol Z_{t+1})$ %of the random variables $\boldsymbol\zeta_t$ and $\boldsymbolrho_{t+1}$,
that satisfies:
\begin{enumerate}
    \item $\mathbb{E}[\boldsymbol{Z}_t] = \vec{x}_t$ and $\mathbb{E}[\boldsymbol{Z}_{t+1}] = \vec{x}_{t+1}$.
    \item $\mathbb{E} \left[ \norm{\boldsymbol Z_{t+1} -\boldsymbol Z_{t}}_{1, \boldsymbol w'}\right] = \BigO{\norm{\vec{x}_{t+1} - \vec{x}_{t}}_{1, \boldsymbol w'}}$.
\end{enumerate}
This algorithm incurs an expected service cost equal to the service cost of the fractional sequence. Selecting $\eta = \Theta\left(\frac{1}{\sqrt{T}}\right)$, gives a \BigO{\sqrt{T}} expected update cost. The regret is therefore \BigO{\sqrt{T}}.
\end{theorem}
The proof can be found in Appendix \ref{proof:rounding_coupled}. In the following section we show that there exists a coupling satisfying the assumptions of Theorem~\ref{theorem:rounding_coupled}.

\begin{algorithm}[!t]
	\begin{algorithmic}[1]
		\Procedure {Online Coupled rounding}{$\vec{x}_t, \vec{x}_{t+1}, \vec{\zeta}_t, p_t$}
	    \State Compute $I = \left\{ i \in \mathcal{N}: x_{t+1,i} - x_{t,i} > 0 \right\}$.
	    \State $m_i \gets |x_{t,i+1} - x_{t,i}|$
	    \State Obtain a flow $[\delta_{i,j}]$ that transports $\sum_{i \in \mathcal{N} \setminus I} m_i$ mass from the nodes $i \in \mathcal{N} \setminus I$ to the nodes $j \in I$.
	    \State $\zeta, p \gets (\zeta_t, p_t)$
	    \For {$ i \in \mathcal{N} \setminus I$}
	        \For {$ j \in I $}
	        \State $\zeta, p \gets$ \textsc{Elementary $\delta$-movement}($\delta_{i,j}, i, j, \vec{x}, \vec{\zeta}, p, $)
	        \EndFor
	    \EndFor
	    \State $\zeta_{t+1}, p_{t+1} \gets \zeta, p$
	    \State \Return $\zeta_{t+1}, p_{t+1}$
		\EndProcedure
	\end{algorithmic}
	\caption{Online coupled rounding}
	\label{algo:online_coupled_rounding}
\end{algorithm}


\subsection{Online Coupled Rounding}
\label{sec:online_coupled_rounding}
Assume at time $t$ the random variable $\boldsymbol Z_t$ with $\mathbb{E}[{\boldsymbol Z_t}] = \vec{x}_t $ has been used to sample the integral state $\boldsymbol \zeta_t$ and that the a-priori probability to sample $\boldsymbol \zeta_t$ was $\mathbb P(\boldsymbol Z_t = \boldsymbol  \zeta_t) = p_t$. 

Algorithm~\ref{algo:online_coupled_rounding} takes as input the fractional states $\vec{x}_{t}$ and $\vec{x}_{t+1}$, the integral state $\boldsymbol\zeta_t$ and its corresponding probability $p_t$. It implicitly constructs a new random variable $\boldsymbol Z_{t+1}$ with $\mathbb{E}[\boldsymbol Z_{t+1}] = \boldsymbol x_{t+1}$ and samples the new integral state $\boldsymbol \zeta_{t+1}$ from it. In more detail, the algorithm generates a sequence of random variables whose marginal distribution is progressively closer to $\vec{x}_{t+1}$. The marginal distributions of two consecutive random variables differ only for a $\delta_{i,j}$ mass moved from file $i$ to file $j$, i.e., the marginal distribution changes from $\vec x$ to $\vec x - \delta_{i,j} \vec e_i + \delta_{i,j} \vec e_j$. 
Each intermediate random variable is sampled through the procedure \textsc{Elementary $\delta$-movement} that is detailed in Algorithm~\ref{algo:elementary_movement} in Appendix~ \ref{app:online_rounding}.
Algorithm~\ref{algo:online_coupled_rounding} returns the new state $\boldsymbol \zeta_{t+1}$ and its corresponding probability $p_{t+1}$.  
% G: REMOVED TO GAIN SPACE
%Note that the algorithm does not keep track of the probability distribution of each random variable $\boldsymbol Z_t$, but only of the probability such distribution assigns to the sampled state $\boldsymbol \zeta_t$.

Starting then from an arbitrary random variable $\boldsymbol Z_1$ with $\mathbb{E}[\boldsymbol Z_{1}] = \vec{x}_{1}$, we can at each time slot use a policy $\mathcal A$ to generate the new fractional state $\vec{x}_{t+1}$ and then Algorithm~\ref{algo:online_coupled_rounding} to sample the integral state. 

The following theorem shows that Algorithm~\ref{algo:online_coupled_rounding} used with an OMD algorithm satisfies the hypothesis of Theorem~\ref{theorem:rounding_coupled} and, hence, provides sublinear regret when the learning rate is opportunely selected.
\begin{theorem}
\label{theorem:algorithm_rounding_coupled}
Algorithm~\ref{algo:online_coupled_rounding} outputs a random integral cache configuration $\boldsymbol Z_{t+1}$ with $\mathbb E[\boldsymbol Z_{t+1}] = \boldsymbol x_{t+1}$.
If the input to Algorithm~\ref{algo:online_coupled_rounding} is sampled from a random variable $\boldsymbol Z_t$ with $\mathbb E[\boldsymbol Z_t] =\vec{x}_t$, then $\mathbb E_{\boldsymbol Z_t}\left[\mathbb E_{\boldsymbol Z_{t+1}| \boldsymbol Z_t} \left[\norm{\boldsymbol Z_{t+1} -\boldsymbol Z_{t}}_{1, \boldsymbol w'}\right]\right] =  \BigO{\norm{\vec{x}_{t+1} - \vec{x}_{t}}_{1, \boldsymbol w'}}$.
\end{theorem}
The proof can be found in Appendix \ref{proof:algorithm_rounding_coupled}. We show that the change from $\vec{x}_t$ to $\vec{x}_{t+1}$ can be decomposed in at most $N-1$ elementary operations (corresponding to calls to the procedure $\textsc{Elementary $\delta$-movement}$), and that for each of them 
the expected  $\vec{w}'$-weighted $l_1$-distance between the sampled integral configuration is bounded by 
$\delta_{i,j} (w'_i + w'_j + 2 \norm{\vec w'}_\infty)$.

Finally, we note that one can find the  joint probability distribution of  $\boldsymbol Z_t$ and $\boldsymbol Z_{t+1}$ by formulating an optimal transport problem \cite{peyre2019computational} to minimize $\mathbb E\left[\norm{\boldsymbol Z_{t+1} - \boldsymbol Z_t}_{1,\boldsymbol w'}\right]$. This approach may lead a smaller expected update cost, but it requires to explicitly consider all possible values of $\vec Z_t$ and $\vec Z_{t+1}$, that may be as many as $|\mathcal Z| = {N \choose k}$. Our algorithm instead efficiently builds the support of these random variables at each step to have size at most linear in $N$.



==> backups__zipped_project_/backup/Z-CacheNetworks.tex <==

\clearpage
\begin{center}
{\Large  Caching Networks}
\end{center}

\begin{table}[t!]
  \caption{Caching networks notation summary.}
  \label{tab:cn_notations_definitions}
  \begin{tabular}{c p{0.8\linewidth}}
    % \hline
    % Notation&Definition\\
    \hline
&\textbf{Caching Network} \\
\hline
    $G(\vertices, \edges)$ & weighted undirected graph with vertices $\vertices$ and edges $\edges$ \\
    $w_{(p_{u}, p_{v})}$ & weight of edge $(p_{u}, p_{v}) \in \edges$ \\
   $k^v$ & caching capacity of node $v \in \vertices$\\
   $\catalog$ & catalog of files \\ 
    $(i, \vec\path)$ & request for item $i \in \catalog$ along the routing path $\vec\path$\\
    $k_{\vec\path}(v)$ & the position of node $v \in \vec\path$\\
    $\requestSet $ / $ \requestSet_i$ & set of all possible requests / set of all possible requests for file $i$ \\
    $R$ & maximum number of requests in a request batch \\  
    $\pathSet$ & set of all possible routing paths \\
    $\vec r$ & request batch vector, where $r_{(i,\vec\path)}$ is the number of request for file $i$ along $\vec \path$\\
    $\setRequestBatch$ & set of all possible request batches \\ 
    $\vec\repo^v$ & vector of permanent allocations at node $v$, where $\repo^v_i$ indicates whether file $i$ is permanently stored at $v$ \\ $\vec\repo$ & vector of permanent allocations of the caching network\\
    $t$ & timeslot \\
    $T$ & time horizon\\
\hline
&\textbf{Fractional Caching Networks} \\
\hline
 $\x^v$ & fractional cache state of node $v$, where $x^v_i$ gives stored fraction of file $i$ at node $v$ \\
 $\statesSetFrac^v$ & set of all possible fractional caching configurations at node $v$ \\
 $\x$ & fractional cache state of the caching network\\
  $\statesSetFrac$ & set of all possible fractional caching configurations for the caching network\\
    $C_{\vec r}(\x)$ / $G_{\vec r}(\x)$ & caching network gain / caching network cost for the fractional state $\x$ when request batch $\vec r$ is received \\
    $\text{Regret}_{T, \statesSetFrac}(\mathcal{A})$ & regret of policy $\mathcal{A}$ over the fractional domain $\statesSetFrac$ and time horizon $T$\\
    $\updatecost^v (\x^v, \x'^v)$ & update cost at cache node $v$ when the cache state is changed from $\x^v$ to $\x'^v$\\
    $\widehat{\text{Regret}}_{T, \statesSetFrac}(\mathcal{A})$ & extended regret that includes the update cost\\
\hline
&\textbf{Integral Caching Networks} \\
\hline
 $\z^v$ & integral cache state of node $v$, where $x^v_i$ indicates whether file $i$ at node $v$ \\
 $\statesSetInt^v$ & set of all possible integral caching configurations at node $v$ \\
 $\z$ & fractional cache state of the caching network\\
  $\statesSetInt$ & set of all possible fractional caching configurations for the caching network\\
    $\psi\text{-Regret}_{T, \statesSetInt}(\mathcal{A})$ & discounted regret of policy $\mathcal{A}$ over the fractional domain $\statesSetInt$ and time horizon $T$\\
    $\psi\text{-}\widehat{\text{Regret}}_{T, \statesSetInt}(\mathcal{A})$ & discounted extended regret that includes the update cost \\
    $\psi$ & discounting factor equal to $1-\frac{1}{e}$ \\
   \hline
&\textbf{Distributed Online Mirror Ascent} \\
\hline 
$\Phi^v(\x^v)$ & local mirror map at node $v$ \\
$\Phi(\x)$ & global mirror map ($\Phi(\x) = \sum_{v \in \vertices }\Phi^v(\x^v) $) \\
$\eta^v$ & local learning rate at node $v$ \\
$\vec g$ & subgradient of the gain function\\
$\vec g^v$ & local subgradient at node $v$ \\
$\y$ &  intermediate cache state of node $v$ \\
$\Pi_{\statesSetFrac^v \cap \mathcal{D}^v}^{\Phi^v}(\y)$ & local projection of the intermediate cache state of node $v$\\
\hline
\end{tabular}

\end{table}



\section{Fractional Caching Networks}
\subsection{System Model}

Our system model is detailed below, and the notation used across the paper is summarized in Table~\ref{tab:cn_notations_definitions}.

\noindent\textbf{Cache Nodes.}  The caching network is modeled as an undirected weighted graph $G(\vertices, \edges)$, where $\weight_{(u,v)}$ is the weight of the edge $(u,v) \in \edges$. A vertex $v \in \vertices$ represents a cache node in the network, and the weight $w_{(u,v)}$  represents the routing cost along the communication link between cache nodes $u$ and $v$. 

We consider a stream of requests for files of equal size from a catalog $\catalog \triangleq \{1,2,\dots, N\}$. The catalog of files is guaranteed to be served within the network through designated repository cache nodes, and we denote by $\repoNodeSet_i$ the set of cache nodes that permanently store file $i \in \mathcal{N}$.
We define the permanent allocations $\repo^v_i$ at node $v \in \vertices$ determined by the sets of repository cache nodes, where $\repo^v_i = 1$ when $v$ permanently stores $i$ ($v \in \repoNodeSet_i$) , and  $\repo^v_i = 0$ otherwise; therefore, the vector of permanent allocations at node $v$ is given as $\vec \repo^v = [\mathds{1}_{\{ v \in \repoNodeSet_i\}}]_{i \in \catalog}$, and for all nodes $\vec \repo = [\mathds{1}_{\{ v \in \repoNodeSet_i\}}]_{(v,i) \in \vertices\times\catalog}$.


As in Sec.~\ref{s:system}, we assume that time is slotted, and we denote by $x^v_{t,i}\in [0,1]$  the fraction of file $i$ stored at node $v \in \vertices$  at timeslot $t \in \{1,2,\dots,T\}$.  The cache state is then given by vector $\vec{x}^v_t=[x^v_{t,i}]_{i\in \mathcal{N}}\in \statesSetFrac^v$, where $\statesSetFrac^v$ is the capped simplex  determined by the capacity constraint $\capacity^k$, i.e.: \begin{align}\statesSetFrac^v = \left\{ \vec{x} \in [\repo^v_i,1]^N : \sum^N_{i=1} x_i = k^v\right\}.\end{align}
Naturally, we can also define the fractional caching network state of the caching network at time slot $t$ as $\vec x = [x^v_i]_{(i,v) \in \catalog \times \vertices}$ in the set $\statesSetFrac \triangleq \bigtimes_{v \in \vertices} \statesSetFrac^v$. 

\noindent\textbf{Requests.}
We assume that every node has a predefined routing path towards a suitable repository node for each file $i \in \catalog$. The routing is therefore predetermined, and our decisions only concern placement of files (i.e., variables $x^v_m$).

A routing path $\vec \path$ of length $|\vec \path| = K$ is a sequence $\{\path_1, \path_2, \dots, \path_K\}$ of nodes $\path_k \in \vertices$ such that edge $(\path_k, \path_{k+1}) \in \edges$ for every $k \in \{1, 2, \dots, K{-}1\}$. We define $k_{\vec \path} (v)$ to be the position of node along a path $\vec \path$, where for every $\path_k \in \vec\path$ we have $k_{\vec \path} (p_k) = k $, otherwise $k_{\vec \path} (v) = +\infty$ for $v \not \in \vec \path$. We assume that paths are simple, i.e., they do not contain repeated nodes. Let $\pathSet$ be the set of all possible routing paths. A request is therefore characterized by the pair $(i, \vec \path)$, where $i$ is the file requested and $\vec \path$ is the routing path to be traversed. This mechanism is illustrated in Fig.~\ref{fig:system_model}.

We denote by $\requestSet$ the set of all possible requests, and by $\requestSet_i$ the set of all possible requests for file $i$. When a request for file $i$ is propagated from node $\path_1$ toward the associated repository node $\path_K \in \repoNodeSet_i$, any intermediate node along the path that stores $i$ can serve it. 

We consider a batch of requests can arrive within a timeslot. We denote by $r_{t,(i,\vec\path)} \in \mathbb{N} \cup \{0\}$  the number of requests for file $i \in \catalog$ along path $\vec \path$ at time $t$, and by $\vec{r}_t=[r_{t,(i,\vec\path)}]_{(i , \vec\path) \in \catalog \times \pathSet}$ the vector of such requests, representing the entire batch. We denote by $R$ the maximum number of requests that can be received at timeslot $t$ and by $\mathcal{B}$ the set of all possible request batches defined as 
\begin{align}
    \mathcal{B} \triangleq \left\{ \vec r \in \left(\naturals\cup \{0\}\right)^{\catalog \times \pathSet} : \sum_{(i,\vec \path) \in \catalog \times \pathSet } r_{(i, \vec \path)}\leq R\right\}.
\end{align}
When a request batch  $\vec{r}_t$ arrives, the system incurs the following cost:
\begin{align}
\label{e:cost}
C_{\vec r_t}( \vec x_t) = \sum_{(i,\vec\path) \in \requestSet} r_{t, (i, \vec \path)} \sum^{|\vec\path|-1}_{k=1} \weight_{\left(\path_k,\path_{k+1}\right)}\left(1- \min\left\{1, \sum^k_{k'=1} x^{\path_{k'}}_{i}\right\}\right),
\end{align}
 In other words, for request $(i, \vec \path)\in\requestSet$, the system pays a cost proportional to: (i) the number of times $r_{t,(i,\vec \path)}$ request~$(i,\vec\path)$ is received in the current batch $\vec{r}_t$, and (ii) the sum of routing costs $\weight_{\left(\path_k,\path_{k+1}\right)}$ scaled by the  file fraction $\left(1- \min\left\{1, \sum^k_{k'=1} x^{\path_{k'}}_{i}\right\}\right)$ remaining to be fetched  at node $\path_{k}$, until the first node $k_*$ is found such that $\sum^{k_*}_{k'=1} x^{\path_{k'}}_{i} \geq 1$.\footnote{When the files are  encoded by
rateless MDS coding (e.g., fountain codes~\cite{raptor2006}), a file can be decoded given that $M$ parity codes are received. As in~\cite{shanmugam2013femtocaching}, the fractional state $x^v_i$ represents the fraction of parity bit of file $i\in \catalog$ are stored at node $v \in \vertices$.} 
 
 Instead of working with the cost $C_{\vec r_t}( \vec x_t) $, we can equivalently consider the \emph{caching gain} defined as the cost reduction due to the presence of the caches (as in \cite{shanmugam2013femtocaching,ioannidis2016adaptive,neglia2019swiss}):
\begin{align}
G_{\vec r_t}( \vec x_t) &= C_{\vec r_t}( \vec\repo) -  C_{\vec r_t}(  \vec x_t) \\ &=  \sum_{(i,\vec\path) \in \requestSet} r_{t, (i, \vec \path)} \sum^{|\vec\path|-1}_{k=1} \weight_{\left(\path_k,\path_{k+1}\right)} \min\left\{1, \sum^k_{k'=1} x^{\path_{k'}}_{i}\right\}.
\label{e:gain_cache_network}
\end{align}
The first term $C_{\vec r_t}( \vec\repo)$ on the right hand side is the service cost when only the repository allocations are present in the network.  A summary of the 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{graphical_res/Aug/SystemCDN.pdf}
    \caption{Caching networks: a network of cache nodes can reply to  requests for files along predefined routing paths. A repository node at the end of each path ensures that requests are satisfied even when there are no allocations on intermediate cache nodes. }
    \label{fig:system_model}
\end{figure}

% \noindent\textbf{Offline Problem.} The static caching network allocation problem can be formulated as finding the caching network allocation $\vec x^*$ that maximizes the aggregate allocation gain  over the time horizon $T$, i.e., 
% \begin{align}
%   \vec x_*  \in \underset{\vec z \in \statesSetInt}{\arg\max}\left( \sum^T_{t=1} G_{\vec r_t}( \vec x)\right).
%   \label{eq:static_gain}
% \end{align}
% The gain function $G_{\vec r_t}$ is concave for any $\x \in \statesSetFrac$ and $\vec r_t \in \setRequestBatch$ and $\statesSetFrac$ is a convex set; thus, the offline problem is a convex optimization problem  that can be solved efficiently.
\noindent\textbf{Online Fractional Caching Networks Algorithms and Regret.} As in Sec~\ref{s:system}, the cache contents are determined online by an online policy $\mathcal{A}$.  We measure the performance of an online algorithm $\mathcal{A}$ in terms of regret. The regret is defined as the gain loss in comparison to the best static allocation in hindsight. Formally,

\begin{align}
\text{Regret}_{T, \statesSetFrac}(\mathcal{A}) = \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{B}^T}{\sup} \left\{ \sum^T_{t=1} G_{\vec r_t}(\vec{x}_*)-\sum^T_{t=1} G_{\vec{r}_t}(\vec{x}_t) \right\},
\label{eq:cn_fractional_regret}
\end{align}
where
$\vec{x_*}=\arg\max_{\vec{x} \in \mathcal{X}}\sum^T_{t=1} G_{\vec{r}_t}(\vec{x})$ 
 is the optimal static cache state (in hindsight). 
 
\noindent\textbf{Update Cost and Extended Regret}
We can extend the caching network model to include the update cost of the cache states  at the end of every time slot $t$. The update cost at node $v \in \vertices$ is defined as
\begin{align}
\updatecost^v (\x^v_{t}, \x^v_{t+1} ) = \sum_{i \in \catalog } w'^v_{i} \max(0, x^v_{t+1,i} - x^v_{t,i}),
\label{eq:cn_update_cost}
\end{align}
where $w'^v_i$ is the cost of retrieving file $i$ at node $v \in \vertices$. We can then define the extended regret as 
\begin{align}
\widehat{\text{Regret}}_{T, \statesSetFrac}(\mathcal{A}) = \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{B}^T}{\sup} \left\{ \sum^T_{t=1} G_{\vec r_t}(\x_*)- \sum^T_{t=1} G_{\vec{r}_t}(\x_t)  + \sum^T_{t=1} \sum_{v \in \vertices} \updatecost^v(\x^v_t, \x^v_{t+1})\right\}.
\label{eq:cn_fractional_extended_regret}
\end{align}

 
 
\begin{algorithm}[!t]
	\begin{algorithmic}[1]
	    \State Sample $\xi^v$ u.a.r in the interval $[0,1]$.
		\Procedure {OnlineMirrorAscent}{$\vec{x}_1 \gets\underset{\vec{x}^v \in \statesSetFrac^v \cap \mathcal{D}^v}{\arg\min} \,\Phi^v(\vec{x}^v),  \eta^v$}
		\State $\vec z_1 \gets \CoupledRounding(\vec x_t, \xi^v)$ \Comment{Sample the initial physical cache state}
		\For{$t \gets1,2,\dots,T$}\tabto {5cm}

		\State Compute $\vec g^v_t$ as in Sec.~\ref{s:distributed_gradient_computation} \Comment{Request batch $\vec r_t$}
		\State
		$\hat{\vec{x}}^v_t\gets\nabla {\Phi^v} (\vec{x}^v_t)$\tabto {5cm}\Comment{{ Map primal point to dual point}}
		\State
		$\hat{\vec{y}}^v_{t+1}   \gets\hat{\vec{x}}^v_t + \eta^v \vec g^v_t$\tabto {5cm}\Comment{{ Take gradient step in the dual}}
		\State
		$\vec{y}^v_{t+1}   \gets\left(\nabla {\Phi^v}\right)^{-1}(\hat{\vec{y}}^v_{t+1})$\tabto {5cm}\Comment{{ Map dual point to a primal point}}
		\State
		$\vec{x}^v_{t+1}\gets\Pi_{\statesSetFrac^v \cap \mathcal{D}^v}^{\Phi^v}(\vec{y}^v_{t+1})$\tabto {5cm}\Comment{{ Project new point onto feasible region}}
		\State $\vec z^v_t \gets \CoupledRounding(\vec x_t, \xi^v) $ \Comment{Sample a physical cache state.}
		\EndFor
		\EndProcedure
	\end{algorithmic}
	\caption{Online Mirror Ascent ($\text{OMA}_{\Phi^v}$).}
	\label{algo:cn_online_mirror_ascent}
\end{algorithm}

\subsection{Distributed Online Mirror Ascent over Caching Networks}
In this section, we propose a family of caching policies based on Online Mirror Ascent (OMA) denoted by \AlgoName{} that operate in a distributed fashion without requiring global knowledge of the allocation state and requests arrival. 

For every timeslot $t$ the policy \LocalAlgoName{} in Algorithm~\ref{algo:cn_online_mirror_ascent} configured with mirror map $\Phi^v: \mathcal{D}^v\to \mathbb{R}$ and learning rate $\eta^v \in \reals_+$ updates the fractional caching states $\x^v_t\in\statesSetFrac^v{\subset} [0,1]^\catalog$ at every node $v \in \vertices$.  \LocalAlgoName{} uses a local mirror map $\Phi^v: \mathcal{D}^v \to \mathbb{R}_+$  to map $\x_t^v$ to a dual space before applying the gradient ascent method using a local subgradient $\vec g^v$; 
then the obtained state is mapped back to the primal space (lines 6--8 of Algorithm~\ref{algo:cn_online_mirror_ascent}). To compute a feasible fractional state $\x_{t+1}^v$, we perform a projection to the set $\statesSetFrac^v$  on node $v$ (line 6 of Algorithm~\ref{algo:cn_online_mirror_ascent}). \AlgoName{} is the collection of \LocalAlgoName{} policies running at each node $v \in \vertices$.
% We configure at each node the neg-entropy mirror map $\Phi^v(\x^v) = \sum_{i\in\catalog}\x^v_{i} \log(\x^v_{i})$.

% \noindent\textbf{Integral State Update.}
% Once the fractional state $\x^v$ has been updated, the final step of \LocalAlgoName{} is to determine a new random discrete allocation $\z^v$ and update the physical cache state accordingly. 

% The sampled allocation $\z^v$ should \textit{(i)}~comply with the capacity constraint on node $v$ (i.e., $\z_v \in \statesSetInt^v$) and \textit{(ii)} be consistent with the fractional state, i.e., $\mathds{E}[\z^v_{i}] = \x^v_{i} \; \forall  i \in \catalog$. This is achieved by calling \CoupledRounding{} in Algorithm~\ref{algo:online_coupled_rounding}.


In the next subsection we detail how each node computes its contribution to the global subgradient.


\subsection{Distributed Subgradient Computation}
\label{s:distributed_gradient_computation}
At the end of every time slot $t$, a subgradient $\vec{g}_t$ of the gain function in Eq.~\eqref{e:gain_cache_network} at point $\x_t \in \statesSetFrac$  is computed in a distributed fashion: each node $v$ evaluates the $(v,i)$-th component of the subgradient for any $i \in \catalog$ as follows (see Appendix~\ref{appendix:subgradient_expression}):
\begin{align}
   g^v_{t,i} = \sum_{(i,\vec\path) \in \requestSet_i}  r_{t, (i, \vec \path)} \sum^{|\vec\path|-1}_{k=k_{\vec \path} (v)}  \weight_{\left(\path_k,\path_{k+1}\right)} \mathds{1}_{\left\{\sum^k_{k'=1}x^{\path_{k'}}_{i} <  1 \right\}}.
   \label{eq:subgradient_expression}
\end{align}
The denote by $\vec g_t^v = [g^v_{t,i}]_{i \in \catalog}$ the vector of subgradient components local to node $v \in \vertices$ at timeslot $t$.

The subgradient can be computed at each node using only information from the control messages collected at the end of the time slot $t$ that piggy-pack the requests traffic. The steps needed to compute the subgradient are as follows.
\begin{enumerate}
    \item  At the end of the time slot,  each node generates a control message for every received request type $(i, \vec \path) \in \requestSet$ that is propagated along $\vec \path$. The control message contains the quantity $r_{i, (i, \vec\path)} \geq 1$ (the multiplicity of the request), and a cumulative counter $Z$ initialized to zero.
    \item 
    As the control message travels upstream, intermediate nodes add to $Z$ the local values $x^{\path_{k'}}_i$. This message is propagated until $Z \geq 1$, and let $k_*$ be the rank of such cache node.
    \item Once the $k_*$-th node is reached, a control message is sent down in the opposite direction, accumulating the routing costs $\weight_{\left(\path_k,\path_{k+1}\right)}$ scaled by the request multiplicity $r_{i, (i, \vec\path)}$. Every node $v$ in the reverse direction reads the cost value from the control message and, for each file $i \in \catalog$, computes the quantity
    \begin{align}
        h^v_{(i, \vec \path)} = r_{t, (i, \vec\path)} \sum^{k_*}_{k = k_{\vec \path(v)}}  \weight_{\left(\path_k,\path_{k+1}\right)} = r_{i, (i, \vec\path)} \sum^{|\vec\path|-1}_{k = k_{\vec \path(v)}}  \weight_{\left(\path_k,\path_{k+1}\right)} \mathds{1}_{\{ \sum^k_{k'=1}x^{\path_{k'}}_{i} <  1\}}
    \end{align}
    \item
    Node $v$ can then compute $g_{t,i}^v$ in Eq.~\eqref{eq:subgradient_expression} as follows
    \begin{align}
    \nonumber
        g^v_{t,i}=  \sum_{(i, \vec\path ) \in \requestSet_i} h^v_{(i, \vec \path)}.
    \end{align}
\end{enumerate}


\subsection{Regret Analysis for Generic Mirror Maps}
\label{sec:cn_regret_analysis}
In order to establish the regret guarantee of \AlgoName{}, we make a set of assumptions on the local mirror maps $\Phi^v$ at every node $v \in \vertices$:
\begin{enumerate}[label=(A\arabic*)]
    \item The map $\Phi^v: \domainPhi^v\to \reals^{\catalog}$ is a valid mirror map (see Sec.~\ref{section:OMD}).\label{asp:first_assumption}
    \item The mirror map $\Phi^v$ is $\theta^v$-strongly convex w.r.t a norm $d^v:\reals^\catalog \to \reals_+$ over $\statesSetFrac^v \cap \domainPhi^v$.
    \item The dual norm of $d^v:\reals^\catalog \to \reals_+$ is $d^{*v}:\reals^\catalog \to \reals_+$.
    \item Any local subgradient $\vec g^v$ at node $v \in \vertices$ of subgradient $\vec g$ of $G_{\vec r}(\x)$ at point $\x \in \statesSetFrac$ and request batch $\vec r \in \setRequestBatch$ is bounded under the dual norm $d^{*v}:\reals^\catalog \to \reals_+$ by $L^v_{\max}$, i.e., $d^{*v}(\vec g^v)\leq L^v_{\max}$. 
    \item The Bregman divergence $D_{\Phi^v} (\x^v,\x^v_1)$ is upper bounded by $D^v_{\max}$ for every node $v \in \vertices$ and $\x^v \in \statesSetFrac^v \cap \domainPhi^v$ for any $v \in \vertices$, where $\x^v_1 = \arg\min_{\x^v \in \statesSetFrac^v\cap\domainPhi^v} \Phi^v(\x^v)$ (line 2 in Algorithm~\ref{algo:cn_online_mirror_ascent}).
    \item The $l_1$ norm is upper bounded by $d^v(\,\cdot\,)$ where   $\norm{\,\cdot\,}_1 \leq M^v d^v(\,\cdot\,)$ for every $v \in \vertices$. \label{asp:upperbound_norm}
\end{enumerate}
The set of assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm} are satisfied when the mirror maps $\Phi^v$ are selected to be neg-entropy or the Euclidean mirror map for any $v \in \vertices$ (see Appendix~\ref{appendix:cn_properties_mp}). Table~\ref{tab:cn_constants} provides the constants for which the assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm} are satisfied for the neg-entropy and Euclidean mirror maps.
\begin{table}[t]
\[
\begin{array}{l|llllll}
\toprule
\text{Mirror map } \Phi^v(\x^v) & \theta^v & d^v(\,\cdot\,) & d^{*v}(\,\cdot\,) & L^v_{\max} & D^v_{\max} & M^v \\
\hline
\frac{1}{2} \norm{\x^v}^2_2 & 1 & \norm{\,\cdot\,}_2 & \norm{\,\cdot\,}_2 & R \max\{\sum^{|\vec\path|-1}_{k=k_{\vec\path} (v)} w_{(p_k, p_{k+1})}: \vec\path \in \pathSet\} & k/2 (1 - k/N)& \sqrt{N}\\
\sum_{i \in \catalog} x^v_i \log(x^v_i) & 1/k^v & \norm{\,\cdot\,}_1 & \norm{\,\cdot\,}_{\infty} & R \max\{\sum^{|\vec\path|-1}_{k=k_{\vec\path} (v)} w_{(p_k, p_{k+1})}: \vec\path \in \pathSet\}& k^v \log(N/k^v) & 1\\
\bottomrule
\end{array}
\]
 \caption{The constants for which  the neg-entropy and Euclidean mirror maps satisfy assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm} in Sec.~\ref{sec:cn_regret_analysis}.}
 \label{tab:cn_constants}
\end{table}



The following theorem establishes an upper bound on the regret of \AlgoName{} for fractional caching networks.
\begin{theorem}
When the local policy \LocalAlgoName{} in Algorithm~\ref{algo:cn_online_mirror_ascent} at every node $v \in \vertices$ is configured with the mirror map $\Phi^v$ (satisfying assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm}) and learning rate $\eta^v = \frac{1}{L^v_{\max}} \sqrt{\frac{2 \theta^v D^v_{\max}}{T}}$, the regret~\eqref{eq:cn_fractional_regret} satisfies:
\begin{align}
       \mathrm{Regret}_{T, \statesSetFrac}(\mathrm{OMA}_{\Phi^{\vertices}}) \leq \left(\sum_{v \in \vertices} L^v_{\max} \sqrt{\frac{2 D^v_{\max}}{\theta^v} }\right) \sqrt{T}\label{eq:cn_regret_bound},
\end{align}
\label{theorem:cn_regret_fractional}
\end{theorem}
The proof is given in Appendix~\ref{proof:cn_regret_fractional}.



We also provide in the following theorem an upper bound on the extended regret of \AlgoName{} for fractional caching networks.
% By selecting the learning rate $\eta^v =\sqrt{\frac{D^v_{\max} \theta^v}{\left( L^v_{\max}/2 + M^v w'^v_{\max}\right) L^v_{\max} T} }$ for every $v \in \vertices$ that gives the tightest upper bound, we finally get
% \begin{align}
%         \widehat{\text{Regret}}_{T, \statesSetFrac}(\mathcal{A})  \leq  \left( \sum_{v \in \vertices} L^v_{\max}\sqrt{\frac{2D^v_{\max} \left( 1 + 2 M^v w'^v_{\max} / L^v_{\max} \right) }{\theta^v}}\right) \sqrt{T}.
 \begin{theorem}
 When the local policy \LocalAlgoName{} in Algorithm~\ref{algo:cn_online_mirror_ascent} at every node $v \in \vertices$ is configured with the mirror map $\Phi^v$ (satisfying assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm}) and learning rate $\eta^v = \sqrt{\frac{D^v_{\max} \theta^v}{\left( L^v_{\max}/2 + M^v w'^v_{\max}\right) L^v_{\max} T}}$, the extended regret~\eqref{eq:cn_fractional_regret} satisfies:
 \begin{align}
     \widehat{\text{Regret}}_{T, \statesSetFrac}(\mathrm{OMA}_{\Phi^{\vertices}})  \leq  \left( \sum_{v \in \vertices} L^v_{\max}\sqrt{\frac{2D^v_{\max} \left( 1 + 2 M^v w'^v_{\max} / L^v_{\max} \right) }{\theta^v}}\right) \sqrt{T}.
 \end{align}
 \label{theorem:cn_extended_fractional_regret}
 \end{theorem}
 The proof is provided in Appendix~\ref{proof:cn_extended_fractional_regret}.
 \subsection{Offline Problem}
 \label{sec:cn_offline_problem}
  The static caching network allocation problem can be formulated as finding the caching network state $\vec x^* \in \statesSetFrac$ that maximizes the time-averaged gain  over the time horizon $T$, i.e., 
\begin{align}
  \vec x_*  \in \underset{\vec x \in \statesSetFrac}{\arg\max}\left( G_{T}(\x) \triangleq \frac{1}{T} \sum^T_{t=1} G_{\vec r_t}( \vec x)\right).
  \label{eq:cn_static_gain_fractional}
\end{align}


 We show in the following theorem that \AlgoName{} can be used a numerical solver for the offline problem when considering the subgradients (line 5 in Algorithm~\ref{algo:cn_online_mirror_ascent}) are taken from the fixed gain function $G_T$ in Eq.~\eqref{eq:cn_static_gain_fractional}. 
 \begin{theorem}
  Let $\bar \x$ be the average fractional caching network state $\bar \x \triangleq \frac{1}{K} \sum^K_{k=1} \x_i $ obtained by running \LocalAlgoName{} at every node $v \in \vertices$ (satisfying assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm}) for $K$ iterations, where $\x_k$ is the fractional state obtained at iteration $k$. When the   subgradients (line 5 in Algorithm~\ref{algo:cn_online_mirror_ascent}) are computed from  the fixed gain function $G_T$ in Eq.~\eqref{eq:cn_static_gain_fractional}, then by selecting the learning rates $\eta^v$ at every node $v \in \vertices$, the gain of $\bar \x$ satisfies:
      \begin{align}
    G_T(\bar\x)   \geq  G_T(\x_*)  - \left(\sum_{v \in \vertices} L^v_{\max} \sqrt{\frac{2 D^v_{\max}}{\theta^v} }\right) \frac{1}{\sqrt{K}}.
  \end{align}
  \label{theorem:cn_fractional_offline_problem}
 \end{theorem}
 The proof is provided in Appendix~\ref{proof:cn_fractional_offline_problem}.
 
\section{Integral Caching Networks}
\label{s:fractional_marginal}
In this section, we turn our attention to the scenario of integral caching networks where caching states can no longer be fractional, and files must be stored in their entirety. In  Proposition~\ref{proposition:deterministic_worst_case_regret}, we showed that any deterministic policy that operates over integral caching decisions have worst case regret, so we are only interested in randomized policies in this section. We denote by $\z^v_t$ the random integral caching state of node $v \in \vertices$ in the set of valid integral caching states given by 
\begin{align}
    \statesSetInt^v \triangleq \statesSetFrac^v \cap \{0,1\}^\catalog.
\end{align}
Naturally, we can also define the random integral caching network state at time slot $t$ as $\vec z = [z^v_i]_{(i,v) \in \catalog \times \vertices}$ in the set $\statesSetInt \triangleq \bigtimes_{v \in \vertices} \statesSetInt^v$. 

The random state  $\vec z^v_t$ of a cache node $v\in \vertices$ can be fully described by a distribution $p^v_t$ with support $\statesSetInt^v$, but it is unfeasible in practice to keep track of a distribution that is exponential in size $|\statesSetInt^v| = {N\choose k^v}$. We instead restrict ourselves to work with the first moment of such distribution given as $\x^v_t = \mathbb{E} [\z^v_t]$, where $x^v_{t,i}$ is the marginal probability that file $i \in \catalog$ is stored at cache node $v \in \vertices$ during timeslot $t$.

In Proposition~\ref{p:cn_moments}, we show that by restricting a policy to maintain only the first moment representation of the random cache states, although we lose a great amount of information about the original distribution, we can reconstruct a distribution $\tilde{p}^v_t$ with support $\tilde{\statesSetInt}^v \subset \statesSetInt$ that is  polynomial in size $|\tilde{\statesSetInt}^v|\leq N$; moreover, the cache states sampled from the new distribution $\tilde{p}^v_t$ yield the same expected caching gain as the cache states sampled from the original distribution $p^v_t$ as long as they are sampled independently for the different nodes $v \in \vertices$.


\noindent\textbf{Online Integral Caching Networks Algorithms and Regret.} 
Since the offline problem is NP-Hard, then the regret of an online policy $\mathcal{A}$ is measured as the gain loss in comparison to the best static allocation in hindsight discounted by a factor $\psi = 1 - \frac{1}{e}$. The regret against an $\psi$-approximation of the static optimum is denoted by $\psi$-regret~\cite{krause2014submodular}, and formally defined as 
\begin{align}
\psi\text{-Regret}_{T, \statesSetInt}(\mathcal{A}) = \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{B}^T}{\sup} \left\{ \psi\sum^T_{t=1} G_{\vec r_t}(\vec{z}_*)- \mathbb{E} \left[\sum^T_{t=1} G_{\vec{r}_t}(\vec{z}_t) \right]\right\}, 
\label{eq:cn_regret}
\end{align}
where the expectation is taken over the random cache states $\vec z_t$; moreover, we can extend the regret definition to account  for the update cost~\eqref{eq:cn_update_cost}, so we define the extended regret as
\begin{align}
    \psi\text{-}\widehat{\text{Regret}}_{T, \statesSetInt}(\mathcal{A}) = \underset{\{\vec{r}_1, \vec{r}_2, \dots, \vec{r}_t\} \in \mathcal{B}^T}{\sup} \left\{ \sum^T_{t=1} G_{\vec r_t}(\z_*)- \mathbb{E} \left[\sum^T_{t=1} G_{\vec{r}_t}(\z_t)  - \sum^T_{t=1} \sum_{v \in \vertices} \updatecost^v(\z^v_t, \z^v_{t+1})\right]\right\}.
    \label{eq:cn_psi_regret_extended}
\end{align}

\subsection{Regret Guarantees Transfer}
In this section, we show that the regret of any fractional caching network policy $\mathcal{A}$ with fractional states $\{\x_t\}^T_{t=1}$ can be transferred to the integral setting when the integral caching states are generated by \CoupledRounding{} with fractional caching state input $\x^v_t$ and random variable $\xi^v$  for every node $v \in \vertices$ and timeslot $t \in [T]$.
\begin{theorem}
\label{theorem:regret_generic_policy}
When  the random integral caching states $\z^v_t$ are  generated by \CoupledRounding{} with the fractional cache state input $\x^v_t$ for every $v\in\vertices$ and $t\in[T]$, then the $\psi$-regret guarantee over the random integral caching states satisfies:
\begin{align}
        \psi\mathrm{-Regret}_{T, \statesSetInt}(\mathcal{A})  \leq \psi \cdot   \mathrm{Regret}_{T, \statesSetFrac}(\mathcal{A}).
\end{align}
\end{theorem}
The proof is provided in Appendix~\ref{proof:regret_generic_policy}.

We provide the upper bound of the extended regret of \AlgoName{} for integral caching networks  in the following theorem.

\begin{theorem}
\label{theorem:cn_extended_psi_regret}
 When  the random integral caching states $\z^v_t$ are  generated by \CoupledRounding{} with the fractional cache state input $\x^v_t$, and the local policy \LocalAlgoName{} in Algorithm~\ref{algo:cn_online_mirror_ascent} is configured with the mirror map $\Phi^v$ (satisfying assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm}) and learning rate $\eta^v = \sqrt{\frac{2 D^v_{\max} \theta^v}{ \left( L^v_{\max} +2 kNM^v w'^v_{\max} / L^v_{\max} \right) L^v_{\max} T} }$ for every $v \in \vertices$ and $t \in [T]$, then the regret~\eqref{eq:cn_fractional_regret} satisfies:
 \begin{align}
     \widehat{\text{Regret}}_{T, \statesSetFrac}(\mathcal{A})  \leq  \left( \sum_{v \in \vertices} L^v_{\max}\sqrt{\frac{2D^v_{\max} \left( 1 + 2 kN M^v w'^v_{\max} / L^v_{\max} \right) }{\theta^v}}\right) \sqrt{T}.
 \end{align}
\end{theorem}
The proof is provided in Appendix~\ref{proof:cn_extended_psi_regret}.
\subsection{Offline Problem}
As in Sec.~\ref{sec:cn_offline_problem}, we seek $\vec z^* \in \statesSetInt$ that maximizes the aggregate gain~\eqref{eq:cn_static_gain_fractional} over the time horizon $T$, i.e., 
\begin{align}
  \vec z_*  \in \underset{\vec z \in \statesSetInt}{\arg\max}\,\, G_{T}(\z).
  \label{eq:cn_static_gain_integral}
\end{align}
In this integral setting  determining the best static allocation $\z_*$ is NP-Hard, and the problem admits at best a $1-\frac{1}{e}$ approximation in polynomial time~\cite{ioannidis2016adaptive}. We show in Corollary~\ref{corollary:cn_integral_offline_problem} that we can also use \AlgoName{} as a numerical solver to find a $1-\frac{1}{e}-\epsilon$ approximation of the static optimum in \BigO{\frac{1}{\epsilon^2}} iterations. 
\begin{corollary}
  Let $\bar \x$ be the average fractional caching network state $\bar \x \triangleq \frac{1}{K} \sum^K_{k=1} \x_k $ obtained by running \LocalAlgoName{} at every node $v \in \vertices$ (satisfying assumptions \ref{asp:first_assumption}--\ref{asp:upperbound_norm}) for $K$ iterations, where $\x_k$ is the fractional state obtained at iteration $k$. When the   subgradients (line 5 in Algorithm~\ref{algo:cn_online_mirror_ascent}) are computed from  the fixed gain function $G_T$ in Eq.~\eqref{eq:cn_static_gain_fractional}, then by selecting the learning rates $\eta^v$ at every node $v \in \vertices$, the gain of $\bar \z$ sampled using \CoupledRounding{} with input $\bar \x$ satisfies:
      \begin{align}
    \mathbb{E}\left[G_T(\bar\z) \right]   \geq \psi G_T(\z_*)  - \psi \left(\sum_{v \in \vertices} L^v_{\max} \sqrt{\frac{2 D^v_{\max}}{\theta^v} }\right) \frac{1}{\sqrt{K}}.
  \end{align}
  \label{corollary:cn_integral_offline_problem}
 \end{corollary}
 The proof is provided in Appendix~\ref{proof:cn_integral_offline_problem}.





